Enriching Automatic Test Case Generation by Extracting Relevant Test Inputs from Bug Reports

The quality of software is closely tied to the effectiveness of the tests it undergoes. Manual test writing, though crucial for bug detection, is time-consuming, which has driven significant research into automated test case generation. However, current methods often struggle to generate relevant inputs, limiting the effectiveness of the tests produced. To address this, we introduce BRMiner, a novel approach that leverages Large Language Models (LLMs) in combination with traditional techniques to extract relevant inputs from bug reports, thereby enhancing automated test generation tools. In this study, we evaluate BRMiner using the Defects4J benchmark and test generation tools such as EvoSuite and Randoop. Our results demonstrate that BRMiner achieves a Relevant Input Rate (RIR) of 60.03% and a Relevant Input Extraction Accuracy Rate (RIEAR) of 31.71%, significantly outperforming methods that rely on LLMs alone. The integration of BRMiner's input enhances EvoSuite ability to generate more effective test, leading to increased code coverage, with gains observed in branch, instruction, method, and line coverage across multiple projects. Furthermore, BRMiner facilitated the detection of 58 unique bugs, including those that were missed by traditional baseline approaches. Overall, BRMiner's combination of LLM filtering with traditional input extraction techniques significantly improves the relevance and effectiveness of automated test generation, advancing the detection of bugs and enhancing code coverage, thereby contributing to higher-quality software development.

==> Sections/BRMiner.tex <==
\section{\name}
\label{sec:brminer}

% This section presents an usage scenario and our approach for mining test input values from bug reports, implemented in a tool called \name.
This section introduces a usage scenario and details our approach for mining test input values from bug reports, which has been implemented in the tool \name.
%Additionally, this section introduces the definition of relevant inputs in the context of bug reports.

% \subsection{Value of bug reports}
% \label{subsec:valueofbugreports}
% Bug reports play a pivotal role in the software development process, serving as crucial documents that outline various software issues, their context, and potential solutions. These reports often contain detailed information about the observed behavior, the conditions leading to the issue, and, notably, specific inputs triggering the reported bugs. Typically, a bug report comprises a comprehensive description of the problem, including steps to reproduce it, the environment in which it occurred, and occasionally, the expected and actual results. Additionally, it may contain snippets of code, stack traces, and user logs, providing developers with an in-depth understanding of the problem.

\subsection{Usage scenario}
\label{subsec:usagescenario}
% In the context of software testing and quality assurance, bug reports offer a goldmine of valuable insights. They not only highlight existing software flaws but also provide a rich source of real-world inputs that can be harnessed to enhance the testing process. Consider the scenario where a developer, Bob, encounters a critical software issue that causes a crash when a specific variable, X, is set to 5. Upon documenting this observation in a bug report, the information becomes instrumental not only for understanding the root cause of the problem but also for informing the testing process.

% Although Bob may be aware of the value of this specific input, the proposed approach delves deeper into the collective wisdom embedded within bug reports, systematically extracting and utilizing such valuable inputs to strengthen the testing and debugging procedures. By effectively mining and integrating these inputs, the proposed tool empowers developers to proactively anticipate and address potential software issues, thereby enhancing the robustness and reliability of the software product. This proactive utilization of bug report inputs serves as a key strategy in fortifying the overall quality and resilience of the software, ensuring a smoother and more efficient development and testing process.
In the context of software testing and quality assurance, bug reports serve as a critical repository of real-world inputs that can significantly enhance the testing process. These reports not only highlight existing software flaws but also provide detailed contextual information, including specific inputs that may trigger bugs. However, extracting and utilizing these inputs effectively, especially across large or complex projects, presents a significant challenge.

Consider the scenario where a developer, Bob, encounters a critical software issue that causes a crash when a specific variable, X, is set to 5. While Bob recognizes the importance of this input and documents it in a bug report, the challenge extends beyond this isolated case. In a large-scale project, developers like Bob may face hundreds or thousands of such reports, each containing valuable inputs that could inform testing. Manually extracting these inputs from each report is not only time-consuming but also prone to error and oversight. \name is particularly beneficial in scenarios where the volume and complexity of bug reports make manual extraction of relevant inputs impractical. This tool systematically analyzes bug reports, identifying and extracting valuable literals—such as specific numbers, strings, and other data types—from descriptions, code snippets, error messages, and other contextual information within the reports. This automated approach ensures that even subtle or complex input patterns are captured and integrated into the testing process.

Consider a bug report describing a crash that occurs when a user enters a specific date format. While the report may mention the date format in passing, it might not explicitly identify it as the cause of the issue. \name can analyze the description, extract the relevant date format, and automatically incorporate it into a test case. This ensures that the software is thoroughly tested for different date formats, including those that might not have been immediately obvious as problematic.

\name excels in scenarios where the volume, complexity, and historical depth of bug reports pose significant challenges to manual analysis. By automating the extraction of valuable inputs, \name ensures that critical data is not overlooked, saving time and reducing the risk of human error. It effectively mines historical bug reports, uncovering inputs that remain relevant for current testing, and identifies complex and hidden inputs, such as those arising from intricate string manipulations or multiple method calls. Additionally, \name’s ability to analyze patterns across multiple reports provides crucial insights that enhance test cases and prevent the recurrence of similar bugs across different modules and project versions. 

By automating the extraction and utilization of these valuable inputs, \name empowers developers to anticipate and address potential software issues more effectively. This approach not only enhances the robustness and reliability of the software product but also plays a critical role in fortifying the overall quality and resilience of the software, ensuring a smoother and more efficient development and testing process.

% \subsection{Overview}
% \label{subsec:overview}
% \subsection{Approach overview}
% \label{subsec:overview}

% \begin{figure}
%     %\includegraphics [scale=0.45] {\brminer-approache}
%     % \includegraphics[width=8.5cm, height=8cm]{Images/approache-vf.pdf}
%     %\includegraphics[width=.9\linewidth]{Images/approache-vf-new.pdf}
%     \includegraphics[width=.99\linewidth]{Images/approache-llm-new.pdf}
%     \caption{Overview of \name, an automatic approach to extract potential test inputs from bug reports}
%     \label{fig:approach}
% \end{figure}

% Figure~\ref{fig:approach} shows a high-level overview of the \name approach. First, by using the respective APIs of GitHub\footnote{https://github.com/sigmavirus24/github3.py} and Jira\footnote{https://github.com/pycontribs/jira}, \name explores and parses the collected bug reports for potential relevant inputs (Section~\ref{subsec:rel-inputs}) and then it separates source code from natural language text (Section~\ref{subsec:rel-input-location}) by using Infozilla~\citep{bettenburg2008extracting},  a tool for extracting structural software engineering data from unstructured data sources such as e-mails, discussions, bug reports, and wiki pages. Finally, it extracts the inputs from source code by using a parser (Javalang\footnote{https://github.com/c2nes/javalang}) and those from natural language text by using regular expression. These extracted inputs can be used to assist the automated test generator.

% %We first parsed each bug report using the respective APIs of GitHub [] and Jira [] and tokenized them with a source code tokenizer []. Next, we parsed the test %cases associated with the bug reports using a Java parser [] to extract the literals (string, integer, float, and hexadecimal).

% Figure~\ref{fig:approach} provides a high-level overview of the \name approach, detailing the key steps involved in extracting valuable inputs from bug reports for automated test generation. The process begins with \name leveraging the respective application programming interfaces (APIs) of GitHub\footnote{https://github.com/sigmavirus24/github3.py} and Jira\footnote{https://github.com/pycontribs/jira} to comprehensively explore and parse the collected bug reports, identifying potential relevant inputs (as outlined in Section~\ref{subsec:rel-inputs}).

% Subsequently, the tool employs Infozilla~\citep{bettenburg2008extracting}, a specialized software for extracting structural software engineering data from unstructured sources such as emails, discussions, bug reports, and wiki pages, to segregate the source code from the natural language text. In Section~\ref{subsec:rel-inputs}, we showed that inputs can be found either in source code as in Figure \ref{fig:identic-input} or directly in natural language text. Therefore, given a bug report that we parsed, we separate natural language text from source code. This segregation process facilitates a clear distinction between the software's codebase and the descriptive content provided within the bug reports.

% The next step involves the extraction of inputs from the source code, which is accomplished through the use of Javalang\footnote{https://github.com/c2nes/javalang}, a robust parser specifically designed for analyzing Java source code. Simultaneously, \name employs regular expressions to extract inputs from the natural language text, enabling the identification of key data elements within the textual descriptions.

% The extracted inputs from both the source code and the natural language text are subsequently harnessed to assist the automated test generator, facilitating the development of more comprehensive and effective test suites. By seamlessly integrating these extracted inputs into the testing process, \name empowers developers to optimize their testing procedures, thereby enhancing the overall robustness and reliability of the software product.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Approach overview}
\label{subsec:overview}
Figure~\ref{fig:approach} provides a high-level overview of the \name  approach, detailing the key steps involved in extracting and refining relevant test inputs from bug reports for automated test generation. These steps are systematically outlined in Algorithm~\ref{alg:BRMiner}, which details the sequential process of parsing, separating, and extracting literals, followed by the integration of Large Language Models (LLMs) for input refinement. The approach is designed to address key challenges in test input generation, including handling complex literals, ensuring the relevance of extracted inputs  and effectively incorporating these inputs into automated test generation tools like EvoSuite and Randoop.

\begin{figure}
    %\includegraphics [scale=0.45] {\brminer-approache}
    % \includegraphics[width=8.5cm, height=8cm]{Images/approache-vf.pdf}
    %\includegraphics[width=.9\linewidth]{Images/approache-vf-new.pdf}
    \includegraphics[width=.99\linewidth]{Images/approache-llm-new.pdf}
    \caption{Overview of \name, an automatic approach to extract potential test inputs from bug reports}
    \label{fig:approach}
    \vspace{3mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{BRMiner Approach}\label{alg:BRMiner}
\begin{algorithmic}[1]

\State \textbf{Input:} Bug reports from GitHub/Jira (Title, Description, Comments)
\State \textbf{Output:} Refined list of relevant inputs for test case generation

\State

\Procedure{BRMiner}{}
    \State \textbf{Step 1: Parse Bug Reports}
    \For{each Bug Report $B_i$ in Repository}
        \State Parse $B_i$ to extract \textit{Title, Description, Comments}
    \EndFor
    
    \State
    
    \State \textbf{Step 2: Separate Code and Text}
    \For{each Bug Report $B_i$}
        \State Use \textit{Infozilla} to separate \textit{source code} from \textit{natural language text}
    \EndFor
    
    \State
    
    \State \textbf{Step 3: Extract Potential Inputs}
    \For{each Bug Report $B_i$}
        \State Use \textit{Javalang} parser to extract literals (strings, numerics) from source code
        \State Use \textit{Regex} to extract literals (strings, numerics) from natural language text
        \State Store extracted inputs as \textit{Potential Relevant Inputs} $P_i$
    \EndFor
    
    \State
    
    \State \textbf{Step 4: Integrate LLM for Filtering}
    \For{each Bug Report $B_i$}
        \State Generate a \textit{Tree of Thoughts (ToT)} prompt based on $B_i$ and $P_i$
        \State Query \textit{GPT-3.5-turbo} with ToT prompt to analyze and filter $P_i$
        \State Retrieve a refined list of relevant inputs $R_i$ from LLM
    \EndFor
    
    \State
    
    \State \textbf{Step 5: Generate Test Cases}
    \State Integrate $R_i$ into \textit{EvoSuite’s} static input pool
    \State Use EvoSuite to generate test cases based on $R_i$
    
    \State \textbf{Return} Generated test cases
\EndProcedure

\end{algorithmic}
%\vspace{3mm}
\end{algorithm}
\vspace{5mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{\textbf{Initial Steps: Parsing and Extraction}}
%\paragraph{Initial Steps: Parsing and Extraction}
\subsubsection{Initial Steps: Parsing and Extraction}
The \name process begins by leveraging the application programming interfaces (APIs) of GitHub\footnote{https://github.com/sigmavirus24/github3.py} and Jira\footnote{https://github.com/pycontribs/jira} to systematically explore and parse bug reports. This step is crucial for identifying potential relevant inputs embedded within the reports, which may include titles, descriptions, and comments. To accurately segregate different types of information within the bug reports, BRMiner employs Infozilla~\citep{bettenburg2008extracting} to separate source code snippets from natural language text. This segregation allows for a clearer distinction between the software's codebase and the descriptive content provided within the bug reports.

\subsubsection{Literal Extraction from Source Code and Natural Language Text}
Once the text and code have been separated, BRMiner proceeds to extract relevant literals using two complementary methods:
\begin{itemize}[leftmargin=*]
    \item {\bf Source Code Extraction:} Using Javalang\footnote{https://github.com/c2nes/javalang}, a robust parser designed for analyzing Java source code, BRMiner identifies and extracts string and numeric literals embedded within the code snippets associated with the bug reports. These literals might include hardcoded values, constants, or any other relevant data embedded directly in the code.

    \item {\bf Natural Language Text Extraction:} Regular expressions (regex) are employed to extract similar literals from the natural language text found in the bug reports. This includes strings enclosed in single or double quotes and numeric values, which could represent key parameters, user inputs, or other critical data mentioned in the bug descriptions.
\end{itemize}
For instance, regex patterns are used to identify and extract strings that may represent variable names, error messages, or specific input values, as well as numeric literals that describe conditions or thresholds leading to a bug.

\subsubsection{Application of Extracted Inputs in Test Case Generation}
The refined inputs produced through the \name approach are then incorporated into EvoSuite’s static input pool, where they serve as seed inputs for automated test generation. EvoSuite leverages these inputs to explore different execution paths and generate comprehensive test suites, thereby enhancing the robustness and reliability of the software.

To establish a baseline for comparison, experiments were also conducted using an LLM alone, without any pre-extracted inputs. In this scenario, the LLM independently analyzes the bug report content to determine relevant test inputs, which are then used for test generation. This baseline helps assess the effectiveness of \name in improving test input relevance. Furthermore, to address concerns about the generalizability of \name across different testing methodologies, we extended our evaluation by incorporating Randoop, a feedback-directed random testing tool. Randoop was used with the same input scenarios, allowing us to benchmark \name against another well-established testing methodology.


%%%%%%%For discussion part
%%%%ajouter un système de priorisation d'input pour le cas des versions différentes
\subsubsection{Technical Challenges and Considerations}
BRMiner is designed to effectively manage complex scenarios where literals may be involved in concatenations or method calls, ensuring the entire concatenated string or argument values are extracted and used in test generation. The tool primarily focuses on extracting relevant inputs from bug reports to enhance the quality of test cases generated by automated tools like EvoSuite or Randoop, which are responsible for generating assertions and validating outputs. 

While BRMiner is not specifically designed to address discrepancies across different software versions, this limitation is mitigated by the versatility of automated test generators, which utilize a variety of inputs to cover diverse execution paths. Although version differences may influence the relevance of some inputs, the broad range of generated test cases typically ensures robust coverage. Additionally, BRMiner’s utility extends to smaller projects by providing a valuable database of pre-extracted inputs, which can be used to bootstrap testing processes even in the absence of extensive bug report histories. This input database is particularly beneficial in Java projects that share common libraries, as it enables comprehensive test case generation across different projects, regardless of the size or age of the project.

% \subsection{Relevant inputs} 
% \label{subsec:rel-inputs}
% In this section, we define what constitutes a relevant input in the context of a bug report.
% %This first step is crucial, as it allows a better understanding of the exploration of bug reports and the next two steps, i.e. the location and the extraction of relevant inputs. But before we identify a relevant input, it is important to define it. \par
% According to Toffola et al.~\citep{ASE-2017-ToffolaSP} and Shahbaz et al.~\citep{shahbaz2012automated} relevant inputs are those that bypass domain-specific sanity checks. In~\citep{mcminn2012search} and also in~\citep{shahbaz2012automated}, relevant inputs are those which are branch-covering and human-readable, especially for cases where there is no automated oracle. Mariani et al.~\citep{mariani2014link} define relevant inputs as inputs that are both syntactically correct and semantically valid and meaningful. While Bozkurt et al.~\citep{bozkurt2011automatically} describe relevant inputs as realistic. Liu et al.~\citep{liu2017automatic} describe relevant inputs as those appropriate to the context.
% From these definitions, a relevant input is an input that is realistic, appropriate to the context or domain, that provides good code coverage, and above all, that allows to detect bugs.

% To define relevant inputs for our tasks, further investigations of both bug reports and human-written test cases are essential.
% %\jk{In the next paragraph, you focus on bug reports, so I guess, we should say: "further investigations of both bug reports and  human-written test cases are essential."}
% %Given a bug report, to make it easier to identify a relevant input, this led us to ask a first research question regarding the definition of a relevant input. \par
% %\textbf{RQ 1: What constitutes a relevant input in the context of a bug report?} \par \lp{remove RQ and rephrase}
% The manual exploration of hundreds of bug reports reveals that the information contained therein differs depending on the user raising an issue. While some bug reports mention input values, API (or method) used, expected values, and actual values, others additionally mention wrapper code and some code portion to reproduce. Therefore, a manual analysis of the bug reports and test cases written by humans to pass the patched version revealed that some input values appearing in some bug reports were also present in the test cases. As an example, we can see in Figure~\ref{fig:identic-input} that some of the inputs mentioned in the bug report appear in the test case.


% % \begin{figure}
% %     \includegraphics[width=8.5cm, height=8cm]{Images/identic-input}
% %     \caption{Input value mentioned in the bug report for issue 3447 in the FasterXML jackson-databind library is in a test case written by a developer after fixing the bug.}
% %     \label{fig:identic-input}
% % \end{figure}


% \begin{figure}
% \centering
%     \subfloat[Bug report.]{
%         \includegraphics[width=.9\linewidth]{Images/identic-input-A1}
%     }\quad
%     \subfloat[Developer-written test case]{%
%         \includegraphics[width=.9\linewidth]{Images/identic-input-A2}
%     }
%   \caption{Input value mentioned in the bug report for issue 3447 in the FasterXML jackson-databind library appears in a test case written by a developer after fixing the bug.}
%   \label{fig:identic-input}
% \end{figure}


% In some cases, the input in the test case is not identical to that provided by the user in the bug report but has the same pattern or format. Figure \ref{fig:same-patern} shows an example of a case where the input in the bug report and the one used in the test case have the same pattern but are not identical.
% \begin{comment}
% \begin{figure}
%     \includegraphics [width=8.5cm, height=8cm]{Images/same-patern}
%     \caption{Pattern of the input value mentioned in the bug report for issue 1205 in the Apache Commons Lang library library is in a test case written by a developer after fixing the bug.}
%     \label{fig:same-patern}
% \end{figure}
% \end{comment}

% \begin{figure}
% \centering
%     \subfloat[Bug report.]{
%         \includegraphics[width=.9\linewidth]{Images/same-patern-A1}
%     }\quad
%     \subfloat[Developer-written test case.]{%
%         \includegraphics[width=.9\linewidth]{Images/same-patern-A2}
%     }
%   \caption{Pattern of the input value mentioned in the bug report for issue 1205 in the Apache Commons Lang library appears in a test case written by a developer after fixing the bug.}
%   \label{fig:same-patern}
% \end{figure}


% From these two observations, we can say that, from the perspective of a bug report, {\em an input is relevant if we use it or its pattern to pass a human-written test after the patching}. 
% Hence, it becomes challenging to verify whether an input extracted from a bug report, distinct from the one included in a human-written test case, holds significant relevance. It's important to note that not all inputs mentioned in a bug report are relevant, and conversely, not all inputs that differ from those in the test case are irrelevant.
% Therefore, for the purpose of evaluating the rate of relevant inputs in bug reports and to assess BRMiner's capability in extracting such inputs we will only consider this definition in its strictest form, i.e., when the inputs are identical.

% \subsection{Relevant input location}
% \label{subsec:rel-input-location}
% From the bug report exploration and the identification of relevant inputs, we know that inputs can be found either in source code as in Figure \ref{fig:identic-input} or directly in natural language text. Therefore, given a bug report that we parsed, we separate natural language text from source code. To this end, \name used Infozilla: running Infozilla on a bug report returns natural language text with all structural elements removed and a machine-analyzable representation of all structural elements.

% \begin{comment}
% \begin{figure}
%     \includegraphics [width=8.5cm, height=8cm]{Images/input-in-natural-langage}
%     \caption{Inputs are part of natural language text.}
%     \label{fig:input-in-natural-langage}
% \end{figure}
% \end{comment}


% %Fig4

% % \begin{figure}[h!]
% % \centering
% %     \subfloat[Bug report.]{
% %         \includegraphics[width=.9\linewidth]{Images/input-in-natural-langage-A1.pdf}
% %     }\quad
% %     \subfloat[Developer-written test case.]{%
% %         \includegraphics[width=.9\linewidth]{Images/input-in-natural-langage-A2.pdf}
% %     }
% %   \caption{Input values mentioned in the bug report for issue 1462 in the Apache Commons Lang library appear in a test case written by a developer after fixing the bug are part of natural language text.}
% %   \label{fig:input-in-natural-langage}
% % \end{figure}

==> Sections/Background.tex <==
\section{Background}
\label{sec:background}
%\textbf{Search-based Test Suite Generation and Dynamic Symbolic Execution}\\
This section presents the foundational concepts and methodologies that support our approach, including Dynamic Symbolic Execution (DSE), EvoSuite, LLM-based test input generation, and prompt engineering techniques.

\subsection{DSE and EvoSuite}
\label{sec:dse-evosuite}
Dynamic Symbolic Execution (DSE) is among the widely adopted techniques for automated test case generation~\citep{valle2022mutation}. This method simultaneously explores multiple paths of the source code using symbolic values in place of concrete ones. Employing a symbolic execution engine enables efficient control over the paths traversed within the source code~\citep{baldoni2018survey}. Its applications include the automated generation of unit tests and the identification of actual defects or memory overflows~\citep{cadar2013symbolic}.

While Search-based testing excels at formulating unit test suites for object-oriented code, it occasionally falters in producing specific values for intricate code parts. In contrast, Dynamic Symbolic Execution (DSE) shines in creating these precise values but finds complexity when faced with data types necessitating a chain of calls. \citet{galeotti2013improving} paved the way for a combined technique, leveraging the advantages of both methods. They refined the Genetic Algorithm (GA) within EvoSuite to smoothly incorporate DSE and, guided by search feedback, determined the optimal moments to employ DSE. This modification led to a jump in average branch coverage. Furthermore, when compared to standalone DSE tools, EvoSuite combined with DSE proved superior in achieving coverage. Empirical analyses underscored the practical advantages of integrating SBST and DSE, with negligible downsides. 

In subsequent research, \citet{galeotti2014extending} highlighted that this fusion not only augments coverage and effectiveness but also upholds SBST's flexibility in tailoring test suites for various metrics and non-functional factors. Crucially, this approach ensures that all test cases correspond to legitimate object conditions. As a testament to its capabilities, EvosuiteDSE made a notable debut at the ninth unit testing competition during SBST 2021, registering a commendable score of 47.14.

\subsection{LLM-based Test Input Generation}
\label{sec:llmbased-test-input}
LLMs have recently gained traction in the field of software testing, particularly in generating or refining test inputs that are both contextually relevant and semantically aligned with the software under test~\citep{fan2023large,wang2024software}. These models, built primarily on the Transformer architecture~\citep{vaswani2017attention}, are trained on vast corpora of text and code using techniques such as Masked Language Modeling and Causal Language Modeling~\citep{shanahan2024talking,naveed2023comprehensive}. The resulting models, including BERT~\citep{devlin2018bert}, GPT~\citep{brown2020language,yenduri2024gpt}, and T5~\citep{raffel2020exploring}, have been enhanced with methods like Reinforcement Learning from Human Feedback (RLHF)~\citep{ziegler2019fine,bai2022training}, which improves their alignment with human intent.

In the context of test input generation, LLMs have demonstrated significant potential in generating diverse and realistic inputs~\citep{liu2024testing,yang2023white}. These models can analyze natural language descriptions, such as bug reports or user stories, to extract meaningful inputs that can be used to trigger specific software behaviors~\citep{tsigkanos2023variable}. By leveraging the extensive knowledge embedded in LLMs, these inputs are not only syntactically correct but also semantically relevant, thereby improving the effectiveness of test cases in uncovering bugs.

Recent advancements in the field have seen LLMs being integrated with traditional testing tools to enhance the coverage and precision of generated test cases. For instance, in the \name approach, an LLM like GPT-3.5-turbo is leveraged to refine extracted inputs from bug reports, ensuring that they are contextually appropriate and likely to trigger relevant software faults. This refinement process is crucial for improving the overall quality of the test cases and increasing the likelihood of exposing latent defects that might be missed by conventional test generation methods.


\subsection{Prompt Engineering}
\label{sec:prompt-engineering}
Prompt engineering involves creating prompts that enable LLMs to effectively address specific tasks~\citep{amatriain2024prompt,siddiq2024quality,vogelsang2024using,naveed2023comprehensive}. This technique is particularly valuable in complex problem-solving scenarios where a single line of reasoning might not be sufficient~\citep{amatriain2024prompt,kojima2022large,wei2022chain,reynolds2021prompt}. By guiding LLMs to consider multiple possibilities before reaching a conclusion, prompt engineering allows these models to adopt a more human-like approach to reasoning.

Prompt engineering is a rapidly evolving field that focuses on crafting prompts to guide LLMs in generating desired outputs, ranging from broad descriptions to detailed specifications. The importance of prompt engineering is twofold: firstly, highly specific prompts yield precise responses, while more general prompts may produce less relevant outputs~\citep{si2022prompting}. Secondly, by carefully adjusting the instructions within prompts, it is possible to control the output format of LLMs, thereby minimizing the need for post-processing and improving the performance evaluation~\citep{macedo2024exploring}.

Various studies~\citep{fan2023large,wang2024software} have leveraged LLMs and prompt engineering for automated software engineering tasks, traditionally employing approaches such as Zero-shot~\citep{kojima2022large} and Few-shot learning~\citep{brown2020language}. However, recent advancements have broadened the scope of prompt engineering to include more sophisticated techniques such as Chain-of-Thought~\citep{wei2022chain} and Tree-of-Thoughts~\citep{yao2024tree, long2023large}.

\textbf{Zero-shot learning} enables models to generalize to new tasks without specific examples but may falter with complex tasks~\citep{sahoo2024systematic,kojima2022large}. \textbf{Few-shot learning}, or \textbf{in-context learning}, involves presenting the model with a few examples to improve its performance on novel tasks~\citep{brown2020language,reynolds2021prompt}. \textbf{Chain-of-Thought} (CoT), introduced by Wei et al.~\citep{wei2022chain}, structures the model's reasoning into intermediate steps, which can be enhanced by combining CoT with few-shot prompts for complex reasoning tasks. 

\textbf{Tree-of-Thoughts} (ToT), proposed by Yao et al.~\cite{yao2024tree} and ~\cite{long2023large}, builds on Chain-of-Thought by employing a systematic exploration of a "tree" of reasoning steps. This method integrates search algorithms, allowing the model to explore different branches of reasoning more strategically, which is particularly useful for solving complex problems.

In the context of \name, we used the Tree-of-Thoughts (ToT) technique to enhance the refinement of inputs extracted from bug reports. By guiding GPT-3.5-turbo through a structured exploration of possible inputs and their relevance to the reported bug, ToT helps in generating more contextually accurate and useful test inputs. This advanced prompt engineering method enables \name to better align LLM behavior with the specific demands of test input generation, leading to more effective and targeted test cases.

==> Sections/Bugreportsandrelevantinputs.tex <==
% \section{Bug reports and relevant input}
% \label{sec:bugreportsandrelevantinputs}
% % This section presents the value of bug reports and introduces the definition of relevant inputs in the context of bug reports.
% This section explores the significance of bug reports in software testing and defines the concept of relevant inputs within the context of these reports, highlighting their critical role in enhancing automated test case generation.

% \subsection{Bug reports}
% \label{subsec:valueofbugreports}
% % Bug reports play a pivotal role in the software development process, serving as crucial documents that outline various software issues, their context, and potential solutions. These reports often contain detailed information about the observed behavior, the conditions leading to the issue, and, notably, specific inputs triggering the reported bugs. Typically, a bug report comprises a comprehensive description of the problem, including steps to reproduce it, the environment in which it occurred, and occasionally, the expected and actual results. Additionally, it may contain snippets of code, stack traces, and user logs, providing developers with an in-depth understanding of the problem.
% Bug reports are integral to the software development lifecycle, serving as essential artifacts that document software issues, their context, and potential resolutions. These reports often provide a wealth of detailed information, including the observed behavior, the specific conditions under which the issue arose, and, crucially, the inputs that triggered the reported bugs. Typically, a bug report includes a thorough description of the problem, outlining the steps required to reproduce it, the environment in which the issue occurred, and sometimes the expected versus actual results. Moreover, bug reports may include supplementary materials such as code snippets, stack traces, and user logs, offering developers a comprehensive perspective on the problem and facilitating a deeper understanding necessary for effective debugging and resolution.


% \subsection{Relevant inputs} 
% \label{subsec:rel-inputs}
% % In this section, we define what constitutes a relevant input in the context of a bug report.
% % %This first step is crucial, as it allows a better understanding of the exploration of bug reports and the next two steps, i.e. the location and the extraction of relevant inputs. But before we identify a relevant input, it is important to define it. \par
% % According to Toffola et al.~\citep{ASE-2017-ToffolaSP} and Shahbaz et al.~\citep{shahbaz2012automated} relevant inputs are those that bypass domain-specific sanity checks. In~\citep{mcminn2012search} and also in~\citep{shahbaz2012automated}, relevant inputs are those which are branch-covering and human-readable, especially for cases where there is no automated oracle. Mariani et al.~\citep{mariani2014link} define relevant inputs as inputs that are both syntactically correct and semantically valid and meaningful. While Bozkurt et al.~\citep{bozkurt2011automatically} describe relevant inputs as realistic. Liu et al.~\citep{liu2017automatic} describe relevant inputs as those appropriate to the context.
% % From these definitions, a relevant input is an input that is realistic, appropriate to the context or domain, that provides good code coverage, and above all, that allows to detect bugs.

% % To define relevant inputs for our tasks, further investigations of both bug reports and human-written test cases are essential.
% % %\jk{In the next paragraph, you focus on bug reports, so I guess, we should say: "further investigations of both bug reports and  human-written test cases are essential."}
% % %Given a bug report, to make it easier to identify a relevant input, this led us to ask a first research question regarding the definition of a relevant input. \par
% % %\textbf{RQ 1: What constitutes a relevant input in the context of a bug report?} \par \lp{remove RQ and rephrase}
% % The manual exploration of hundreds of bug reports reveals that the information contained therein differs depending on the user raising an issue. While some bug reports mention input values, API (or method) used, expected values, and actual values, others additionally mention wrapper code and some code portion to reproduce. Therefore, a manual analysis of the bug reports and test cases written by humans to pass the patched version revealed that some input values appearing in some bug reports were also present in the test cases. As an example, we can see in Figure~\ref{fig:identic-input} that some of the inputs mentioned in the bug report appear in the test case.

% % According to various studies ~\citep{ASE-2017-ToffolaSP,shahbaz2012automated,mcminn2012search,mariani2014link,bozkurt2011automatically,liu2017automatic}, a relevant input bypasses domain-specific sanity checks, offers branch coverage, is both syntactically and semantically valid, realistic, appropriate to the context, and facilitates effective bug detection.

% % Further investigations of both bug reports and human-written test cases are crucial in defining relevant inputs for our tasks. Manual exploration of numerous bug reports indicates variations in the included information, with some reports detailing input values, APIs, expected and actual values, and even featuring wrapper and reproducible code segments. Manual analysis of these reports and corresponding test cases that pass the patched version revealed overlapping input values between the bug reports and the test cases. Figure~\ref{fig:identic-input} illustrates instances where inputs mentioned in the bug reports are also present in the test cases. In some cases, the test case input shares a pattern with, but is not identical to, the input from the bug report. Figure~\ref{fig:same-patern} exemplifies this scenario.
% Relevant inputs are defined by several key characteristics, as highlighted in various studies~\citep{ASE-2017-ToffolaSP,shahbaz2012automated,mcminn2012search,mariani2014link,bozkurt2011automatically,liu2017automatic}. These inputs bypass domain-specific sanity checks, contribute to branch coverage, and are both syntactically and semantically valid. They are realistic, context-appropriate, and crucially, they facilitate effective bug detection.

% A deeper understanding of what constitutes relevant inputs in the context of bug reports requires thorough examination of both bug reports and human-written test cases. Through manual analysis of numerous bug reports, we observed significant variations in the information they contain. Some reports include detailed input values, APIs, expected and actual results, and even complete code segments for reproducing the issue. By comparing these reports with the corresponding human-written test cases that successfully pass after a patch, we discovered a notable overlap in the input values provided. Figure~\ref{fig:identic-input} illustrates instances where inputs from bug reports are directly reflected in the test cases. Additionally, in some cases, the input values in the test cases share a similar pattern with those in the bug reports, though they may not be identical, as shown in Figure~\ref{fig:same-patern}.


% % \begin{figure}
% %     \includegraphics[width=8.5cm, height=8cm]{Images/identic-input}
% %     \caption{Input value mentioned in the bug report for issue 3447 in the FasterXML jackson-databind library is in a test case written by a developer after fixing the bug.}
% %     \label{fig:identic-input}
% % \end{figure}


% % \begin{figure}
% % \centering
% %     \subfloat[Bug report.]{
% %         \includegraphics[width=.9\linewidth]{Images/identic-input-A1}
% %     }\quad
% %     \subfloat[Developer-written test case]{%
% %         \includegraphics[width=.9\linewidth]{Images/identic-input-A2}
% %     }
% %   \caption{Input value mentioned in the bug report for issue 3447 in the FasterXML jackson-databind library appears in a test case written by a developer after fixing the bug.}
% %   \label{fig:identic-input}
% % \end{figure}


% \begin{figure*}[!ht]
%     \centering
%     \flushleft
%     \subfigure[Bug report]{
%     \includegraphics[scale=0.65]{Images/identic-input-A1}%
%     }
%     \subfigure[Developer-written test case]{
%     \includegraphics[scale=0.65]{Images/identic-input-A2}%
%     }
%     \caption{Input value mentioned in the bug report for issue 3447 in the FasterXML jackson-databind library appears in a test case written by a developer after fixing the bug}
%     \label{fig:identic-input}
%     \vspace{3mm}
% \end{figure*}


% % In some cases, the input in the test case is not identical to that provided by the user in the bug report but has the same pattern or format. Figure~\ref{fig:same-patern} shows an example of a case where the input in the bug report and the one used in the test case have the same pattern but are not identical.


% \begin{comment}
% \begin{figure}
%     \includegraphics [width=8.5cm, height=8cm]{Images/same-patern}
%     \caption{Pattern of the input value mentioned in the bug report for issue 1205 in the Apache Commons Lang library library is in a test case written by a developer after fixing the bug.}
%     \label{fig:same-patern}
% \end{figure}
% \end{comment}

% % \begin{figure}
% % \centering
% %     \subfloat[Bug report.]{
% %         \includegraphics[width=.9\linewidth]{Images/same-patern-A1}
% %     }\quad
% %     \subfloat[Developer-written test case.]{%
% %         \includegraphics[width=.9\linewidth]{Images/same-patern-A2}
% %     }
% %   \caption{Pattern of the input value mentioned in the bug report for issue 1205 in the Apache Commons Lang library appears in a test case written by a developer after fixing the bug.}
% %   \label{fig:same-patern}
% % \end{figure}

% \begin{figure*}[!ht]
%     \centering
%     \flushleft
%     \subfigure[Bug report]{
%     \includegraphics[scale=0.65]{Images/same-patern-A1}%
%     }
%     \subfigure[Developer-written test case]{
%     \includegraphics[scale=0.65]{Images/same-patern-A2}%
%     }
%     \caption{Pattern of the input value mentioned in the bug report for issue 1205 in the Apache Commons Lang library appears in a test case written by a developer after fixing the bug}
%     \label{fig:same-patern}
%     \vspace{3mm}
% \end{figure*}


% % From these two observations, we can say that, from the perspective of a bug report, {\em an input is relevant if we use it or its pattern to pass a human-written test after the patching}. 
% % Hence, it becomes challenging to verify whether an input extracted from a bug report, distinct from the one included in a human-written test case, holds significant relevance. It's important to note that not all inputs mentioned in a bug report are relevant, and conversely, not all inputs that differ from those in the test case are irrelevant.
% % Therefore, for the purpose of evaluating the rate of relevant inputs in bug reports and to assess BRMiner's capability in extracting such inputs we will only consider this definition in its strictest form, i.e., when the inputs are identical.

% % From these observations, we define bug report inputs as relevant when they enable a human-written test to pass post-patching. However, verifying the relevance of bug report inputs distinct from those in test cases presents a challenge. Notably, not all inputs in bug reports are relevant, and conversely, differing inputs in test cases are not necessarily irrelevant. To evaluate the rate of relevant inputs in bug reports and BRMiner's extraction capability, we strictly consider only identical inputs.
% Based on these observations, we define inputs from bug reports as relevant when they contribute to the success of a human-written test case after the software has been patched. However, determining the relevance of bug report inputs that differ from those used in test cases presents a unique challenge. It's important to note that not all inputs found in bug reports are necessarily relevant, and conversely, test case inputs that differ from those in the bug report are not automatically irrelevant. To accurately assess the rate of relevant inputs in bug reports and the effectiveness of BRMiner's extraction process, our evaluation focuses specifically on inputs that are identical between the bug reports and the corresponding test cases.

% % \subsection{Relevant input location}
% % \label{subsec:rel-input-location}
% % From the bug report exploration and the identification of relevant inputs, we know that inputs can be found either in source code as in Figure \ref{fig:identic-input} or directly in natural language text. Therefore, given a bug report that we parsed, we separate natural language text from source code. To this end, \name used Infozilla: running Infozilla on a bug report returns natural language text with all structural elements removed and a machine-analyzable representation of all structural elements.

% \begin{comment}
% \begin{figure}
%     \includegraphics [width=8.5cm, height=8cm]{Images/input-in-natural-langage}
%     \caption{Inputs are part of natural language text.}
%     \label{fig:input-in-natural-langage}
% \end{figure}
% \end{comment}


% %Fig4

% % \begin{figure}[h!]
% % \centering
% %     \subfloat[Bug report.]{
% %         \includegraphics[width=.9\linewidth]{Images/input-in-natural-langage-A1.pdf}
% %     }\quad
% %     \subfloat[Developer-written test case.]{%
% %         \includegraphics[width=.9\linewidth]{Images/input-in-natural-langage-A2.pdf}
% %     }
% %   \caption{Input values mentioned in the bug report for issue 1462 in the Apache Commons Lang library appear in a test case written by a developer after fixing the bug are part of natural language text.}
% %   \label{fig:input-in-natural-langage}
% % \end{figure}

==> Sections/abstract.tex <==
% \begin{abstract}
% The quality of a software is highly dependent on the quality of the tests it is submitted to. Writing tests for bug detection is thus essential. However, it is time-consuming when done manually. Automating test cases generation has therefore been an exciting research area in the software engineering community. Most approaches have been focused on generating unit tests. Unfortunately, current efforts often do not lead to the generation of relevant inputs, which limits the efficiency of automatically generated tests. Towards improving the relevance of test inputs, we present \name, a technique for exploring bug reports to identify input values that can be fed to automatic test generation tools. In this work, we investigate the performance of using  inputs extracted from bug reports with \name to generate test cases with Evosuite. The evaluation is performed on the Defects4J benchmark. For Defects4J projects, our study has shown that \name successfully extracted 68.68\% of relevant inputs when using regular expression in its approach versus 50.21\% relevant inputs without regular expression. Further, our study has shown the potential to improve the Line and Instruction Coverage across all projects. Overall, we successfully collected relevant inputs that led to the detection of 45 bugs that were previously undetected by the baseline.
% \end{abstract}
\begin{abstract} 
The quality of software is closely tied to the effectiveness of the tests it undergoes. Manual test writing, though crucial for bug detection, is time-consuming, which has driven significant research into automated test case generation. However, current methods often struggle to generate relevant inputs, limiting the effectiveness of the tests produced. To address this, we introduce \name, a novel approach that leverages Large Language Models (LLMs) in combination with traditional techniques to extract relevant inputs from bug reports, thereby enhancing automated test generation tools. In this study, we evaluate \name using the Defects4J benchmark and test generation tools such as EvoSuite and Randoop. Our results demonstrate that \name achieves a Relevant Input Rate (RIR) of 60.03\% and a Relevant Input Extraction Accuracy Rate (RIEAR) of 31.71\%, significantly outperforming methods that rely on LLMs alone. The integration of BRMiner's input enhances EvoSuite ability to generate more effective test, leading to increased code coverage, with gains observed in branch, instruction, method, and line coverage across multiple projects. Furthermore, \name facilitated the detection of 58 unique bugs, including those that were missed by traditional baseline approaches. Overall, \name's combination of LLM filtering with traditional input extraction techniques significantly improves the relevance and effectiveness of automated test generation, advancing the detection of bugs and enhancing code coverage, thereby contributing to higher-quality software development. 
\end{abstract}



==> Sections/bibliography.tex <==
\begin{thebibliography}{00}

\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.


\end{thebibliography}

==> Sections/conclusion.tex <==
% \section{Conclusion}
% \label{sec:conclusion}

% In this paper, we demonstrate the feasibility of extracting relevant inputs from bug reports for enriching automatic test case generation. We first introduce \name, a practical approach that extracts relevant inputs from bug reports to help automatic testing approaches in generating better test cases.

% Our experiments systematically compared the performance of a search-based tool with a dynamic symbolic execution module (EvosuiteDSE) without and with our relevant inputs for the task of relevant test cases generation for bug detection and code coverage. Our study shows that \name successfully extracts relevant inputs from Defects4J bug reports and most of those input values were used in the developer-written test cases. 

% Additional experiments have shown that \name successfully extracted 68.68\% of relevant inputs when using regular expression leading to the detection of 45 bugs that were previously not detected by the baseline. 
% While our study shows promising results regarding code coverage and bug detection, our approach only builds the first milestone in leveraging bug reports for relevant test inputs enabling the practical adoption of test generation tools for real-world software projects. 


% %we propose an approach to automatically generate test cases by using relevant inputs extracted from bug reports.

% %effective approach called \name, that extracts relevant inputs from bug reports in order to automatically generate test cases with an automated test generator EvoSuite. Given a bug report, \name is able to 

\section{Conclusion}
\label{sec:conclusion}
In this paper, we introduced \name, a novel approach designed to enhance automatic test case generation by extracting relevant inputs directly from bug reports. Our approach systematically identifies and integrates these inputs into test generation tools such as EvoSuite and Randoop, with the goal of improving both bug detection and code coverage. Through a comprehensive set of experiments on the Defects4J dataset, we evaluated the effectiveness of \name across multiple projects and configurations. Our results demonstrate that \name significantly improves the quality of automatically generated test cases. Specifically, \name successfully extracted relevant inputs that led to the detection of additional bugs not identified by the baseline approaches. For instance, our approach achieved a bug detection increase of up to 18 bugs in certain configurations, and a notable enhancement in code coverage metrics across various dimensions, including branch, instruction, method, and line coverage.

While \name shows significant promise, particularly in improving bug detection and code coverage, it also highlights the need for further exploration in real-world scenarios. Future work will involve integrating \name into continuous integration pipelines and applying it to live systems where bug reports are actively being resolved. This will enable us to evaluate \name’s effectiveness in real-time software development environments and further refine its capabilities. Moreover, the potential of \name to manage discrepancies across different software versions, as well as its adaptability to projects with varying levels of bug report history, will be key areas for future research. These enhancements will ensure that \name remains a robust tool for diverse software development contexts, including smaller or less mature projects where bug reports are scarce.

In conclusion, \name represents a significant step forward in leveraging bug reports to enhance the capabilities of automated test generation tools. By providing a practical method for extracting and utilizing relevant inputs, \name paves the way for more effective and reliable software testing, ultimately contributing to the production of higher-quality software.

==> Sections/discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}
% This section first of all discusses the threats to validity of this study, then the limitations and the future work and at the end discusses the related work concerning this study.

% \subsection{Threats to Validity}
% Our research, like any study, is subject to various validity threats that need consideration. One such threat is the generalizability of our findings. Although we experimented with a diverse range of projects from Defects4J, the results may not directly apply to all software systems. The effectiveness of incorporating relevant inputs can be influenced by specific characteristics of bug reports, test cases, and programming languages. To address this, we implemented rigorous experimental methodologies and conducted multiple iterations.

% %An internal validity threat is that we did not manually investigate all tests that detected faults to validate bug detection accuracy. However, we took measures to mitigate this by conducting sanity checks and manual inspections on a significant number of test suites. These steps ensured the reliability and validity of our bug detection results.

% %A potential threat to construct validity is related to the use of the Defects4J dataset, which does not differentiate between types or severity of faults. The dataset represents bugs using minimized diffs instead of actual code changes, which may underestimate the effectiveness of automated test generation tools for regression testing. The study could also overestimate effectiveness if some detected faults are unlikely to be introduced in the future.

% %Additionally, our study relied on code versions committed to a public repository and did not consider regressions detected by developers before committing changes. This may underestimate  the effectiveness of EvoSuite if uncommitted changes are easier to detect. However, this threat is partially mitigated as the dataset includes bugs from various stages of project history.

% Additionally, considering only identical inputs and excluding inputs with the same pattern when we compare the inputs extracted by BRMiner and the inputs in Defects4J tests is a limitation of our approach. This omission may result in overlooking some relevant inputs mentioned in bug reports. The tokenizer used in the first research question may not have captured all the literals in the bug reports, affecting the inclusion of certain inputs. Conventional tokenizers may not be adequate in capturing all relevant inputs, impacting the results for research questions 1 and 2.

% Moreover, the use of the Javalang parser may have limited the extraction of literals from test cases and bug reports, affecting the rate of relevant input extraction. These limitations should be considered when interpreting the results.

% \subsection{Limitations and Future Work}
% Our study has limitations that should be acknowledged. Firstly, we only considered identical inputs and did not account for inputs with similar patterns, potentially underestimating the presence of relevant inputs in bug reports. Future research could explore advanced techniques for capturing inputs with similar patterns. Secondly, due to resource constraints, we had a limited time budget and conducted a limited number of iterations, which may have affected the completeness of our results. Increasing the time budget and iterations could provide a more comprehensive analysis.

% The tokenizer used in our experiments may not have achieved perfect tokenization, leading to the underestimation of relevant inputs in both test cases and bug reports. Using advanced tokenization techniques or alternative approaches could address this limitation. 
% %The Javalang parser used in some cases may have missed parsing all literals in test cases, impacting the completeness of our results. Future studies could consider alternative parsing techniques or employ multiple parsers for better extraction of relevant inputs.

% Additionally, our evaluation focused primarily on bug detection and code coverage, overlooking other aspects like fault localization or test suite efficiency. Future studies could incorporate additional evaluation metrics for a more comprehensive assessment. To enhance generalizability, conducting experiments on a wider range of software systems and programming languages would be valuable. This would validate the effectiveness of incorporating relevant inputs across diverse contexts and explore language-specific challenges and opportunities.

% Lastly, exploring the integration of relevant inputs from bug reports into other test generation approaches beyond EvoSuite could provide broader insights into their applicability and benefits.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
\label{sec:discussion}
This section discusses the potential threats to validity, limitations of our study, and suggestions for future work, along with a comparison to related work.

\subsection{Threats to Validity}
Our study, while comprehensive, is subject to several validity threats that need to be addressed to strengthen the reliability of our findings. One of the primary threats is related to the generalizability of our results. Although we utilized a diverse set of projects from Defects4J, the applicability of our findings to other software systems, particularly those that differ in size, complexity, or domain, may be limited. The effectiveness of BRMiner in extracting relevant inputs can be highly dependent on the nature of the bug reports, the structure of test cases, and the programming languages used. To mitigate this threat, we adopted rigorous experimental methodologies and conducted multiple iterations across varied projects, but the limitation remains that our conclusions may not be universally applicable.

Another concern arises from the potential discrepancies between different software versions, which could impact the relevance of the extracted inputs. Bug reports may pertain to older versions, while significant changes could have been implemented in newer versions, potentially altering the context in which the bug manifests. BRMiner is not specifically designed to address these discrepancies across software versions, but this limitation is somewhat mitigated by the versatility of automated test generators, which use a variety of inputs to cover diverse execution paths. Although version differences may influence the relevance of some inputs, the broad range of generated test cases typically ensures robust coverage. Future work could enhance BRMiner by incorporating an input prioritization system that adapts to version-specific differences, thus further strengthening its effectiveness.

The oracle problem in regression testing presents another potential threat to the validity of our study. Our approach relies on fixed versions to generate test oracles, inspired by previous studies. However, in real-world scenarios, fixed versions are not always available, which raises questions about the practical applicability of our method. While our approach is justified in controlled experimental settings, its effectiveness in practical, "in-the-wild" scenarios may be limited. Future research could focus on exploring automated test oracle generation or assessing BRMiner’s effectiveness when used with open bug reports directly, without relying on fixed versions.

Another potential limitation is related to input scarcity in less popular projects. The effectiveness of BRMiner assumes the availability of a substantial number of bug reports, which may not be the case for newer or less popular software projects. This assumption could limit the generalizability of our approach. However, BRMiner mitigates this by providing a valuable database of pre-extracted inputs, which can bootstrap the testing process even in the absence of extensive bug report histories. This feature is particularly beneficial for smaller projects or those using common Java libraries, enabling comprehensive test case generation regardless of the project's size or age.

To enhance the real-world applicability of BRMiner, future work could explore its use in live systems where bug reports are actively being resolved. This could involve integrating BRMiner into a continuous integration pipeline, allowing it to automatically extract inputs from incoming bug reports and generate targeted test cases to catch bugs before they reach production. Such integration would demonstrate the practical utility of BRMiner in ongoing software development processes, thereby extending its relevance beyond controlled experiments.

A potential threat in our approach relates to data leakage when utilizing Large Language Models (LLMs) like the one used in BRMiner. Data leakage occurs when information from the training data inadvertently influences the model’s outputs in a way that would not be possible in a real-world scenario, potentially compromising the validity of the results. However, in our case, the risk of data leakage is mitigated by the fact that we only used the content of bug reports without including any specific project names, source code, or other identifiable details. The inputs extracted from these bug reports are abstract and generic, reducing the likelihood that they carry sensitive or identifiable information. Additionally, these inputs were further processed and filtered to ensure that no confidential data was exposed inadvertently. While this approach minimizes the risk of data leakage, it remains a consideration that future studies should address, particularly if more direct interaction with project-specific data is involved.



\subsection{Limitations and Future Work}

Our study has several limitations that need to be acknowledged. One of the key limitations is the focus on a limited set of coverage metrics, primarily bug detection and code coverage. While these metrics are crucial, they do not provide a complete picture of test suite quality. Future studies could incorporate additional metrics such as fault localization, test suite efficiency, and maintainability to provide a more comprehensive assessment of BRMiner's impact.

Another limitation lies in the tokenization and input extraction process used in our experiments. The tokenizer may not have captured all relevant inputs from bug reports and test cases, potentially leading to an underestimation of BRMiner's effectiveness. Conventional tokenizers may miss certain inputs, especially those with complex patterns. While BRMiner is designed to handle complex scenarios where literals may be involved in concatenations or method calls, ensuring that the entire concatenated string or argument values are extracted and used in test generation, there is room for improvement. Future research could explore advanced tokenization techniques or machine learning-based approaches to enhance input extraction accuracy.

Our study was also constrained by the time budget and the number of iterations conducted. Due to resource limitations, we imposed a time budget of three minutes per iteration and conducted a limited number of iterations. This constraint may have impacted the completeness of our results. Increasing the time budget and the number of iterations in future experiments could yield more comprehensive data and potentially reveal additional insights into BRMiner's effectiveness.

The applicability of our findings across diverse software contexts is another area of concern. Our evaluation was limited to projects in the Defects4J dataset, which, while diverse, may not represent all possible software contexts. Future research should expand the evaluation to include a broader range of software systems, programming languages, and domains. This would help validate the generalizability of BRMiner across different types of software and explore any language-specific challenges that may arise.

Additionally, while our study focused on integrating BRMiner with EvoSuite, there is value in exploring how BRMiner can be integrated with other test generation tools and techniques. Broadening the scope of integration could enhance the applicability of our approach and provide insights into its benefits across different test generation paradigms.

Lastly, addressing the challenge of input relevance across different software versions could involve developing an input prioritization system that adapts to changes in software versions. This would help maintain the relevance of test inputs and ensure that BRMiner remains effective even as software evolves. Such advancements could further strengthen BRMiner's utility in dynamic and evolving software environments.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Related Work}
% \label{subsec:related-work}
% % % In an empirical study~\citep{shamshiri2015automatically}, the authors focused on evaluating the effectiveness of automatic test case generators for bug detection. They examined three tools, EvoSuite, Randoop, and AgitarOne, using the Defects4J dataset in a regression scenario. However, the study did not incorporate specific inputs for testing and evaluated the tools in their default mode of operation.
% In a study by \citet{shamshiri2015automatically}, the authors evaluated the efficacy of automatic test case generators for bug detection. Their examination of three tools, EvoSuite, Randoop, and AgitarOne, utilized the Defects4J dataset in a regression scenario. However, the study did not integrate specific inputs for testing and assessed the tools in their default operational mode. Due to the utilization of older versions of EvoSuite and Defects4J in this research, it is not feasible to directly compare our empirical findings with their study. \citet{almasi2017industrial} conducted subsequent experiments with EvoSuite for bug detection, their assessments were performed on a proprietary financial application. As a result, access to their source code and relevant bug reports remains unavailable.

% In another study~\citep{ASE-2017-ToffolaSP}, the authors addressed the limitations of current test generation techniques in providing relevant input values for effective software testing. They introduced TestMiner, a technique that extracts literals from existing tests to identify suitable values for specific domains. By mining this information, TestMiner aims to improve test generation by providing more relevant input values and enhancing the overall quality of software testing. Unlike our approach, their methodology involves extracting literals from a multitude of tests and employing information retrieval techniques to identify domain-specific values, enhancing efficacy for previously challenging classes. Although Randoop was employed instead of EvoSuite for their implementation, the classes in the projects they used are currently largely inaccessible and outdated. Additionally, we lack sufficient information on bug reports from these projects. Given these reasons, it is challenging for us to make a direct comparison between their approach and ours.

% \citet{rabin2021configuring} presented the K-Config approach, which improves the configuration of the Csmith test generator for compiler testing using code snippets from bug reports. By analyzing bug reports, the approach generates test programs that effectively uncover bugs in the compiler implementation. The results demonstrate that incorporating bug report information enhances the bug detection capabilities of K-Config. This study leverages code snippets within GCC bug reports, emphasizing language features that might be inadequately implemented. The aim is to direct test generators towards achieving higher coverage and triggering more miscompilation failures compared to existing techniques for GCC. However, the focus of their study differs from ours, as it primarily concerns test generation for compilers using code snippets. While Gcc and Csmith serve as test generators for compilers, EvoSuite specializes in generating JUnit 4 tests. Hence, these distinctions present challenges in making a direct comparison between their approach and ours.

% \citet{zhong2022enriching} explored enhancing compiler tests by incorporating real programs extracted from bug reports. They introduced the LeRe tool, which extracts test programs from bug reports and utilizes differential testing to identify compiler bugs. By leveraging bug report information, the approach enriches the pool of test programs and improves the quality of compiler testing. In this study, the authors introduce compiler bug reports as a novel source for compiler testing, introducing the LeRe tool that extracts test programs from these reports. They utilize differential testing to identify compiler bugs using these extracted programs and provide an analysis of invalid bug reports. Similar to the study by \citet{rabin2021configuring} , their research focuses on test generators for compilers, but with a distinct approach involving program extracts. These disparities make a direct comparison with our study challenging.

% Addressing the challenge of identifying and understanding performance bugs in software systems, \citet{han2018perflearner} proposed PerfLearner. This approach utilizes bug reports to extract execution commands and input parameters associated with performance bugs. The findings highlight the effectiveness of PerfLearner in enhancing the detection and understanding of performance bugs, ultimately improving the quality of software testing. PerfLearner, an automated approach aimed at extracting execution commands and input parameters from performance bug report descriptions. These extracted elements are then used to construct test frameworks guiding the generation of actual performance test cases. While the study also utilizes bug reports, its focus differs from ours, as it does not involve generating tests for bug detection or guiding the generation of test cases for bug detection. Consequently, a direct comparison between their approach and ours proves challenging.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Work}
\label{subsec:related-work}

\subsubsection{Automated Test Generation}
In this section, we will discuss general approaches to automated test generation, focusing on the tools and methodologies that are most relevant to our study.

\vspace{0.2cm}\noindent\textbf{General Approaches to Automated Test Generation.}
\citet{shamshiri2015automatically} evaluated the effectiveness of automatic test case generators like EvoSuite, Randoop, and AgitarOne for bug detection using the Defects4J dataset in a regression scenario. This study forms a foundation for understanding the efficacy of these tools in generating test cases but did not integrate specific inputs for testing. The study's use of older versions of EvoSuite and Defects4J limits direct comparisons with our work. \citet{almasi2017industrial} conducted experiments with EvoSuite for bug detection on a proprietary financial application, further exploring the tool's capabilities. However, the lack of access to their source code and bug reports prevents direct comparison with our approach.

\vspace{0.2cm}\noindent\textbf{Enhancing Test Generation with Domain-Specific Knowledge.}
TestMiner by ~\citet{ASE-2017-ToffolaSP} proposed enhancing test generation by mining literals from existing tests to identify domain-specific values, particularly for challenging classes. Although this method differs from ours, which extracts literals from bug reports rather than existing tests, it provides valuable insights into improving test generation by incorporating relevant inputs.

\subsubsection{Bug Report-Based Test Generation}
This section will focus on methodologies that utilize bug reports to enhance the test generation process.

\vspace{0.2cm}\noindent\textbf{Compiler Testing with Bug Reports.}
K-Config by \citet{rabin2021configuring} utilized code snippets from GCC bug reports to improve the configuration of the Csmith test generator for compiler testing. By analyzing bug reports, K-Config generated test programs that effectively uncovered compiler bugs. While this study focused on compiler testing rather than general software testing, it highlights the value of integrating bug report information into test generation. LeRe by \citet{zhong2022enriching} took a similar approach by extracting real programs from bug reports to enhance compiler testing. The study introduced differential testing techniques, which could enrich test programs and improve test quality, especially for compilers. Although focused on compilers, this research emphasizes the importance of leveraging bug reports for test generation, aligning with our approach but in a different domain.

\vspace{0.2cm}\noindent\textbf{Performance Testing from Bug Reports.}
PerfLearner by \citet{han2018perflearner} targeted performance bugs by extracting execution commands and input parameters from bug reports. This method improved the detection and understanding of performance bugs by using the extracted information to guide the generation of performance test cases. Although it does not directly involve generating tests for bug detection in the same way our study does, it demonstrates the broader applicability of bug report-based approaches in various testing contexts.

\subsubsection{LLM-Based Inputs for Test Generation}
\vspace{0.2cm}\noindent\textbf{LLMs for Input Generation.}
\citet{liu2024testing} explored the potential of LLMs in generating unusual text inputs that can be used to detect crashes in mobile apps. Their study demonstrates how LLMs can be employed to create diverse and complex inputs, which aligns with our use of LLMs for generating inputs in BRMiner. The insights from this work could inform future enhancements of BRMiner, particularly in generating inputs that cover a broader range of edge cases.

\vspace{0.2cm}\noindent\textbf{White-Box Testing Empowered by LLMs.}
\citet{yang2023white} examine the use of LLMs in white-box compiler fuzzing. Their study shows how LLMs can assist in creating test inputs that expose deeper and more intricate bugs in compilers. This approach shares similarities with our work, where LLMs are used to filter and enhance the relevance of inputs extracted from bug reports for test generation, though applied in a different domain.

\vspace{0.2cm}\noindent\textbf{LLMs for Variable Discovery in Metamorphic Testing.}
\citet{tsigkanos2023variable} focuse on the use of LLMs to discover variables that can be used in metamorphic testing of scientific software. This research highlights the ability of LLMs to understand and manipulate domain-specific knowledge, which can be parallelized with our work's use of LLMs to identify and utilize relevant inputs from bug reports for more effective test generation.

==> Sections/intro.tex <==
% \section{Introduction}
% \label{sec:intro}
% Software testing is as old as the software industry. It requires test suites, which are often incomplete since developer-provided test cases are  typically non-exhaustive as they are not systematically produced in most projects for the whole code~\citep{kochhar2015understanding,kochhar2013empirical,kochhar2013adoption}. Thus, automated software test generation has early attracted significant attention in the research and practice communities due to its numerous potential benefits, including the reduction of manual effort and the increase of test coverage~\citep{ASE-2017-ToffolaSP}. To that end, a large body of the literature has proposed several techniques for the automatic generation of test inputs, including Search-Based Software Testing (SBST)~\citep{5342440}, feedback-directed random test generation~\citep{pacheco2007feedback,artzi2011framework,pradel2012fully}, Dynamic Symbolic Execution (DSE)~\citep{king1976symbolic,godefroid2005dart,xie2005symstra,majumdar2007directed,cadar2013symbolic}, and concolic execution~\citep{sen2005cute,cadar2008exe,sen2006cute}. While the tools based on those techniques have shown effectiveness, they often face limitations that hinder their adoption in real-world projects.

% %According to prior work~\citep{shamshiri2015automatically}, only 19.9\% of bugs from the Defects4J~\citep{just2014defects4j} benchmark could be detected by test suites generated by state-of-the-art test generators. 
% For example, while prior research has underscored the efficacy of Search-Based Software Testing (SBST) techniques in attaining notable code coverage~\citep{panichella2015reformulating, panichella2017automated}, \citet{perera2020defect} argue that high code coverage alone does not guarantee the optimal detection of bugs.
% In line with this, \citet{shamshiri2015automatically} then \citet{almasi2017industrial} assessed the performance of EvoSuite~\citep{fraser2011evosuite}, a leading SBST tool against alternative test generation methods and tools like Randoop~\citep{pacheco2007feedback}, focusing on open-source and proprietary software projects, respectively. Their findings suggest a superior performance by EvoSuite over its counterparts, but also demonstrate that it falls short in effectively detecting genuine bugs. Notably, EvoSuite could identify only about 23\% of bugs from the Defects4J dataset~\citep{just2014defects4j}. It's worth noting that both in both studies, the testing criterion is set at 100\% branch coverage.

% One of the main reasons behind this limitation is that these generators primarily rely on either randomly-generated inputs or inputs from a fixed pool, which may not match the project specifications~\citep{ASE-2017-ToffolaSP}. Additionally, test generators tend to focus on the source code and its dynamic execution, generating less natural and readable values~\citep{shelke2014generation}.

% To address these challenges, researchers have proposed various approaches: Some have utilized test corpora~\citep{ASE-2017-ToffolaSP}, while others have explored web search queries~\citep{shelke2014generation,mcminn2012search,shahbaz2012automated}, user session data~\citep{elbaum2003improving}, web services~\citep{bozkurt2011automatically}, or the web of data~\citep{mariani2014link} to generate realistic test inputs. Regarding mobile application testing, \citet{liu2017automatic} leveraged the Google news corpus. In~\citep{milani2014leveraging}, researchers leveraged existing tests to automate test generation for web applications. Nevertheless, despite the existence of these approaches, the potential of bug reports as a valuable source of relevant inputs, including strings for test data generation, remains largely untapped.


% % \textbf{Search-based Test Suite Generation and Dynamic Symbolic Execution}
% % Dynamic Symbolic Execution (DSE) is among the widely adopted techniques for automated test case generation~\citep{valle2022mutation}. This method simultaneously explores multiple paths of the source code using symbolic values in place of concrete ones . Employing a symbolic execution engine enables efficient control over the paths traversed within the source code~\citep{baldoni2018survey}. Its applications include the automated generation of unit tests and the identification of actual defects or memory overflows~\citep{cadar2013symbolic}.

% % While search-based testing excels at formulating unit test suites for object-oriented code, it occasionally falters in producing specific values for intricate code parts. In contrast, Dynamic Symbolic Execution (DSE) shines in creating these precise values but finds complexity when faced with data types necessitating a chain of calls. Galeotti et al.~\citep{galeotti2013improving} paved the way for a combined technique, leveraging the advantages of both methods. They refined the Genetic Algorithm (GA) within EVOSUITE to smoothly incorporate DSE and, guided by search feedback, determined the optimal moments to employ DSE. This modification led to a jump in average branch coverage. Furthermore, when compared to standalone DSE tools, EVOSUITE combined with DSE proved superior in achieving coverage. Empirical analyses underscored the practical advantages of integrating SBST and DSE, with negligible downsides. In subsequent research, Galeotti et al.~\citep{galeotti2014extending} highlighted that this fusion not only augments coverage and effectiveness but also upholds SBST's flexibility in tailoring test suites for various metrics and non-functional factors. Crucially, this approach ensures that all test cases correspond to legitimate object conditions. As a testament to its capabilities, EvosuiteDSE made a notable debut at the ninth unit testing competition during SBST 2021, registering a commendable score of 47.14.

% % \tb{I removed "novel" as qualifier. Please propagate. We are not selling the approach, but the results...}
% \textbf{This paper.} Bug reports offer a diverse range of example inputs which remain largely untapped in the extraction of inputs for automatic test case generation. Leveraging bug reports for this purpose offers two significant advantages. Firstly, they provide a wealth of valid inputs for various string types, enhancing test coverage and bug detection. Secondly, bug reports typically contain human-readable inputs, which prove invaluable when manual confirmation is necessary due to the absence of an automated oracle.


% In this study, we propose a simple, and yet effective, approach for automatically extracting real test inputs from bug reports, aimed at addressing the problem of automatic test case generation containing relevant test inputs. Our approach involves exploring bug reports to identify and extract relevant inputs found in bug reports. We developed a tool called \name that enables us to automatically extract these relevant inputs, both qualitatively and quantitatively.
% To generate test cases incorporating these inputs, we modified the source code of EvoSuite~\citep{fraser2011evosuite}, a widely known Search-based test suite generator tool used for automatic test case generation. To evaluate our generated test cases we use the Defects4J benchmark~\citep{just2014defects4j}.

% The main contributions of this paper are as follows:
% \begin{enumerate}
% \item We present \name, an automatic test input extraction approach. This approach offers several advantages, such as the ability to efficiently extract realistic test input for testing projects with semantic information and the improvement of the efficiency of automatic test case generation for inputs that cannot be effectively generated randomly.
% %\item We conduct an empirical study to demonstrate the effectiveness of our approach, showing that it is possible to find valid and well-formed inputs from bug reports and they can improve bug detection and test coverage of a program's source code.
% \item We showcase findings from practical case studies conducted on Defects4J projects. These were designed to assess the efficacy of our methodology in generating test cases based on bug reports, in contrast to the baseline approach of EvoSuite which operates without external inputs.
% \item We emphasize the significance of integrating a feature in EvoSuite that allows for external inputs, especially from bug reports. These inputs offer crucial context, bolstering EvoSuite's performance in tandem with Dynamic Symbolic Execution (DSE).
% %\item We have made the implementation of our approach and our empirical study, along with all relevant data for the experiments, publicly available in an anonymous repository to facilitate further research in this area. The repository can be accessed at the following link: 
% \item We demonstrate the effectiveness of our approach by showcasing the finding of valid, well-formed inputs from bug reports, resulting in improved bug detection and enhanced test coverage for a program's source code. To foster further research in this area, we have publicly shared the implementation of our approach and all relevant experimental data in an anonymous repository. The repository is accessible via the following link:
% \begin{center}
%     \url{https://anonymous.4open.science/r/\name-C853}
% %\ah{This is still not addressed? Anonymous link or saying we will provide it later?}
% \end{center}
% \end{enumerate}

% %\jk{Can be removed if we need space} 
% The rest of this paper is organized as follows. Section~\ref{sec:\name} presents our approach for relevant input extraction from bug reports. Section~\ref{sec:setup} provides an overview of our experimental setup, including implementation details, evaluation of technical challenges, and presentation of results (Section~\ref{sec:results}). Section~\ref{sec:discussion} discusses existing research on test input extraction and generation in the field of automatic test generation, along with the limitations of our approach and future research directions. Finally, Section~\ref{sec:conclusion} summarizes the paper, draws conclusions, and mentions future work.
\section{Introduction}
\label{sec:intro}
Software testing is as old as the software industry. It requires test suites, which are often incomplete since developer-provided test cases are typically non-exhaustive as they are not systematically produced in most projects for the whole code~\citep{kochhar2015understanding,kochhar2013empirical,kochhar2013adoption}. Thus, automated software test generation has early attracted significant attention in the research and practice communities due to its numerous potential benefits, including the reduction of manual effort and the increase of test coverage~\citep{ASE-2017-ToffolaSP}. To that end, a large body of literature has proposed several techniques for the automatic generation of test inputs, including Search-Based Software Testing (SBST)~\citep{5342440}, feedback-directed random test generation~\citep{pacheco2007feedback,artzi2011framework,pradel2012fully}, Dynamic Symbolic Execution (DSE)~\citep{king1976symbolic,godefroid2005dart,xie2005symstra,majumdar2007directed,cadar2013symbolic}, and concolic execution~\citep{sen2005cute,cadar2008exe,sen2006cute}. While the tools based on those techniques have shown effectiveness, they often face limitations that hinder their adoption in real-world projects.

For example, while prior research has underscored the efficacy of Search-Based Software Testing (SBST) techniques in attaining notable code coverage~\citep{panichella2015reformulating, panichella2017automated}, \citet{perera2020defect} argue that high code coverage alone does not guarantee the optimal detection of bugs. In line with this, \citet{shamshiri2015automatically} and \citet{almasi2017industrial} assessed the performance of EvoSuite~\citep{fraser2011evosuite}, a leading SBST tool, against alternative test generation methods and tools like Randoop~\citep{pacheco2007feedback}, focusing on open-source and proprietary software projects, respectively. Their findings suggest a superior performance by EvoSuite over its counterparts, but also demonstrate that it falls short in effectively detecting genuine bugs. Notably, EvoSuite could identify only about 23\% of bugs from the Defects4J dataset~\citep{just2014defects4j}, even when the testing criterion was set at 100\% branch coverage.

One of the main reasons behind this limitation is that these generators primarily rely on either randomly-generated inputs or inputs from a fixed pool, which may not match the project specifications~\citep{ASE-2017-ToffolaSP}. Additionally, test generators tend to focus on the source code and its dynamic execution, generating less natural and readable values~\citep{shelke2014generation}.

To address these challenges, researchers have proposed various approaches: Some have leveraged test corpora~\citep{ASE-2017-ToffolaSP}, while others have explored web search queries~\citep{shelke2014generation,mcminn2012search,shahbaz2012automated}, user session data~\citep{elbaum2003improving}, web services~\citep{bozkurt2011automatically}, or the web of data~\citep{mariani2014link} to generate realistic test inputs. Regarding mobile application testing, \citet{liu2017automatic} leveraged the Google news corpus. In~\citep{milani2014leveraging}, researchers leveraged existing tests to automate test generation for web applications. Nevertheless, despite the existence of these approaches, the potential of bug reports as a valuable source of relevant inputs, including strings for test data generation, remains largely untapped.

Researchers have previously explored extracting test cases from bug reports, such as analyzing multicore dumps to facilitate concurrency bug reproduction~\citep{weeratunge2010analyzing}, reproducing system-level concurrency failures~\citep{yu2017descry}, translating bug reports into test cases for mobile apps~\citep{fazzini2018automatically}, and enriching compiler testing with real programs from bug reports~\citep{zhong2022enriching}. Our work builds on these foundations by introducing a new angle: we propose \name, a technique that mines literal inputs from bug reports to improve the relevance and effectiveness of automated test case generation.

Unlike previous studies, which often focus on generating test cases as a whole, our approach emphasizes the extraction of specific input values from bug reports, which are crucial for enhancing test coverage and bug detection capabilities. Furthermore, to address the complexity and ambiguity often present in bug reports, \name incorporates a filtering mechanism using a Large Language Model (LLM), specifically GPT-3.5-turbo\footnote{https://platform.openai.com/docs/models/gpt-3-5-turbo/[accessed 2024-05-21]}. This LLM component is capable of understanding the semantic nuances of bug reports, allowing it to refine the extracted literals and improve their relevance for triggering bugs during test execution~\citep{fan2023large, wang2024software}.

Additionally, \name integrates seamlessly with the EvoSuite test case generation tool, allowing for the direct incorporation of these LLM-refined literals into automatically generated test cases. This integration not only enhances the traditional test generation process by ensuring more contextually relevant inputs but also addresses challenges in test oracle generation by increasing the likelihood that the generated test cases will expose latent defects~\citep{liu2024testing}.

\textbf{This paper.} Bug reports offer a diverse range of example inputs which remain largely untapped in the extraction of inputs for automatic test case generation. Leveraging bug reports for this purpose offers two significant advantages. Firstly, they provide a wealth of valid inputs for various string types, enhancing test coverage and bug detection. Secondly, bug reports typically contain human-readable inputs, which prove invaluable when manual confirmation is necessary due to the absence of an automated oracle.

In this study, we propose a simple, yet effective approach for automatically extracting real test inputs from bug reports, aimed at addressing the problem of automatic test case generation containing relevant test inputs. Our approach involves exploring bug reports to identify and extract relevant inputs found in bug reports. We developed a tool called \name that enables us to automatically extract these relevant inputs, both qualitatively and quantitatively. To further enhance the effectiveness of the extracted inputs, we integrate a filtering step using GPT-3.5-turbo, an LLM capable of understanding the semantic context of bug reports and refining the inputs accordingly~\citep{tsigkanos2023variable, yang2023white}.

To generate test cases incorporating these inputs, we modified the source code of EvoSuite~\citep{fraser2011evosuite}, a widely known search-based test suite generator tool used for automatic test case generation. Additionally, we extended our evaluation by incorporating Randoop~\citep{pacheco2007feedback}, a feedback-directed random testing tool, to compare the effectiveness of test cases generated with \name's extracted inputs. To evaluate our generated test cases, we use the Defects4J benchmark~\citep{just2014defects4j}.

The main contributions of this paper are as follows:
\begin{enumerate}
\item We present \name, an automatic test input extraction approach. This approach offers several advantages, such as the ability to efficiently extract realistic test inputs for testing projects with semantic information, and the improvement of the efficiency of automatic test case generation for inputs that cannot be effectively generated randomly.
\item We showcase findings from practical case studies conducted on Defects4J projects. These were designed to assess the efficacy of our methodology in generating test cases based on bug reports, in contrast to the baseline approach of EvoSuite and Randoop which operate without external inputs.
\item We emphasize the significance of integrating external inputs into EvoSuite and Randoop, particularly inputs extracted from bug reports. For EvoSuite, we modified its source code to enable the use of external inputs, as it does not support this feature by default. In contrast, Randoop inherently supports external input files, so we directly fed it with the extracted inputs. These inputs offer crucial context, bolstering the performance of both tools, particularly when used in conjunction with Dynamic Symbolic Execution (DSE) for EvoSuite.
\item We demonstrate the effectiveness of our approach by showcasing the finding of valid, well-formed inputs from bug reports, resulting in improved bug detection and enhanced test coverage for a program's source code. To foster further research in this area, we have publicly shared the implementation of our approach and all relevant experimental data in an anonymous repository. The repository is accessible via the following link:
\begin{center}
    \url{https://anonymous.4open.science/r/BRMiner-C853/}
\end{center}
\end{enumerate}

The rest of this paper is organized as follows. Section~\ref{sec:brminer} presents our approach for relevant input extraction from bug reports. Section~\ref{sec:setup} provides an overview of our experimental setup, including implementation details, evaluation of technical challenges, and presentation of results (Section~\ref{sec:results}). Section~\ref{sec:discussion} discusses existing research on test input extraction and generation in the field of automatic test generation, along with the limitations of our approach and future research directions. Finally, Section~\ref{sec:conclusion} summarizes the paper, draws conclusions, and mentions future work.





==> Sections/results.tex <==
\section{Experimental Results}
\label{sec:results}
This section outlines the experimental results and addresses the research questions.

% \subsection{[RQ1]: Incorporation of relevant inputs from bug reports into human-written test cases.}
% %\subsection{[RQ1]: What is the extent to which relevant inputs mentioned in bug reports are incorporated into manually written test cases by humans?}

% \noindent\textbf{Experiment Goal: }In this experiment, we aim to explore the prevalence of relevant inputs from bug reports in manually written test cases on a large scale. While initial manual verification has identified certain relevant inputs, it is essential to determine their general presence in bug reports used for successful patched versions. Following the definition provided in Section~\ref{subsec:rel-inputs} and excluding instances of similar patterns, we can evaluate the frequency and consistency of their incorporation into the manual test cases. \par
% %\vspace{0.2cm}\noindent {\bf Experiment Objective:}
% %On a large scale, this allows us to confirm the presence of relevant inputs in the bug reports. 
% % Our objective in this experiment is to investigate the presence of relevant inputs from bug reports in manually written test cases on a large scale. While manual verification of a few bug reports has allowed us to identify some relevant inputs, it is crucial to determine whether there are generally relevant inputs in the bug reports used for the test cases that have successfully passed the patched version. Thus, by following the definition of a relevant input provided in Section~\ref{subsec:rel-inputs} and excluding cases where the same patterns were found, we can evaluate the frequency and consistency of their inclusion in the manual test cases.
% \noindent\textbf{Experiment Design: } To consolidate the results of the manual check, we performed an automatic check on the Defects4J projects, as it provides us with the associated test case for each bug report. We utilized the code-tokenize tool, developed as part of~\citep{richter2022tssb}, to tokenize the bug reports. Subsequently, we extracted the inputs present in the test cases using the Javalang parser described in Section~\ref{subsec:overview}. Finally, for each bug report, we intersected the tokens from the bug reports with the literals extracted from the test cases. \par
% %Figure~\ref{fig:relevant-inputs-definition} gives an overview of the approach we implemented for large-scale verification on Defects4J. 
% %\begin{figure}[h!]
%     %\includegraphics[scale=0.5]{relevant-inputs-definition}
%     %\includegraphics[width=8.5cm, height=8cm]{relevant-inputs-definition}
%     %\caption{Overview of the intersection approach between bug reports and test cases.}
%     %\label{fig:relevant-inputs-definition}
% %\end{figure}
% % \begin{figure*}
% %   \centering
% %   \includegraphics[width=0.8\textwidth]{Images/Relevant-inputs-definition}
% %   \caption{Overview of the intersection approach between bug reports and test cases.\jk{you can save space by reducing and redoing this figure.}
% %   \ah{We can remove this figure altogether. The approach it shows is quite simple and we don't need a figure to explain it.}}
% %     \label{fig:relevant-inputs-definition}
% % \end{figure*}
% %\textbf{RQ 2: What is the extent to which relevant inputs mentioned in bug reports are incorporated into manually written test cases by humans?} \par
% \noindent\textbf{Experiment Results: }To answer this research question, we analyze and compare the number of literals in the test cases and those in the bug reports.
% Table~\ref{table:1} shows that in Defects4J, of the 7,855 inputs extracted from the test cases, 1,129 were in the bug reports (14.37\%), confirming the observations of the manual exploration. This outcome is promising, although it does not consider relevant inputs that differ but share a similar pattern.
% %\vspace{0.2cm}\noindent {\bf Results:}

% \begin{table}
%     \centering
%     \caption{Number of relevant inputs in bug reports and associated test cases}
%     \scalebox{0.8}
% {
%     \begin{tabular}{@{}l@{}rrr@{}}
%         \toprule
%         \textbf{Projects} & \textbf{\# of bugs} & \textbf{\# of inputs} & \textbf{Bug reports inputs} \\
%         & & \textbf{in test cases} & \textbf{$\cap$ test cases literals}\\\midrule
%         Cli & 39 & 484 & 93 \\ 
%         Codec & 18 & 119 & 29 \\ 
%         Collections & 4 & 20 & 17 \\
%         Compress & 47 & 260 & 49 \\ 
%         Csv & 16 & 96 & 30 \\ 
%         JxPath & 22 & 188 & 23 \\ 
%         Lang & 64 & 1,102 & 120 \\ 
%         Math & 106 & 1,295 & 408 \\ 
%         Closure & 174 & 2,486 & 33 \\
%         Gson & 18 & 67 & 11 \\ 
%         JacksonCore & 26 & 158 & 30 \\ 
%         JacksonDatabind & 112 & 446 & 101 \\
%         JacksonXml & 6 & 43 & 8 \\ 
%         Jsoup & 93 & 660 & 119 \\ 
%         Mockito & 38 & 89 & 12 \\ 
%         Time & 26 & 342 & 46 \\ \midrule
%         \centering \textbf{Total} & \textbf{809} & \textbf{7,855} & \textbf{1,129} \\
%         \bottomrule
%     \end{tabular}
%     \label{table:1}
% }
% \end{table}

% \highlight{Summary of \textbf{RQ1:} 
% %The experiment aimed to investigate the extent to which relevant inputs mentioned in bug reports are incorporated into manually written test cases by humans. 
% We found 1,129 relevant inputs from bug reports to be present in test cases written by developers. 
% This highlights the importance of leveraging bug reports as a source of test input values for effective automatic test case generation and hence underlines the value of \name.}
\subsection{[RQ1]: Incorporation of relevant inputs from bug reports into human-written test cases.}

\noindent\textbf{Experiment Goal: }In this experiment, we aim to assess the consistency with which relevant inputs from bug reports are incorporated into manually written test cases across a large dataset. Initial manual verification identified certain relevant inputs; however, this study seeks to determine their consistent presence in bug reports associated with successful patched versions of the software. By following the definition provided in Section~\ref{subsec:rel-inputs}, and considering the aggregation of results by project, we provide an overall estimate of the incorporation of these inputs into manual test cases.

\noindent\textbf{Experiment Design: } To validate and extend the findings from the manual verification, we performed an automated analysis on the Defects4J projects, which provide both bug reports and associated test cases. The process involved two key steps:
\begin{itemize}
    \item \textbf{Grouping by Project:} For each project in Defects4J, we first extracted all the inputs contained in the test cases using the \texttt{Javalang} parser. These extracted inputs were then grouped by project. Similarly, we tokenized each bug report within a project using the \texttt{code-tokenize} tool, developed as part of~\citep{richter2022tssb}, and grouped the resulting tokens by project.
    
    \item \textbf{Intersection Analysis:} Once the inputs from the test cases and the tokens from the bug reports were grouped by project, we performed an intersection analysis for each project. This analysis identified the common inputs shared between the bug reports and the test cases written by human developers. By aggregating the results across all bug reports within each project, we obtained a global estimate of the number of identical inputs found in both sources.
\end{itemize}

Given the variability in the quality and completeness of bug reports, we aggregated the results by project. This aggregation provides a comprehensive estimate that highlights the extent to which inputs found in bug reports are consistently leveraged in human-written test cases, even when individual reports may vary in quality and quantity. Algorithm~\ref{alg:intersection} outlines the process.

\begin{algorithm}
\vspace{3mm}
\caption{Incorporation of Relevant Inputs from Bug Reports into Test Cases}\label{alg:intersection}
\begin{algorithmic}[1]
    \Procedure{AnalyzeRelevantInputs}{}
        \State \textbf{Input:} BugReports[], TestCases[]
        \State \textbf{Output:} CommonInputs[]
        
        \For{each Project \textit{P} in Defects4J}
            \State \textbf{Step 1: Tokenization}
            \State \textit{P\_Tokens} $\gets$ TokenizeAndGroupByProject(BugReports[P])
            
            \State \textbf{Step 2: Literal Extraction}
            \State \textit{P\_Literals} $\gets$ ExtractAndGroupByProject(TestCases[P])
            
            \State \textbf{Step 3: Intersection Analysis}
            \State \textit{CommonInputs[P]} $\gets$ Intersection(P\_Tokens, P\_Literals)
        \EndFor
        
        \State \textbf{return} CommonInputs
    \EndProcedure
\end{algorithmic}
%\vspace{3mm}
\end{algorithm}
\vspace{5mm}

\noindent\textbf{Experiment Results: }The results of this experiment, shown in Table~\ref{table:1}, indicate that across the Defects4J projects, 1,129 out of the 7,855 inputs extracted from the test cases (approximately 14.37\%) were also present in the bug reports. This finding, which aligns with the initial manual exploration, demonstrates a significant overlap and highlights the importance of bug reports as a source of relevant inputs for automatic test case generation. It is important to note that this analysis provides an aggregated view, ensuring that the results reflect a consistent trend across projects rather than isolated instances.

\begin{table}
\vspace{3mm}
    \centering
    \caption{Number of relevant inputs in bug reports and associated test cases}
    \scalebox{0.8}
{
    \begin{tabular}{@{}l@{}rrr@{}}
        \toprule
        \textbf{Projects} & \textbf{\# of bugs} & \textbf{\# of inputs} & \textbf{Bug reports inputs} \\
        & & \textbf{in test cases} & \textbf{$\cap$ test cases literals}\\\midrule
        Cli & 39 & 484 & 93 \\ 
        Codec & 18 & 119 & 29 \\ 
        Collections & 4 & 20 & 17 \\
        Compress & 47 & 260 & 49 \\ 
        Csv & 16 & 96 & 30 \\ 
        JxPath & 22 & 188 & 23 \\ 
        Lang & 64 & 1,102 & 120 \\ 
        Math & 106 & 1,295 & 408 \\ 
        Closure & 174 & 2,486 & 33 \\
        Gson & 18 & 67 & 11 \\ 
        JacksonCore & 26 & 158 & 30 \\ 
        JacksonDatabind & 112 & 446 & 101 \\
        JacksonXml & 6 & 43 & 8 \\ 
        Jsoup & 93 & 660 & 119 \\ 
        Mockito & 38 & 89 & 12 \\ 
        Time & 26 & 342 & 46 \\ \midrule
        \centering \textbf{Total} & \textbf{809} & \textbf{7,855} & \textbf{1,129} \\
        \bottomrule
    \end{tabular}
    \label{table:1}
}
\vspace{3mm}
\end{table}

\vspace{0.2cm}\noindent\highlight{Summary of \textbf{RQ1:}
The identification of 1,129 relevant inputs from bug reports within the manually written test cases underscores the importance of leveraging bug reports as a critical source of test input values. This finding validates the utility of BRMiner in extracting these inputs, which can significantly enhance the effectiveness of automated test case generation.
}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{[RQ2]: Relevance rate of \name-extracted potential relevant inputs}
% %\subsection{[RQ2]: What is the rate of actual relevant inputs among the potential inputs extracted by \name?}

% \noindent\textbf{Experiment Goal: }The experiment aims to evaluate \name's efficacy in automatically extracting relevant inputs from bug reports. The focus lies in assessing the extraction rate and accuracy within the Defects4J projects. By conducting this analysis on these projects, the aim is to gather empirical evidence on \name's performance in automatically extracting relevant inputs from real-world bug reports. \par
% %The goals of our empirical study are to determine if our approach can extract all the relevant inputs in a bug report or at least half of them and to determine if these inputs improve the quality of tests generated by the automated test generator.
% %The research question presented in Section XXX is the one that our experiments are designed to answer.
% %The research questions provided in the following paragraphs are what our experiments are intended to address.
% % The objective of this experiment is to assess the efficiency of \name in automatically extracting relevant inputs from bug reports. In this evaluation, we focus on measuring \name's extraction rate and accuracy in extracting these inputs from bug reports within the Defects4J projects. By conducting this experiment on the Defects4J projects, we can gather empirical evidence on the performance of \name in automatically extracting relevant inputs from real-world bug reports.
% \noindent\textbf{Experiment Design: }In this section, we present the method we developed to assess \name's efficiency and provide an overview of the evaluation process. For the input extraction, we employed two implementations of \name: one utilizing regular expressions (Regex) to extract inputs from natural language texts, and the other exclusively relying on Javalang, a parser mentioned in Section~\ref{subsec:overview}, to extract inputs from both source code and natural language texts. All the inputs we extract are potentially relevant inputs. To evaluate the effectiveness of \name in extracting relevant inputs, we conducted tests on the sixteen Defects4J projects listed in Table~\ref{table:1}. \par
% %Once the text has been structured into source code and natural language, we proceed to input extraction. For the text containing the source codes, we used a parser, Javalang mentioned in section ~\ref{\name-overview}, to retrieve the various literals contained therein (string and numeric). The extraction of inputs contained in the natural language text was performed using regular expressions. All the inputs we extract are potentially relevant inputs.
% %: Apache Commons Cli, Apache Commons Codec, Apache Commons Collections,
% %Apache Commons Compress, Apache Commons Csv, Apache Commons Jxpath, Apache Commons Lang, Apache Commons Math, Gson, Closure, Jackson-core, Jackson-databind, Jackson-dataformat-xml, Jsoup, Mockito and Joda Time . \par
% %In this section, we present the method we developed to assess \name's efficiency and provide an overview of the evaluation process. We employed two implementations of \name: one utilizing regular expressions (Regex) to extract inputs from natural language texts, and the other exclusively relying on Javalang to extract inputs from both source code and natural language texts. The outcomes of these experiments are summarized in Table ~\ref{result-with-&-without-regex}.
% \noindent\textbf{Experiment Results: }The findings, summarized in TableTable~\ref{result-with-&-without-regex}, indicate that the extraction rate with regexes stands at 68.7\%, dropping to 50.2\% without regexes, presenting a difference of 18.47\%. While the use of regexes boosts the extraction rate, it introduces more false positives, reducing precision. Specifically, precision stands at 8.1\% with regexes and 35.17\% with Javalang alone. While regexes enhance the extraction rate, precision suffers due to increased false positives. Conversely, relying solely on Javalang improves precision while maintaining a satisfactory extraction rate. However, it's important to note that false positives may include potentially relevant inputs that exhibit a similar pattern to those in human-written tests. \par
% % The outcomes of these experiments are summarized in Table~\ref{result-with-&-without-regex},
% % %The results in Table ~\ref{result-with-&-without-regex} 
% % which reveal that the extraction rate with regexes is 68.7\%, whereas it decreases to 50.2\% without regexes, representing a difference of 18.47\% points. 
% % However, although the extraction rate is higher when using regexes, it also leads to an increase in false positives, which subsequently lowers precision. %\jk{Be careful, we have "precision" in the table. i guess we should only discuss precision here, and not accuracy.}. 
% % Specifically, the precision is 8.1\% when regexes are employed, compared to 35.17\% when solely utilizing Javalang. %Additionally, Table~\ref{result-with-&-without-regex} demonstrates that an approach based on simple tokenization yields sub-optimal results.
% % %\jk{precision?} 
% % We observe that employing regexes improves the extraction rate; however, it comes at the expense of precision due to the higher false positive rate. On the other hand, relying solely on Javalang enhances precision while maintaining a satisfactory extraction rate. However me must keep in mind that false positives may include potentially relevant inputs that, while not identical to those in human-written tests, exhibit a similar pattern.
% % %These results highlight the limitations of a tokenization-based approach, as demonstrated in Table~\ref{result-with-&-without-regex}.

% \begin{table*}
%     \centering
%     \caption{Results for \name effectiveness. BR for Bug Reports, TC for Test Cases, \name inputs for unique inputs extracted by \name, BR $\cap$ TC inputs for the intersection of inputs extracted from Bug Reports and Test Cases, BR unique Tokens for the number of unique tokens in each Bug Report, and \name $\cap$ TC Inputs for the intersection of inputs extracted by \name and Test Cases}
    
%     \label{result-with-&-without-regex}
%     \scalebox{0.55}
% {
%     \begin{tabular}{@{}l@{}rr|rrrr|rrrr@{}}
%  \toprule
%  & & & \multicolumn{4}{c|}{without regex}  & \multicolumn{4}{c}{ with regex} \\ 
% \midrule
%                  & BR $\cap$ TC & BR unique & \name $\cap$ & \name  & \name & Precision & BR $\cap$ TC & \name  & \name & Precision \\
%         Projects & inputs       & tokens    & TC inputs    & inputs & (\%)  & (\%)           & Inputs       & inputs & (\%)  & (\%)           \\
%         \midrule
%         Cli & 93 & \num{13146} & 62 & 149 & 66.7 & 41.6 & 70 & 628 & 75.3 & 11.1 \\
%         Codec & 29 & \num{9702} & 13 & 73 & 44.8 & 17.8 & 15 & 488 & 51.7 & 3.1 \\
%         Collections & 17 & \num{2320} & 15 & 32 &  88.2 & 46.9 & 15 & 94 & 88.2 & 15.9 \\
%         Compress & 49 & \num{20002} & 24 & 123 & 49.0 & 19.5 & 45 & 975 & 91.8 & 4.6 \\
%         Csv & 30 & \num{5143} & 13 & 53 & 43.3 & 24.5 & 13 & 186 & 43.0 & 7.0 \\
%         JxPath & 23 & \num{5525} & 12 & 40 & 52.0 & 30.0 & 15 & 261 & 65.2 & 5.7 \\
%         Lang & 120 & \num{17429} & 56 & 135 & 46.7 & 41.5 & 65 & 736 & 54.2 & 8.8 \\
%         Math & 408 & \num{41444} & 161 & 312 &  39.5 & 51.6 & 257 & 2201 & 63.0 & 11.7 \\
%         Closure & 33 & \num{12927} & 0 & 65 & 00.0 & 0.0 & 0 & 881 & 00.0 & 0.0 \\
%         Gson & 11 & \num{2825} & 5 & 23 & 45.4 & 21.7 & 8 & 23 & 72.7 & 34.8 \\
%         JacksonCore & 30 & \num{4239} & 19 & 40 & 63.3 & 47.5 & 25 & 256 & 83.3 & 9.8 \\
%         JacksonDatabind & 101 & \num{21507} & 56 & 182 & 55.4 & 30.8 & 92 & 1794 & 91.1 & 5.0 \\
%         JacksonXml & 8 & \num{1372} & 7 & 19 & 87.5 & 36.8 & 7 & 41 & 87.5 & 17.1 \\
%         Jsoup & 119 & \num{11935} & 55 & 154 & 46.2 & 35.7 & 87 & 154 & 73.1 & 56.5 \\
%         Mockito & 12 & \num{5698} & 3 & 26 & 25.0 & 11.5 & 7 & 445 & 58.3 & 1.6 \\
%         Time & 46 & \num{3010} & 23 & 64 & 50.0 & 35.9 & 46 & 270 & 100 & 17.0 \\
%         \midrule
%         Total & \num{1129} & \num{178224} & 524 & 1490 & 50.2 & 35.2 & 767 & 9433 & 68.7 & 8.1 \\ \bottomrule
%     \end{tabular}
% }
% \end{table*}
% % \begin{comment}
% %     \begin{table*}[!t]
% %     \centering
% %     \caption{Results for \name effectiveness}
% %    % \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% %     \begin{tabular}{|P{1.8cm}|P{1.0cm}||P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}||P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}}
% %  \hline
% %  & & \multicolumn{5}{c||}{without regex}  & \multicolumn{5}{c|}{ with regex} \\ 
% %      \hline
% %         Projects & BR \& TC Inputs & \name \& TC Inputs & \name inputs & BR unique Tokens & \name Percentage & Precision & BR \& TC Inputs & \name inputs & BR unique Tokens & \name Percentage & Precision
% %         \\ \hline
% %         CLI & 93 & 62 & 149 & 13146 & 66,7 & 41,6 & 70 & 628 & 13146 & 75,3 & 
% % 11,1 \\ \hline
% %         CODEC & 29 & 13 & 73 & 9702 & 44,8 & 17,8 & 15 & 488 & 9702 & 
% % 51,7 & 3,1 \\ \hline
% %         COLLECTIONS & 17 & 15 & 32 & 2320 & 88,2 & 46,9 & 15 & 94 & 
% % 2320 & 88,2 & 15,9 \\ \hline
% %         COMPRESS & 49 & 24 & 123 & 20002 & 49 & 19,5 & 45 & 975 & 
% % 20002 & 91,8 & 4,6 \\ \hline
% %         CSV & 30 & 13 & 53 & 5143 & 43,33 & 24,53 & 13 & 186 & 5143 & 
% % 43 & 7 \\ \hline
% %         JXPATH & 23 & 12 & 40 & 5525 & 52 & 30 & 15 & 261 & 5525 & 65,2 
% % & 5,7 \\ \hline
% %         LANG & 120 & 56 & 135 & 17429 & 46,7 & 41,5 & 65 & 736 & 17429 
% % & 54,2 & 8,8 \\ \hline
% %         MATH & 408 & 161 & 312 & 41444 & 39,5 & 51,6 & 257 & 2201 & 
% % 41444 & 63 & 11,7 \\ \hline
% %         CLOSURE & 33 & 0 & 65 & 12927 & 0 & 0 & 0 & 881 & 12927 & 0 & 
% % 0 \\ \hline
% %         GSON & 11 & 5 & 23 & 2825 & 45,45 & 21,7 & 8 & 23 & 2825 & 
% % 72,7 & 34,8 \\ \hline
% %         J.CORE & 30 & 19 & 40 & 4239 & 63,3 & 47,5 & 25 & 256 & 4239 & 
% % 83,3 & 9,8 \\ \hline
% %         J.DATABIND & 101 & 56 & 182 & 21507 & 55,4 & 30,8 & 92 & 1794 
% % & 21507 & 91,1 & 5, \\ \hline
% %         J.XML & 8 & 7 & 19 & 1372 & 87,5 & 36,8 & 7 & 41 & 1372 & 87,5 & 
% % 17,1 \\ \hline
% %         JSOUP & 119 & 55 & 154 & 11935 & 46,2 & 35,7 & 87 & 154 & 
% % 11935 & 73,1 & 56,5 \\ \hline
% %         MOCKITO & 12 & 3 & 26 & 5698 & 25,0 & 11,5 & 7 & 445 & 5698 & 
% % 58,3 & 1,6 \\ \hline
% %         TIME & 46 & 23 & 64 & 3010 & 50,00 & 35,9 & 46 & 270 & 3010 & 
% % 100 & 17,0 \\ \hline
% %         TOTAL & 1129 & 524 & 1490 & 178224 & 50,2 & 35,2 & 767 & 9433 
% % & 178224 & 68,7 & 8,1 \\ \hline
% %     \end{tabular}
% %     \label{result-with-&-without-regex}
% % \end{table*}
% % \end{comment}
% %Projects & Inputs from BR \cap TC & Inputs from \name \cap TC & Inputs extracted by \name & BR unique tokens & \name Percentage & Precision & Inputs from BR \cap TC & Inputs from \name \cap TC & Inputs extracted by \name & BR unique tokens & \name Percentage & Precision
% %Projects & Inputs in Bug Report and test cases & Inputs in \name and test cases & All Inputs extracted by \name & Bug Report unique Tokens & \name Percentage & Precision & Inputs in \name and test cases & All Inputs extracted by \name & Bug Report unique Tokens & \name Percentage & Precision 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \highlight{Summary of \textbf{RQ2:} Using regular expressions improves test input extraction rates (+18.5\%) but decreases the precision from 35.2\% to 8.1\%. 
% %Simple tokenization also has limitations in effectively extracting precise test inputs.
% } \par

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{[RQ2]: Relevance Rate of \name-Extracted Potential Relevant Inputs}

\vspace{0.2cm}\noindent\textbf{Experiment Goal:}
The goal of this experiment is to evaluate BRMiner’s effectiveness in automatically extracting relevant inputs from bug reports. Specifically, we aim to assess both the Relevant Input Rate (RIR) and the Relevant Input Extraction Accuracy Rate (RIEAR) across various configurations. This analysis seeks to provide empirical evidence of BRMiner’s performance in identifying relevant inputs from real-world bug reports within the Defects4J projects.

\vspace{0.2cm}\noindent\textbf{Experiment Design:}
To achieve this, we conducted experiments using four different configurations:

\begin{itemize}
\item \textbf{Javalang Only:} This configuration uses the Javalang parser to extract inputs from both source code and natural language texts.
\item \textbf{Regex + Javalang:} This combines regular expressions (Regex) with Javalang to enhance input extraction from both source code and natural language texts.
\item \textbf{BRMiner:} This configuration represents our BRMiner approach, which integrates LLM filtering. BRMiner refines the extracted inputs using a ToT prompt and GPT-3.5-turbo to enhance the relevance of the final inputs used for testing.
\item \textbf{LLM Alone:} As a baseline, LLM Alone uses GPT-3.5-turbo to analyze bug reports and identify potential test inputs without any pre-extracted inputs.
\end{itemize}

The performance of these configurations was quantified using two key metrics:


\vspace{0.2cm}\noindent\textbf{Relevant Input Rate (RIR):} This metric measures the proportion of relevant inputs extracted by BRMiner (or any other configuration) relative to the total relevant inputs identified from the intersection of bug reports and test cases. It is calculated as:

\[
\text{RIR(\%)} = \left(\frac{| \text{TC} \cap \text{BRM} |}{| \text{BR} \cap \text{TC} |}\right) \times 100
\]

\vspace{0.2cm}\noindent\textbf{Relevant Input Extraction Accuracy Rate (RIEAR):} This metric indicates the proportion of BRMiner-extracted inputs that are actually relevant, considering the total number of unique inputs extracted by BRMiner. It is calculated as:

\[
\text{RIEAR(\%)} = \left(\frac{| \text{TC} \cap \text{BRM} |}{| \text{BRM} |}\right) \times 100
\]


Where:

\begin{itemize}
\item $| \text{TC} \cap \text{BRM} |$ represents the number of inputs that are present both in the test cases (TC) and those extracted by BRMiner (BRM).
\item $| \text{BR} \cap \text{TC} |$ represents the number of relevant inputs identified from the intersection of bug reports (BR) and test cases (TC).
\item $| \text{BRM} |$ represents the total number of unique inputs extracted by BRMiner.
\end{itemize}

\vspace{0.2cm}\noindent\textbf{Experiment Results:}
\begin{table*}
    \centering
    \caption{Effectiveness results for \name. BR represents Bug Reports, TC stands for Test Cases, BRM refers to unique inputs extracted by \name approach with the four scenarios, BR $\cap$ TC indicates the intersection of inputs extracted from Bug Reports and Test Cases, BR unique Tokens corresponds to the number of unique tokens in each Bug Report, and \name $\cap$ TC represents the intersection of inputs extracted by \name and Test Cases. "Databind" in the projects column refers to the jacksonDatabind project.}
    \label{brminer-extraction-efficacy}
    %\scalebox{0.55}
    \scalebox{0.41}
     %\scriptsize
    {
        \begin{tabular}{@{}l@{}rr|rrrr|rrrr|rrrr|rrrr@{}}
            \toprule
            & & & \multicolumn{4}{c|}{Javalang Only} & \multicolumn{4}{c|}{Regex + Javalang} & \multicolumn{4}{c|}{BRMiner} & \multicolumn{4}{c}{LLM Alone} \\
            \midrule
            & BR $\cap$ TC & BR unique & BRM $\cap$ & BRM  & RIR & RIEAR & BRM $\cap$ & BRM  & RIR & RIEAR & BRM $\cap$ & BRM  & RIR & RIEAR & BRM $\cap$ & BRM  & RIR & RIEAR \\
            Projects & inputs       & tokens    & TC    & inputs & (\%)  & (\%) & TC       & inputs & (\%)  & (\%) & TC       & inputs & (\%)  & (\%) & TC       & inputs & (\%)  & (\%) \\
            \midrule
            Cli & 93 & \num{13146} & 62 & 149 & 66.7 & \textbf{41.6} & \textbf{70} & 628 & \textbf{75.3} & 11.1 & 65 & 165 & 69.89 & 39.39 & 39 & 135 & 41.94 & 28.89 \\
            Codec & 29 & \num{9702} & 13 & 73 & 44.8 & 1\textbf{7.8} & \textbf{15} & 488 & 51.7 & 3.1 & 11 & 267 & 37.93 & 4.12 & 10 & \textbf{57} & 34.48 & 17.54 \\
            Collections & 17 & \num{2320} & \textbf{15} & 32 &  \textbf{88.2} & \textbf{46.9} & \textbf{15} & 94 & \textbf{88.2} & 15.9 & 10 & 55 & 58.82 & 18.18 & 9 & 24 & 52.94 & 37.50 \\
            Compress & 49 & \num{20002} & 24 & 123 & 49.0 & 19.5 & \textbf{45} & 975 & \textbf{91.8} & 4.6 & 39 & 158 & 79.59 & \textbf{24.68} & 17 & 73 & 34.69 & 23.29 \\
            Csv & 30 & \num{5143} & 13 & 53 & 43.3 & 24.5 & 13 & 186 & 43.0 & 7.0 & 18 & 64 & 60.0 & 28.13 & \textbf{19} & 41 & \textbf{63.33} & \textbf{46.34} \\
            JxPath & 23 & \num{5525} & 12 & 40 & 52.0 & 30.0 & \textbf{15} & 261 & \textbf{65.2} & 5.7 & 10 & 55 & 43.48 & 18.18 & 13 & 27 & 56.52 & \textbf{48.15} \\
            Lang & 120 & \num{17429} & 56 & 135 & 46.7 & 41.5 & 65 & 736 & 54.2 & 8.8 & \textbf{69} & 195 & \textbf{57.50} & 35.38 & 60 & 93 & 50.0 & \textbf{64.52} \\
            Math & 408 & \num{41444} & 161 & 312 &  39.5 & 51.6 & \textbf{257} & 2201 & \textbf{63.0} & 11.7 & 239 & 537 & 58.58 & 44.51 & 100 & 175 & 24.51 & \textbf{57.14} \\
            Closure & 33 & \num{12927} & 0 & 65 & 00.0 & 0.0 & 0 & 881 & 00.0 & 0.0 & 0 & 213 & 0.0 & 0.0 & 0 & 36 & 0.0 & 0.0 \\
            Gson & 11 & \num{2825} & 5 & 23 & 45.4 & 21.7 & 8 & 23 & 72.7 & 34.8 & 5 & 18 & 45.45 & 27.78 & \textbf{9} & 17 & \textbf{81.82} & \textbf{52.94} \\
            JacksonCore & 30 & \num{4239} & 19 & 40 & 63.3 & \textbf{47.5} & \textbf{25} & 256 & \textbf{83.3} & 9.8 & 23 & 105 & 76.67 & 21.90 & 11 & 28 & 36.67 & 39.29 \\
            Databind & 101 & \num{21507} & 56 & 182 & 55.4 & 30.8 & 92 & 1794 & 91.1 & 5.0 & \textbf{95} & 135 & \textbf{94.06} & \textbf{70.37} & 35 & 103 & 34.65 & 33.98 \\
            JacksonXml & 8 & \num{1372} & \textbf{7} & 19 & \textbf{87.5} & 36.8 & \textbf{7} & 41 & \textbf{87.5} & 17.1 & 5 & 21 & 62.50 & 23.81 & \textbf{7} & 19 & \textbf{87.5} & \textbf{36.84} \\
            Jsoup & 119 & \num{11935} & 55 & 154 & 46.2 & 35.7 & 87 & 154 & 73.1 & 56.5 & \textbf{92} & 96 & \textbf{77.31} & \textbf{95.83} & 39 & 99 & 32.77 & 39.39 \\
            Mockito & 12 & \num{5698} & 3 & 26 & 25.0 & 11.5 & \textbf{7} & 445 & 58.3 & 1.6 & \textbf{7} & 93 & \textbf{58.33} & 7.53 & 5 & 26 & 41.67 & \textbf{19.23} \\
            Time & 46 & \num{3010} & 23 & 64 & 50.0 & \textbf{35.9} & \textbf{46} & 270 & \textbf{100} & 17.0 & 37 & 109 & 80.43 & 33.94 & 21 & 78 & 45.65 & 26.92 \\
            \midrule
            Total/Average & \num{1129} & \num{178224} & 524 & 1490 & 50.2 & 35.2 & \textbf{767} & 9433 & \textbf{68.7} & 8.1 & 725 & 2286 & 60.03 & 31.71 & 394 & 1031 & 44.95 & \textbf{38.22} \\
            \bottomrule
        \end{tabular}
    }
    \vspace{3mm}
\end{table*}

The results, summarized in Table \ref{brminer-extraction-efficacy}, reveal that The \textbf{Javalang Only} method achieved a moderate Relevant Input Rate (RIR) of 50.2\% and a Relevant Input Extraction Accuracy Rate (RIEAR) of 35.2\%, indicating that while it effectively identifies relevant inputs, it may miss some due to its reliance on syntactic parsing alone. In contrast, the \textbf{Regex + Javalang} configuration showed the highest RIR at 68.7\% but had a lower RIEAR of 8.1\%, suggesting that this approach extracts a large number of inputs but includes many that are not relevant, leading to lower accuracy. The \textbf{BRMiner} approach demonstrated a balanced performance with an RIR of 60.03\% and an RIEAR of 31.71\%, highlighting its effectiveness in refining the input extraction process and balancing input extraction with accuracy. Lastly, the \textbf{LLM Alone} configuration, despite having the lowest RIR at 44.95\%, exhibited the highest RIEAR at 38.22\%, indicating that the LLM is effective in identifying precise and relevant inputs, though it may miss some without pre-extracted inputs.


\vspace{0.2cm}\noindent\highlight{Summary of \textbf{RQ2:} The results demonstrate that BRMiner is effective in extracting relevant inputs from bug reports, particularly when compared to configurations that either rely solely on syntactic analysis (Javalang Only) or combine regex with parsing. While the Regex + Javalang configuration excels in extracting a high quantity of inputs, it does so at the expense of accuracy. BRMiner, by integrating LLM filtering, provides a balanced approach with both a strong RIR and RIEAR, indicating its capability to enhance the quality of test case generation and contribute to software robustness and reliability.
}








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %Selecting the appropriate approach is crucial for accurate and efficient input extraction from bug reports.\lp{maybe to much the same as paragraphe above}}
% % The findings indicate that using regular expressions improves the extraction rate of potential inputs from bug reports. However, it also increases the false positive rate, leading to lower accuracy but it cannot hurt in our context. Relying solely on Javalang enhances accuracy while maintaining a satisfactory extraction rate. The tokenization-based approach showed limitations in effectively extracting relevant inputs. These findings emphasize the importance of selecting the appropriate approach for accurate and efficient input extraction from bug reports.
% \subsection{[RQ3]: Effect of \name-extracted inputs on bug detection rate}
% %\subsection{[RQ3]: Do tests generated using the extracted relevant inputs by \name exhibit a higher bug detection rate compared to tests generated without utilizing these inputs?}
% \noindent\textbf{Experiment Goal: }This experiment evaluates the effectiveness of \name's extracted inputs from bug reports in automatically generated test cases. We aim to determine if incorporating these inputs enhances bug detection compared to test generation without external inputs, thus assessing their impact on the test case quality. \par
% % This experiment evaluates the effectiveness of automatically generated test cases using inputs extracted from bug reports by \name. We want to determine if incorporating \name's extracted inputs enhances test case quality by detecting more bugs than test generation without external inputs. We compare two scenarios: one without external inputs (baseline) and another with inputs extracted by \name. This enables us to assess the impact of integrating relevant bug report inputs on the bug detection capability of the generated test cases.
% \noindent\textbf{Experiment Design:} \label{RQ3-experiment-design}Regression testing experiments were conducted using an approach similar to the one described in a prior study~\citep{shamshiri2015automatically}. In an empirical study, the authors focused on evaluating the effectiveness of automatic test case generators for bug detection. They examined three tools, EvoSuite, Randoop, and AgitarOne, using the Defects4J dataset in a regression scenario. Tests were generated on the fixed version of the bug, then executed on the buggy version to assess their ability to detect the bug. This methodology, depicted in Figure~\ref{fig:bug-detection-methodology}, resembles regression testing, serving to gauge the efficacy of the generated tests in identifying software defects. Omitting projects JacksonXml, Mockito, and Closure from the experiment was necessary due to Evosuite's inability to generate tests for these projects or the non-compilable nature of most generated tests. Three experiments were conducted, each employing different inputs for EvoSuite. The first experiment, \nolit, used EvoSuite without specific inputs as a baseline. The second, \projlit, utilized EvoSuite with inputs from \name tailored to each project. The third experiment, alllit, employed \name inputs from all projects, leveraging cross-project insights to maximize the mined test inputs \par
% % We conducted regression testing experiments following a similar approach as described in a previous study ~\citep{shamshiri2015automatically} where we generate tests on the fixed version of the bug and then run the tests on the buggy version and check if the tests could detect the bug, i.e., fail on the buggy version.
% % Figure ~\ref{fig:bug-detection-methodology} provides an overview of this methodology, highlighting the main steps and components involved.
% % This setup is akin to regression testing where we measure the effectiveness of the generated tests in identifying software defects.
% % % We have not presented the results for JacksonXml, as Evosuite was unable to generate test cases for all three experiments. We didn't select Mockito because Evosuite generated very few test cases, and these are not compilable. With Closure we were unable to generate any test cases. The thirteen open-source projects from Defects4J used for our experiments are enumerated in Figure~\ref{fig:test}.
% % Projects JacksonXml, Mockito, and Closure are omitted from this experiment because Evosuite either did not generate any tests for those projects or most of the generated tests were uncompilable.
% % %: Apache Commons Cli, Apache Commons Codec, Apache Commons Collections, Apache Commons Compress, Apache Commons Csv, Apache Commons Jxpath, Apache Commons Lang, Apache Commons Math, Gson, Jackson-core, Jackson-databind, Jackson-dataformat-xml, Joda Time, and Jsoup. 
% % Three experiments were performed with different inputs provided to EvoSuite.
% % %\jk{I counted 13 projects in Figure 7. Moreover, (maybe I missed something), please explain why you have less projects than in Table 2.}
% % In the first experiment, \nolit, we generated tests using EvoSuite without specific inputs as a baseline. The second experiment, \projlit, utilized EvoSuite with \name inputs specific to each project. In the third experiment, \alllit, \name inputs  extracted from all projects were used to capture cross-project knowledge and maximize the number of mined test inputs.
% % %\jk{are they \name inputs? If so, say: "with \name inputs"}
% % %\jk{are they \name inputs? If so, say: "with \name inputs"}
% % % Our experimental design was based on the methodology proposed by Shamshiri et al. ~\citep{shamshiri2015automatically}, which provided a solid foundation for our study. Figure ~\ref{fig:bug-detection-methodology} provides an overview of the methodology, highlighting the main steps and components involved. Adapting their methodology to our study's objectives and requirements ensured a robust experimental design.
% \begin{figure*}
%   \centering
%   %\includegraphics[width=0.8\textwidth]{Images/Bug-Detection-Experiments.pdf}
%   \includegraphics[width=0.9\textwidth]{Images/Bug-Detection-Experiments.pdf}
%    \caption{Overview of the methodology used to design the bugs detection experiments}
%     \label{fig:bug-detection-methodology}
% \end{figure*}
% %\jk{where is \name? simply add in "Evosuite with all the \name inputs. Same with "specific inputs"}
% % \noindent\textbf{Experiment Results: }The comparison between bug detection outcomes in experiments  with different time budgets, as depicted in Figure~\ref{fig:bug-detected-1minute} and Figure~\ref{fig:bug-detected-3minutes}, sheds light on the impact of time constraints on bug detection effectiveness. It helps us understand whether allocating more time for test generation improves bug detection rates or enhances testing coverage.
% \noindent\textbf{Experiment Results: }Comparing bug detection results with and without \name inputs, as depicted in Figure~\ref{fig:bug-detected-3minutes}, highlights the impact of these inputs on EvoSuite's bug detection efficiency, providing insights into their effectiveness. \par
% %\begin{figure}[h!]
%    % %\includegraphics[width=9cm, height=4.5cm]{bug-detection-methodology}
%      %\includegraphics[width=0.5\textwidth]{bug-detection-methodology}
%     %\caption{Overview of the methodology used to design the bugs detection experiments.}
%     %\label{fig:bug-detection-methodology}
% %\end{figure}
% %\begin{figure}[h!]
% %    \includegraphics[width=9cm, height=6.5cm]{Images/bug-detected}
% %    \caption{Number of bugs detected during the five iterations per project and for each experiment.}
% %    \label{fig:bug-detected}
% %\end{figure}
% % %%%%%%%%%%%%%%
% % \begin{figure*}[t]
% % \begin{subfigure}[t]{0.45\linewidth}\centering
% %  \includegraphics[width=\linewidth]{Images/test-generated-1minute.pdf}
% %     \caption{Number of test generated during the five iterations per project and for each experiment.}
% %     \label{fig:test-generated-1minute}
% % \end{subfigure}
% % \hfill
% % \begin{subfigure}[t]{0.45\linewidth}\centering
% %  \includegraphics[width=\linewidth]{Images/bug-detected-exp-1minute}
% %     \caption{Number of bugs detected during the five iterations per project and for each experiment.}
% %     \label{fig:bug-detected-1minute}
% % \end{subfigure}%
% % \caption{Number of generated test and number of detected bugs with a time budget of one minute.}
% % \label{fig:test}
% % \end{figure*}
% % %%%%%%%%%%%%%
% %%%%%%%%%%%%%%
% % \begin{figure*}[t]
% % %\begin{subfigure}[t]{0.45\linewidth}\centering
% % \begin{subfigure}[t]{0.5\linewidth}\centering
% %  \includegraphics[width=\linewidth]{Images/test-generated-3minutes}
% %     \caption{Number of test generated during the five iterations per project.}
% %     \label{fig:test-generated-3minutes}
% % \end{subfigure}
% % \hfill
% % %\begin{subfigure}[t]{0.45\linewidth}\centering
% % \begin{subfigure}[t]{0.5\linewidth}\centering
% %  \includegraphics[width=\linewidth]{Images/bug-detected-exp-3minutes}
% %     \caption{Number of bugs detected during the five iterations per project.}
% %     \label{fig:bug-detected-3minutes}
% % \end{subfigure}%
% % \caption{Number of generated tests and number of detected bugs with a time budget of three minutes and five iterations.}
% % \end{figure*}


% \begin{figure*}[!ht]
%     \centering
%     \flushleft
%     \subfigure[Number of test generated during the five iterations per project]{\label{fig:test-generated-3minutes}
%     \includegraphics[scale=0.35]{Images/test-generated-3minutes}%
%     }
%     \subfigure[Number of bugs detected during the five iterations per project]{\label{fig:bug-detected-3minutes}
%     \includegraphics[scale=0.35]{Images/bug-detected-exp-3minutes}%
%     }
%     \caption{Number of generated tests and number of detected bugs with a time budget of three minutes and five iterations.}
% \end{figure*}


% % %%%%%%%%%%%%%
% % In the experiments conducted with a one-minute time budget Figure~\ref{fig:bug-detected-1minute}, the use of inputs in the test case generation process resulted in improved bug detection. The experiment without inputs detected 268 bugs, while the experiment with project-specific inputs detected 267 bugs. However, when all inputs were employed, 270 bugs were detected, indicating a slight increase compared to the other two experiments. A detailed analysis using a Venn diagram Figure~\ref{fig:ven-diagram-1minute} revealed that specific inputs and all inputs exclusively detected 10 and 14 bugs, respectively. Additionally, the combination of these two experiments detected 19 bugs exclusively. Comparatively, the baseline approach detected 20 bugs alone, whereas our approach detected a total of 43 (14+19+10) bugs, demonstrating a significant improvement.
% % %\jk{alone}
% % %\jk{is it 14+19+10? If so, write: a total of 43 (14+19+10) bugs}
% % Despite generating more tests (106,140 generated test cases) as we can see in Figure~\ref{fig:test-generated-1minute}, the baseline approach detected fewer bugs than the experiments using inputs. The second experiment -ProjLit- with project-specific inputs generated fewer tests (105,383 generated test cases), while the third experiment -AllLit- with all inputs generated even fewer tests (106,116 generated test cases). Surprisingly, the third experiment detected two additional bugs, demonstrating the effectiveness of using all inputs. Combining the results of the second and third experiments, a total of 43 bugs were detected, surpassing the 20 bugs uniquely detected by the baseline. A closer analysis of Figure~\ref{fig:bug-detected-1minute} shows better bug detection results for Apache Commons Codec and Apache Commons Lang with our approach. The experiment with project-specific inputs performed well with Jsoup, while the experiment with all inputs showed slightly better results for Apache Commons Compress, Apache Commons Jxpath, and Jackson-core. These findings highlight the benefits of incorporating inputs, enhancing bug detection capabilities. The specific projects exhibited varying bug detection performance, emphasizing the importance of project-specific inputs and broader input application.
% % %\jk{uniquely}
% Significant improvements can be observed in bug detection, particularly for experiments utilizing inputs. The experiments incorporating \name-extracted literals detect more bugs compared to the baseline approach. Analysis from Figure~\ref{fig:test-generated-3minutes} reveals insights into the number of tests generated per project and experiment. Interestingly, although the experiment without literals generates a higher number of test cases, it detects fewer bugs compared to the other two experiments. \par
% % \begin{comment}
% % Figure \ref{fig:test-generated-vs-bug-detected} further illustrates the relationship between the number of test cases generated and the number of bugs detected.
% % \end{comment}
% In these experiments, the approach without inputs generated 131,111 test cases and detected 295 bugs out of the 591 in the fourteen projects. The experiment utilizing project-specific literals generated 128,130 test cases and detected 304 bugs, 9 bugs more than the baseline. The experiment incorporating all literals generated 125,381 test cases and detected 307 bugs, surpassing the baseline by 12 bugs.
% % \begin{comment}
% % \begin{figure}[h!]
% %     \includegraphics[width=9cm, height=6.5cm]{Images/test-generated}
% %     \caption{Number of test generated during the five iterations per project and for each experiment.}
% %     \label{fig:test-generated}
% % \end{figure}
% % \begin{figure}[h!]
% %     \includegraphics[width=9cm, height=6.5cm]{Images/test-generated-vs-bug-detected}
% %     \caption{Relationship between the number of test cases generated and the number of bugs detected.}
% %     \label{fig:test-generated-vs-bug-detected}
% % \end{figure}
% % \end{comment}
% The Venn diagram in Figure~\ref{fig:ven-diagram-3minutes} illustrates bug detection relationships among the experiments. A detailed analysis reveals that the baseline exclusively detected 13 bugs, while project-specific inputs and all inputs exclusively detected 11 and 12 bugs, respectively. Moreover, 22 bugs were detected when both project-specific inputs and all inputs were utilized, resulting in a total of 45 (11+12+22) bugs detected with \name-extracted inputs, over three times the number detected by the baseline. \par
% % \begin{comment}
% % \begin{figure}[h!]
% %     \includegraphics[width=9cm, height=6.5cm]{Images/venn-diagram}
% %     \caption{Relations between the three experiments in terms of bug detection.}
% %     \label{fig:venn-diagram}
% % \end{figure}
% % \end{comment}
% %\begin{figure}
% \begin{figure}
%     %\includegraphics [scale=0.45] {\brminer-approache}
%     % \includegraphics[width=8.5cm, height=8cm]{Images/approache-vf.pdf}
%     \includegraphics[width=\linewidth, height=6.8cm]{Images/venn_diagram_3minutes-nocolors}
%      %\includegraphics[width=.9\linewidth]{Images/venn_diagram_3minutes-nocolors}
%     \caption{Relations between the three experiments in terms of bug detection with three minutes}
%     \label{fig:ven-diagram-3minutes}
% \end{figure}
% % %%%%%%%%%%%
% % \begin{figure*}[t]
% % \begin{subfigure}[t]{0.45\linewidth}\centering
% %  %\includegraphics[width=9cm, height=6.5cm]{Images/venn_diagram_1minute}
% %  \includegraphics[width=\linewidth]{Images/venn_diagram_1minute-nocolors}
% % \caption{Relations between the three experiments in terms of bug detection with one minute.}
% % \label{fig:ven-diagram-1minute}
% % \end{subfigure}
% % \hfill
% % \begin{subfigure}[t]{0.45\linewidth}\centering
% %  %\includegraphics[width=9cm, height=6.5cm]{Images/venn_diagram_3minutes}
% %  \includegraphics[width=\linewidth]{Images/venn_diagram_3minutes-nocolors}
% % \caption{Relations between the three experiments in terms of bug detection with three minutes.}
% % \label{fig:ven-diagram-3minutes}
% % \end{subfigure}%
% % % \vspace{-2mm}
% % \caption{Relations between the three experiments in terms of bug detection with one and three minutes.}
% % %\vspace{-1mm}
% % \end{figure*}
% % %%%%%%%%%%%
% Figure~\ref{fig:bug-detected-3minutes} highlights that in the experiments using project-specific inputs and all inputs, more bugs are detected in Apache Commons Codec, Apache Commons Csv, Jackson-core, and Jsoup. When exclusively utilizing project-specific inputs, more bugs are detected in Apache Commons Cli, Gson, and Apache Commons Math. However, experimenting with all inputs reveals a higher bug detection rate for JxPath. These findings indicate the efficacy of our approach in utilizing inputs extracted by \name, resulting in improved bug detection capabilities. Additionally, the observed reduction in the number of generated tests (Figure~\ref{fig:test-generated-3minutes}) while detecting more bugs demonstrates the efficiency and effectiveness of our approach. \par
% The experiments conducted highlight the significant benefits of incorporating inputs into the test generation process alongside EvoSuite's normal execution. Using inputs leads to the detection of a higher number of bugs compared to using EvoSuite alone. The experiments utilizing inputs detected 45 bugs, while only 13 bugs were detected without inputs. This demonstrates the effectiveness of incorporating inputs in improving EvoSuite's fault-detection capability. Additionally, combining test cases generated by EvoSuite with and without inputs resulted in the detection of 309 bugs, surpassing the bug-detection outcomes achieved by either approach individually. These findings emphasize the importance of leveraging both EvoSuite's automated test generation techniques and external inputs to achieve a more comprehensive and effective testing approach. This combination approach enhances test quality and increases bug detection rates by leveraging the strengths of EvoSuite's algorithmic capabilities and the contextual relevance provided by external inputs. \par
% \highlight{Summary of \textbf{RQ3:} Automatically generated test cases that utilize test input values extracted by \name consistently outperform the baseline approach which relies on randomly generated inputs in terms of bug detection, demonstrating the utility of \name and the overall benefit of mining bug report for test inputs.
% % By leveraging the contextual relevance provided by external inputs, the generated tests exhibit a higher ability to detect software defects, leading to enhanced test quality and increased fault-detection capability.
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{[RQ3]: Effect of \name-extracted inputs on bug detection rate}

\noindent\textbf{Experiment Goal: }The goal of this experiment is to evaluate the effectiveness of BRMiner in improving the bug detection capabilities of automated test generation tools, specifically EvoSuite and Randoop. We aim to assess how incorporating various input extraction strategies, including those derived from BRMiner, impacts the number of bugs detected compared to baseline scenarios where no inputs are used.

\noindent\textbf{Experiment Design:}\label{RQ3-experiment-design}
This experiment evaluates the effectiveness of BRMiner in enhancing the bug detection capabilities of automated test generation tools, specifically EvoSuite and Randoop. The objective is to determine whether the inputs extracted by BRMiner from bug reports can improve the performance of these tools in identifying software bugs compared to scenarios where no external inputs are used (NoLit).

We employed a regression testing scenario, a common practice in software testing, to assess the effectiveness of automatically generated test cases. In this approach, test cases are generated on a fixed version of the software where the bug has been resolved, and then these tests are executed on the buggy version to determine if they can detect the defect. This methodology allows us to use the behavior of the fixed version as a reliable oracle, addressing the challenge of determining whether a test has passed or failed (the oracle problem). While we acknowledge that this approach assumes the availability of a fixed version, it provides a controlled environment for a systematic comparison of different input strategies, making it a practical method for evaluating the contributions of BRMiner. In real-world scenarios, where a fixed version may not always be available, developers often manually verify the results, which is time-consuming. This highlights the importance of further research into automated test oracle generation, which we suggest as a future direction. The regression testing scenario used in this study is inspired by previous work~\citep{shamshiri2015automatically} that successfully applied this methodology to evaluate automatic test generation tools. The overall process, depicted in Figure~\ref{fig:bug-detection-methodology}, involves generating test cases on the fixed version of the software and then executing these tests on the buggy version to measure their bug detection effectiveness.

\begin{figure*}
  \centering
  %\includegraphics[width=0.8\textwidth]{Images/Bug-Detection-Experiments.pdf}
  \includegraphics[width=0.9\textwidth]{Images/Bug-Detection-Experiments.pdf}
   \caption{Overview of the methodology used to design the bugs detection experiments}
    \label{fig:bug-detection-methodology}
\end{figure*}

To assess the impact of BRMiner, we conducted experiments using the following input strategies:
\begin{itemize}
    \item \textbf{NoLit:} A baseline scenario where no specific inputs are provided to EvoSuite or Randoop.
    \item \textbf{ProjLit:} Uses project-specific literals extracted from bug reports.
    \item \textbf{AllLit:} Incorporates all literals from all projects.
    \item \textbf{ProjLitLLM:} Project-specific literals filtered through BRMiner with LLM.
    \item \textbf{AllLitLLM:} All project literals filtered through BRMiner with LLM.
    \item \textbf{ProjLitLLMOnly:} Inputs generated solely by LLM for each project.
    \item \textbf{AllLitLLMOnly:} Inputs generated solely by LLM across all projects.
\end{itemize}


In Table~\ref{table:bug-detection-results}, the terms "ProjLit" and "AllLit" refer to configurations where only the \textbf{Regex + Javalang} approach was used.
These configurations allow us to compare the effectiveness of using literals from different sources, both with and without the filtering and generation capabilities of LLM, to determine the most effective strategy for enhancing bug detection.

The experiments were conducted on the Defects4J dataset, featuring real-world software bugs across multiple projects. Test cases were generated using EvoSuite and Randoop under the various input strategies, with each experiment allocated a three-minute time budget per iteration over five iterations to ensure robust results. Certain projects, such as JacksonXml, Mockito, and Closure, were omitted from some experiments due to limitations in EvoSuite's ability to generate tests or issues with non-compilable test cases. Additionally, Randoop failed to execute tests for Compress, JacksonDatabind and JacksonXml, for Cli, Csv, and Math, it executed but did not generate error-revealing tests, influencing the overall bug detection outcomes.

We analyzed the number of bugs detected by each input strategy, the number of test cases generated, and the overlap of bugs detected across different strategies. This comprehensive analysis provides insights not only into the number of bugs detected but also into the specific contributions of BRMiner and its ability to enhance the effectiveness of automated test generation.


\noindent\textbf{Experiment Results: }
The results presented in Table~\ref{table:bug-detection-results} show that the use of inputs, especially when filtered through BRMiner, significantly enhances the bug detection capabilities of both EvoSuite and Randoop. The BRMiner approach, particularly in the \textbf{AllLitLLM} scenario, detected the highest number of bugs (\textbf{313 with EvoSuite and 111 with Randoop}) across all experiments, surpassing the baseline NoLit scenario (\textbf{295 with EvoSuite and 93 with Randoop}). In the EvoSuite experiments, the AllLitLLM scenario led to the detection of 313 bugs, the highest among all scenarios, demonstrating the effectiveness of using comprehensive, LLM-filtered inputs. The ProjLitLLM scenario also performed well, detecting 311 bugs, underscoring the value of project-specific inputs, while the baseline NoLit scenario detected 295 bugs, illustrating the substantial improvement brought by the use of extracted inputs. In the Randoop experiments, AllLitLLM and ProjLitLLM detected 111 and 107 bugs, respectively, outperforming the NoLit baseline, which detected 93 bugs. Although Randoop generally detected fewer bugs than EvoSuite, the integration of BRMiner inputs still provided significant improvements in bug detection. These results collectively demonstrate that integrating BRMiner, especially with LLM filtering, significantly enhances the effectiveness of automated test generation tools like EvoSuite and Randoop in detecting bugs.


%%%%%%%%%%%%%%%BUG DETECTED
\begin{table*}
    \centering
    %\caption{Bug detection results for different experiments}
    \caption{Comparison of bug detection effectiveness across different input strategies for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}

    \label{table:bug-detection-results}
    % \scriptsize
    %\scalebox{0.85}
    \scalebox{0.58}
    {
        \begin{tabular}{l|c|cccccccccccccc}
            \toprule
            & \textbf{\#Bugs} & \multicolumn{14}{c}{Bug Detection (\#)} \\
            \cmidrule{3-16}
            Projects & \textbf{} & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            &  & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 39 & 28 & 0 & \textbf{29} & 0 & 28 & 0 & 28 & 0 & \textbf{29} & 0 & 28 & 0 & \textbf{29} & 0 \\
            Codec & 18 & 10 & 9 & 11 & 10 & \textbf{12} & 11 & \textbf{12} & 11 & 11 & \textbf{12} & 11 & 10 & 11 & 10 \\
            Collections & 4 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
            Compress & 47 & 28 & -- & 27 & -- & 27 & -- & 28 & -- & 28 & -- & 28 & -- & 28 & -- \\
            Csv & 16 & 13 & 0 & 14 & 0& \textbf{15} & 0 & \textbf{15} & 0 & 14 & 0 & \textbf{15} & 0 & \textbf{15} & 0 \\
            Gson & 18 & 5 & 3 & \textbf{6} & 4 & 5 & 3 & 5 & 5 & \textbf{6} & 4 & 5 & 3 & 5 & 4 \\
            JacksonCore & 26 & 17 & 8 & 18 & 8 & \textbf{19} & 9 & \textbf{19} & 9 & \textbf{19} & 9 & 17 & 8 & 18 & 8 \\
            Databind & 112 & 4 & -- & 4 & -- & \textbf{5} & -- & \textbf{5} & -- & \textbf{5} & -- & \textbf{5} & -- & \textbf{5} & -- \\
            JacksonXml & 6 & 0 & -- & 0 & -- & 0 & -- & 0 & -- & 0 & -- & 0 & -- & 0 & -- \\
            Jsoup & 93 & 52 & 35 & 55 & 37 & \textbf{59} & 41 & \textbf{59} & 41 & \textbf{59} & 44 & 54 & 35 & 54 & 35 \\
            JxPath & 22 & 17 & 8 & 17 & 8 & \textbf{19} & 9 & \textbf{19} & 8 & \textbf{19} & 9 & 17 & 8 & 17 & 9 \\
            Lang & 64 & 40 & 22 & \textbf{41} & 23 & 40 & 22 & 40 & 23 & \textbf{41} & 23 & 40 & \textbf{41} & \textbf{41} & 23 \\
            Math & 106 & 70 & 0 & \textbf{71} & 0 & 67 & 0 & 70 & 0 & \textbf{71} & 0 & 70 & 0 & \textbf{71} & 0 \\
            Time & 26 & 10 & 7 & 10 & 8 & 10 & 9 & 10 & 9 & 10 & 9 & 10 & 9 & 10 & 9 \\
            \midrule
            \textbf{Total} & 597 & 295 & 93 & 304 & 99 & 307 & 105 & 311 & 107 & \textbf{313} & 111 & 301 & 96 & 305 & 99 \\
            \bottomrule
        \end{tabular}
    }
    \vspace{2mm}
\end{table*}

In Table~\ref{generated-tests-results}, we observe a clear relationship between the number of tests generated and the number of bugs detected across different scenarios. In EvoSuite, the AllLitLLM scenario, despite generating fewer tests (144\,248), detected the highest number of bugs (313), demonstrating an efficient balance between test generation and bug detection. The ProjLitLLM scenario generated slightly more tests (145\,291) but detected slightly fewer bugs (311). Conversely, the baseline NoLit scenario generated the most tests (148\,246) yet detected fewer bugs (295), indicating lower efficiency in converting tests into detected bugs. Similar trends were observed in Randoop, where AllLitLLM generated fewer tests (6\,294) but detected the most bugs (111), while the NoLit scenario generated the most tests (6\,568) but detected fewer bugs (93).These results underscore the importance of using well-filtered inputs, which lead to more efficient and effective test generation, as evidenced by higher bug detection rates with fewer generated tests.
%%%%%%%%%%%%%%%TEST GENERATED
\begin{table*}
    \centering
    \caption{Number of generated tests and number of detected bugs with a time budget of three minutes and five iterations for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}
    \label{generated-tests-results}
    %\scriptsize
    %\scalebox{0.90}
    \scalebox{0.51}
    {
        \begin{tabular}{l|cccccccccccccc}
            \toprule
            & \multicolumn{14}{c}{Generated Tests (\#)} \\
            \cmidrule{2-15}
            Projects & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 2059 & 0 & 1818 & 0 & 1853 & 0 & 1811 & 0 & 1782 & 0 & 1826 & 0 & 1834 & 0 \\
            Codec & 5946 & 523 & 6112 & 550 & 6113 & 563 & 6068 & 530 & 6050 & 535 & 6106 & 563 & 6108 & 560 \\
            Collections & 19528 & 391 & 18899 & 460 & 19884 & 454 & 19842 & 395 & 19813 & 391 & 19857 & 455 & 19865 & 454 \\
            Compress & 22010 & -- & 21672 & -- & 21887 & -- & 21755 & -- & 21771 & -- & 21793 & -- & 21812 & -- \\
            Csv & 1149 & 0 & 1127 & 0 & 1068 & 0 & 1073 & 0 & 1020 & 0 & 1109 & 0 & 1095 & 0 \\
            Gson & 4568 & 1741 & 4438 & 2285 & 4331 & 2387 & 4360 & 1850 & 4295 & 1800 & 4372 & 1950 & 4364 & 1735 \\
            JacksonCore & 18472 & 376 & 17836 & 384 & 17390 & 489 & 17558 & 323 & 17424 & 350 & 17521 & 370 & 17503 & 365 \\
            Databind & 3001 & -- & 3671 & -- & 2984 & -- & 3303 & -- & 21952 & -- & 3273 & -- & 22011 & -- \\
            JacksonXml & 207 & -- & 184 & -- & 247 & -- & 191 & -- & 169 & -- & 210 & -- & 219 & -- \\
            Jsoup & 9151 & 676 & 10524 & 748 & 10470 & 587 & 10432 & 730 & 10401 & 535 & 10447 & 755 & 10454 & 634 \\
            JxPath & 11783 & 12 & 11373 & 12 & 11041 & 12 & 11182 & 12 & 11062 & 12 & 11237 & 12 & 11179 & 12 \\
            Lang & 23639 & 455 & 22439 & 449 & 21613 & 497 & 21956 & 423 & 21735 & 433 & 21968 & 449 & 21881 & 443 \\
            Math & 4759 & 0 & 3791 & 0 & 3729 & 0 & 3735 & 0 & 3682 & 0 & 3739 & 0 & 3740 & 0 \\
            Time & 21974 & 2797 & 22073 & 3241 & 21995 & 3443 & 22009 & 2875 & 21952 & 2641 & 22011 & 2833 & 22011 & 2739 \\
            \midrule
            \textbf{Generated Tests (\#)} & 148246 & 6568 & 146957 & 7617 & 144605 & 7966 & 145291 & 6731 & \textbf{144248} & 6294 & 145468 & 6920 & 145278 & 6476 \\
            \textbf{Bugs Detected (\#)} & 295 & 138 & 304 & 145 & 307 & 147 & 311 & 153 & \textbf{313} & 157 & 301 & 142 & 305 & 144 \\
            \bottomrule
        \end{tabular}
    }
    \vspace{2mm}
\end{table*}

Table~\ref{evo-randoop-intersections-results} presents the unique and intersection-based bug detection results, highlighting the effectiveness of the BRMiner approach. In EvoSuite, the AllLitLLM scenario detected all 13 bugs uniquely identified by the NoLit scenario in the Regex + Javalang configuration, along with additional unique bugs. BRMiner's ProjLitLLM and AllLitLLM scenarios detected all the bugs found by other approaches, including the unique bugs identified by Regex + Javalang. Similarly, in Randoop, BRMiner detected all the bugs captured by the NoLit and other configurations, demonstrating the robustness and comprehensiveness of the BRMiner approach. These findings underscore the superiority of BRMiner, particularly when combined with LLM filtering, in detecting a wide range of bugs, including those that might be overlooked by traditional methods.

%%%%%%%%%%%%%%%INTERSECTION
% \begin{table*}
%     \centering
%     \caption{Analysis of unique and intersection-based bug detection across different input strategies. \textbf{NoLit}: Bugs detected without using any input literals. 
% \textbf{ProjLit}: Bugs detected using only literals extracted from ProjLit (project literals). 
% \textbf{AllLit}: Bugs detected using only literals extracted from AllLit (all literals). 
% \textbf{P $\cap$ A}: Bugs detected using literals that intersect between ProjLit and AllLit. 
% \textbf{P $\cap$ N}: Bugs detected using literals that intersect between ProjLit and NoLit. 
% \textbf{N $\cap$ A}: Bugs detected using literals that intersect between NoLit and AllLit. 
% \textbf{N $\cap$ P $\cap$ A}: Bugs detected using literals that intersect among NoLit, ProjLit, and AllLit.}
   
%     \label{evo-randoop-intersections-results}
%     %\scalebox{0.75}
%     % Sous-tableau pour EvoSuite
%     %\begin{subtable}{0.85\textwidth} %{\textwidth}
%     \begin{subtable}{\textwidth}
%     \centering
%     \caption{Intersection and unique bug detection results for EvoSuite}
%     \label{result-with-&-without-regex}
%     \scalebox{0.5}{
%         \begin{tabular}{@{}l|ccccccc|ccccccc|ccccccc@{}}
%             \toprule
%             & \multicolumn{7}{c|}{Regex + Javalang} & \multicolumn{7}{c|}{BRMiner} & \multicolumn{7}{c}{LLM Alone} \\
%             \cmidrule{2-22}
%             Projects & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} \\
%             \midrule
%             Cli & 1 & 0 & 1 & 2 & 1 & 1 & 25 & 0 & 0 & 1 & 0 & 0 & 0 & 28 & 0 & 0 & 1 & 1 & 0 & 0 & 28 \\
%             Codec & 0 & 2 & 1 & 0 & 0 & 0 & 11 & 0 & 1 & 0 & 1 & 0 & 0 & 10 & 0 & 0 & 0 & 1 & 0 & 0 & 11 \\
%             Collections & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
%             Compress & 1 & 1 & 0 & 1 & 1 & 1 & 23 & 0 & 0 & 0 & 0 & 0 & 0 & 28 & 1 & 0 & 0 & 0 & 0 & 0 & 27 \\
%             Csv & 0 & 1 & 0 & 1 & 0 & 0 & 13 & 0 & 1 & 0 & 1 & 0 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 13 \\
%             Gson & 0 & 0 & 1 & 0 & 0 & 0 & 5 & 0 & 0 & 1 & 0 & 0 & 0 & 5 & 0 & 0 & 0 & 0 & 0 & 0 & 5 \\
%             JacksonCore & 1 & 2 & 0 & 1 & 0 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 17 & 1 & 0 & 1 & 0 & 0 & 0 & 17 \\
%             Databind & 0 & 1 & 0 & 0 & 0 & 0 & 4 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 1 & 0 & 0 & 4 \\
%             JacksonXml & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%             Jsoup & 3 & 2 & 1 & 8 & 4 & 1 & 42 & 0 & 0 & 0 & 7 & 0 & 0 & 52 & 1 & 0 & 0 & 2 & 0 & 0 & 52 \\
%             JxPath & 1 & 1 & 1 & 2 & 2 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 17 & 1 & 0 & 0 & 0 & 0 & 0 & 17 \\
%             Lang & 3 & 1 & 1 & 4 & 1 & 6 & 34 & 0 & 0 & 1 & 0 & 0 & 0 & 40 & 0 & 0 & 1 & 0 & 0 & 0 & 40 \\
%             Math & 3 & 1 & 5 & 3 & 10 & 14 & 57 & 0 & 0 & 1 & 0 & 0 & 0 & 70 & 2 & 0 & 1 & 5 & 0 & 0 & 64 \\
%             Time & 0 & 0 & 0 & 0 & 0 & 0 & 10 & 0 & 0 & 0 & 0 & 0 & 0 & 10 & 0 & 0 & 0 & 0 & 0 & 0 & 10 \\
%             \midrule
%             Total/Average & 13 & 12 & 11 & 22 & 19 & 23 & 251 & 0 & 2 & 4 & 14 & 0 & 0 & 295 & 6 & 0 & 4 & 12 & 0 & 0 & 289 \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{subtable}

%     \vspace{1cm} % Espace entre les deux sous-tableaux

%     % Sous-tableau pour Randoop
%     \begin{subtable}{\textwidth}
%     \centering
%     \caption{Intersection and unique bug detection results for Randoop}
%     \label{result-with-&-without-regex-randoop}
%     \scalebox{0.5}{
%         \begin{tabular}{@{}l|ccccccc|ccccccc|ccccccc@{}}
%             \toprule
%             & \multicolumn{7}{c|}{Regex + Javalang} & \multicolumn{7}{c|}{BRMiner} & \multicolumn{7}{c}{LLM Alone} \\
%             \cmidrule{2-22}
%             Projects & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} \\
%             \midrule
%             Cli & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%             Codec & 0 & 0 & 1 & 1 & 0 & 0 & 9 & 0 & 1 & 2 & 1 & 0 & 0 & 9 & 0 & 0 & 0 & 1 & 0 & 0 & 9 \\
%             Collections & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
%             Csv & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%             Gson & 0 & 1 & 0 & 0 & 0 & 0 & 3 & 0 & 2 & 1 & 0 & 0 & 0 & 3 & 0 & 0 & 1 & 0 & 0 & 0 & 3 \\
%             JacksonCore & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 0 & 1 & 0 & 0 & 8 & 0 & 0 & 0 & 0 & 0 & 0 & 8 \\
%             Jsoup & 1 & 0 & 7 & 2 & 0 & 0 & 35 & 0 & 5 & 8 & 1 & 0 & 0 & 35 & 0 & 0 & 0 & 0 & 0 & 0 & 35 \\
%             JxPath & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 1 & 0 & 0 & 0 & 8 \\
%             Lang & 0 & 1 & 0 & 0 & 0 & 0 & 22 & 0 & 0 & 0 & 1 & 0 & 0 & 22 & 0 & 0 & 1 & 0 & 0 & 0 & 22 \\
%             Math & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%             Time & 0 & 0 & 1 & 1 & 0 & 0 & 7 & 0 & 1 & 1 & 1 & 0 & 0 & 7 & 0 & 1 & 1 & 1 & 0 & 0 & 7 \\
%             \midrule
%             Total & 1 & 2 & 11 & 4 & 0 & 0 & 93 & 0 & 9 & 13 & 5 & 0 & 0 & 93 & 0 & 1 & 4 & 2 & 0 & 0 & 93 \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{subtable}

% \end{table*}
\begin{table*}
    \centering
    \caption{Analysis of unique and intersection-based bug detection across different input strategies. \textbf{NoLit}: Bugs detected without using any input literals. 
\textbf{ProjLit}: Bugs detected using only literals extracted from ProjLit (project literals). 
\textbf{AllLit}: Bugs detected using only literals extracted from AllLit (all literals). 
\textbf{P $\cap$ A}: Bugs detected using literals that intersect between ProjLit and AllLit. 
\textbf{P $\cap$ N}: Bugs detected using literals that intersect between ProjLit and NoLit. 
\textbf{N $\cap$ A}: Bugs detected using literals that intersect between NoLit and AllLit. 
\textbf{N $\cap$ P $\cap$ A}: Bugs detected using literals that intersect among NoLit, ProjLit, and AllLit.}
   
    \label{evo-randoop-intersections-results}
    %\scalebox{0.75}
    
    % Sous-tableau pour EvoSuite
    %\begin{subtable}{0.85\textwidth} %{\textwidth}
    %\begin{subtable}{\textwidth} %{\textwidth}
    
    % \centering
    %\caption{Intersection and unique bug detection results for EvoSuite}
    % \label{result-with-&-without-regex}
    % \scalebox{0.5}{
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}l|ccccccc|ccccccc|ccccccc@{}}
            \toprule
            \multicolumn{22}{c}{\textbf{Intersection and unique bug detection results for EvoSuite}} \\
            \midrule
            & \multicolumn{7}{c|}{Regex + Javalang} & \multicolumn{7}{c|}{BRMiner} & \multicolumn{7}{c}{LLM Alone} \\
            \cmidrule{2-22}
            Projects & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} \\
            \midrule
            Cli & 1 & 0 & 1 & 2 & 1 & 1 & 25 & 0 & 0 & 1 & 0 & 0 & 0 & 28 & 0 & 0 & 1 & 1 & 0 & 0 & 28 \\
            Codec & 0 & 2 & 1 & 0 & 0 & 0 & 11 & 0 & 1 & 0 & 1 & 0 & 0 & 10 & 0 & 0 & 0 & 1 & 0 & 0 & 11 \\
            Collections & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
            Compress & 1 & 1 & 0 & 1 & 1 & 1 & 23 & 0 & 0 & 0 & 0 & 0 & 0 & 28 & 1 & 0 & 0 & 0 & 0 & 0 & 27 \\
            Csv & 0 & 1 & 0 & 1 & 0 & 0 & 13 & 0 & 1 & 0 & 1 & 0 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 13 \\
            Gson & 0 & 0 & 1 & 0 & 0 & 0 & 5 & 0 & 0 & 1 & 0 & 0 & 0 & 5 & 0 & 0 & 0 & 0 & 0 & 0 & 5 \\
            JacksonCore & 1 & 2 & 0 & 1 & 0 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 17 & 1 & 0 & 1 & 0 & 0 & 0 & 17 \\
            Databind & 0 & 1 & 0 & 0 & 0 & 0 & 4 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 1 & 0 & 0 & 4 \\
            JacksonXml & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
            Jsoup & 3 & 2 & 1 & 8 & 4 & 1 & 42 & 0 & 0 & 0 & 7 & 0 & 0 & 52 & 1 & 0 & 0 & 2 & 0 & 0 & 52 \\
            JxPath & 1 & 1 & 1 & 2 & 2 & 0 & 13 & 0 & 0 & 0 & 2 & 0 & 0 & 17 & 1 & 0 & 0 & 0 & 0 & 0 & 17 \\
            Lang & 3 & 1 & 1 & 4 & 1 & 6 & 34 & 0 & 0 & 1 & 0 & 0 & 0 & 40 & 0 & 0 & 1 & 0 & 0 & 0 & 40 \\
            Math & 3 & 1 & 5 & 3 & 10 & 14 & 57 & 0 & 0 & 1 & 0 & 0 & 0 & 70 & 2 & 0 & 1 & 5 & 0 & 0 & 64 \\
            Time & 0 & 0 & 0 & 0 & 0 & 0 & 10 & 0 & 0 & 0 & 0 & 0 & 0 & 10 & 0 & 0 & 0 & 0 & 0 & 0 & 10 \\
            \midrule
            Total/Average & 13 & 12 & 11 & 22 & 19 & 23 & 251 & 0 & 2 & 4 & 14 & 0 & 0 & 295 & 6 & 0 & 4 & 12 & 0 & 0 & 289 \\
            \bottomrule
        \end{tabular}
    }
%\end{subtable}

    \vspace{3mm} % Espace entre les deux sous-tableaux

    % Sous-tableau pour Randoop
    % \begin{subtable}{\textwidth}
    % \centering
    %\caption{Intersection and unique bug detection results for Randoop}
    % \label{result-with-&-without-regex-randoop}
    % \scalebox{0.5}{
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}l|ccccccc|ccccccc|ccccccc@{}}
            \toprule
            \multicolumn{22}{c}{\textbf{Intersection and unique bug detection results for Randoop}} \\
            \midrule
            & \multicolumn{7}{c|}{Regex + Javalang} & \multicolumn{7}{c|}{BRMiner} & \multicolumn{7}{c}{LLM Alone} \\
            \cmidrule{2-22}
            Projects & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} & \makecell{No\\Lit} & \makecell{Proj\\Lit} & \makecell{All\\Lit} & \makecell{P\\$\cap$\\A} & \makecell{P\\$\cap$\\N} & \makecell{N\\$\cap$\\A} & \makecell{N\\$\cap$\\P\\$\cap$\\A} \\
            \midrule
            Cli & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
            Codec & 0 & 0 & 1 & 1 & 0 & 0 & 9 & 0 & 1 & 2 & 1 & 0 & 0 & 9 & 0 & 0 & 0 & 1 & 0 & 0 & 9 \\
            Collections & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
            Csv & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
            Gson & 0 & 1 & 0 & 0 & 0 & 0 & 3 & 0 & 2 & 1 & 0 & 0 & 0 & 3 & 0 & 0 & 1 & 0 & 0 & 0 & 3 \\
            JacksonCore & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 0 & 1 & 0 & 0 & 8 & 0 & 0 & 0 & 0 & 0 & 0 & 8 \\
            Jsoup & 1 & 0 & 7 & 2 & 0 & 0 & 35 & 0 & 5 & 8 & 1 & 0 & 0 & 35 & 0 & 0 & 0 & 0 & 0 & 0 & 35 \\
            JxPath & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 1 & 0 & 0 & 0 & 8 \\
            Lang & 0 & 1 & 0 & 0 & 0 & 0 & 22 & 0 & 0 & 0 & 1 & 0 & 0 & 22 & 0 & 0 & 1 & 0 & 0 & 0 & 22 \\
            Math & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
            Time & 0 & 0 & 1 & 1 & 0 & 0 & 7 & 0 & 1 & 1 & 1 & 0 & 0 & 7 & 0 & 1 & 1 & 1 & 0 & 0 & 7 \\
            \midrule
            Total & 1 & 2 & 11 & 4 & 0 & 0 & 93 & 0 & 9 & 13 & 5 & 0 & 0 & 93 & 0 & 1 & 4 & 2 & 0 & 0 & 93 \\
            \bottomrule
        \end{tabular}
    }
%\end{subtable}


\end{table*}










Table~\ref{unique-bug-detection}  highlights the unique bugs detected using inputs exclusively extracted by BRMiner. The BRMiner approach detected 58 unique bugs that were not detected by other methods, with 13 of these bugs being uniquely identified by BRMiner alone. This finding solidifies the argument that BRMiner significantly improves the detection of unique and hard-to-find bugs, which are critical for ensuring software robustness.

%%%%%%%%%%%%%%%INTERSECTION UNIQUE
\begin{table*}[ht]
    \centering
    \caption{Unique bugs detected (58) using only the extracted inputs from BRMiner and Regex + Javalang across various projects by Bug-ID. This table presents bugs uniquely detected using specific input literals (ProjLit, AllLit, and P $\cap$ A). Bugs marked with an asterisk (*) were detected exclusively by BRMiner (13 bugs), while the rest were found by both BRMiner and Regex + Javalang. A value of 1 indicates detection in at least one of five iterations, while 0 indicates no detection.}
    \label{unique-bug-detection}
    \scalebox{0.82}{
        \begin{tabular}{@{}l|ccc|l|ccc@{}}
            \toprule
            \textbf{Bug-ID} & \textbf{ProjLit} & \textbf{AllLit} & \textbf{P $\cap$ A} & \textbf{Bug-ID} & \textbf{ProjLit} & \textbf{AllLit} & \textbf{P $\cap$ A} \\
            \midrule
            Cli-12 & 0 & 0 & 1 & Jsoup-13 & 0 & 0 & 1 \\
            Cli-26* & 0 & 0 & 1 & Jsoup-34 & 0 & 0 & 1 \\
            Cli-28 & 0 & 1 & 0 & Jsoup-48 & 0 & 0 & 1 \\
            Cli-33 & 0 & 0 & 1 & Jsoup-51 & 0 & 0 & 1 \\
            Cli-36 & 0 & 0 & 1 & Jsoup-54 & 0 & 1 & 0 \\
            Cli-7* & 0 & 1 & 0 & Jsoup-6 & 0 & 0 & 1 \\
            Cli-9* & 1 & 0 & 0 & Jsoup-67 & 1 & 0 & 0 \\
            Codec-1* & 0 & 0 & 1 & Jsoup-73 & 0 & 0 & 1 \\
            Codec-16 & 1 & 0 & 0 & Jsoup-80 & 0 & 0 & 1 \\
            Codec-3 & 0 & 1 & 0 & JxPath-1 & 0 & 1 & 0 \\
            Codec-8* & 0 & 1 & 0 & JxPath-11 & 1 & 0 & 0 \\
            Compress-15 & 0 & 0 & 1 & JxPath-2 & 0 & 0 & 1 \\
            Compress-32* & 0 & 0 & 1 & JxPath-20 & 0 & 0 & 1 \\
            Compress-39* & 0 & 0 & 1 & Lang-20 & 0 & 0 & 1 \\
            Compress-47 & 1 & 0 & 0 & Lang-24 & 0 & 1 & 0 \\
            Csv-15 & 1 & 0 & 0 & Lang-31* & 0 & 0 & 1 \\
            Csv-7 & 0 & 0 & 1 & Lang-42 & 0 & 0 & 1 \\
            Gson-11 & 0 & 1 & 0 & Lang-58 & 0 & 0 & 1 \\
            Gson-15* & 1 & 0 & 0 & Lang-60 & 1 & 0 & 0 \\
            Gson-6* & 0 & 1 & 0 & Lang-62 & 0 & 0 & 1 \\
            JacksonCore-12 & 1 & 0 & 0 & Math-104 & 0 & 1 & 0 \\
            JacksonCore-13 & 0 & 0 & 1 & Math-105 & 0 & 1 & 0 \\
            JacksonCore-21 & 1 & 0 & 0 & Math-17 & 0 & 1 & 0 \\
            JacksonCore-24* & 0 & 1 & 0 & Math-2 & 0 & 0 & 1 \\
            JacksonCore-26* & 0 & 0 & 1 & Math-43 & 0 & 1 & 0 \\
            JacksonDatabind-16 & 1 & 0 & 0 & Math-48 & 0 & 1 & 0 \\
            Jsoup-10* & 0 & 0 & 1 & Math-50 & 0 & 1 & 0 \\
            Jsoup-12 & 1 & 0 & 0 & Math-72 & 0 & 0 & 1 \\
            Math-79 & 1 & 0 & 0 & Math-86 & 0 & 0 & 1 \\
            \midrule
            & \multicolumn{2}{c}{\textbf{ProjLit}} & \multicolumn{2}{c}{\textbf{AllLit}} & \multicolumn{2}{c}{\textbf{P $\cap$ A}} \\
            \midrule
            \textbf{Total} & \textbf{13} & & & \textbf{16} & \textbf{29} &   \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

\highlight{Summary of \textbf{RQ3:} BRMiner, particularly when integrated with LLM filtering, consistently outperforms others input extraction methods (Regex + Javalang, LLM Alone) in terms of bug detection. Specifically, BRMiner detected 58 unique bugs that were missed by NoLit, including 13 bugs that were uniquely identified by BRMiner alone. Additionally, BRMiner achieved higher bug detection efficiency, requiring fewer generated tests to achieve these results. This enhanced bug detection capability underscores the value of mining bug reports for test inputs and integrating advanced filtering techniques. As a result, BRMiner significantly improves the effectiveness of automated test generation tools like EvoSuite and Randoop, making it a powerful tool in the software testing process.
}


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{[RQ4]: Effect of \name-extracted inputs on code coverage}
% %\subsection{[RQ4]: Does the utilization of extracted relevant inputs by \name result in higher code coverage compared to tests generated without using these inputs?}
% \noindent\textbf{Experiment Goal: }The objective of this experiment is to assess the adequacy of automatically generated test cases using inputs extracted by \name. The evaluation aims to determine whether the inclusion of extracted inputs from bug reports improves the adequacy of the generated tests compared to scenarios where such inputs are not utilized. To conduct this evaluation, we also compare two different test generation scenarios: one where test cases are generated without the incorporation of extracted inputs (baseline scenario) and another where the extracted inputs from bug reports are integrated into the test generation process. \par
% % Through this experiment, we aim to determine whether the incorporation of inputs extracted by \name enhances the adequacy of the automatically generated test cases.
% \noindent\textbf{Experiment Design: }To assess test adequacy in our study, we employed coverage metrics, specifically code coverage and requirements coverage. These metrics quantitatively measure how much the test suite exercises the code or requirements of the software system. We focused on code coverage metrics, including branch, instruction, method, and line coverage.

% As in Section~\ref{RQ3-experiment-design}, we conducted three experiments using EvoSuite on selected Defects4J projects to evaluate test adequacy. Each experiment varied in the inputs provided to EvoSuite: generating tests with no literals (\nolit), generating tests with project-specific literals (\projlit), and generating tests with literals extracted from all projects (\alllit).
% % \begin{comment}
% %     As in section \ref{RQ3-experiment-design}, we conducted three experiments using EvoSuite on selected Defects4J projects to evaluate test adequacy. Each experiment varied in the inputs provided to EvoSuite: generating tests without literals (EXP-1), generating tests with project-specific literals (EXP-2), and generating tests with literals extracted from all projects (EXP-3).
% % \end{comment}
% Each class had a 3-minute time limit, and the experimental setup was the same as in Section~\ref{RQ3-experiment-design}. To ensure reliable results, we executed each experiment five times and aggregated the results. We used Jacoco\footnote{https://github.com/jacoco/jacoco}, a widely used coverage measurement tool in the literature, to measure code coverage.

% For this experiment, we selected some recent versions of the same projects in the Defects4J dataset. 
% The selected projects and their versions are as follows: Apache Commons Cli 1.5.0, Apache Commons Codec 1.15, Apache Commons Collections 4-4.4, Apache Commons Compress 1.2.1, Apache Commons Csv 1.9.0, Gson 2.9.1, Jackson-core 2.14-rc2, Jackson-dataformat-xml 2.14.0-rc2, Jackson-databind 2.14.0-rc2, Jsoup 1.15.3, Apache Commons Jxpath 1.3, Apache Commons Lang 3-3.12.0, Mockito 4.8.1, Joda Time 2.12.0.
% We excluded projects Closure and Math because either Evosuite crashed, failed to generate tests, or generated uncompilable tests.

% Using these methodologies, tools, and recent versions of the projects, we can assess test adequacy in terms of code coverage for each experiment and evaluate the impact of different inputs on the achieved coverage. Additionally, we aim to evaluate the effectiveness and performance of our approach using up-to-date code bases. \par
% \begin{table*}
%     \centering
%     \caption{Results of the code coverage measurements using branch coverage, instruction coverage, method coverage, and line coverage}
%     \label{code-coverage-results}
%     % \vspace{-3mm}
%     \scalebox{0.57}
% {
%     \begin{tabular}{lrrr|rrr|rrr|rrr}
%         \toprule
%         & \multicolumn{3}{c|}{Branch coverage (\%)} & \multicolumn{3}{c|}{Instruction coverage (\%)} & \multicolumn{3}{c|}{Method coverage (\%)} & \multicolumn{3}{c}{Line coverage (\%)} \\
%         \cmidrule{2-13}
%         %Project & EXP1 & EXP2 & EXP3 & EXP1 & EXP2 & EXP3 & EXP1 & EXP2 & EXP3 & EXP1 & EXP2 & EXP3\\
%         Project & \nolit & \projlit & \alllit & \nolit & \projlit & \alllit & \nolit & \projlit & \alllit & \nolit & \projlit & \alllit \\

% \midrule
%         Cli & 50.0 &  49.4  &  49.8  &  96.2  &  \textbf{97.8}  &  \textbf{97.8}  &  99.8  & \textbf{100.0} & \textbf{100.0} &  96.7  &  \textbf{97.9}  &  \textbf{98.1}  \\
%         Codec & 38.0 &  \textbf{38.8}  &  \textbf{40.6}  &  86.6  &  \textbf{86.8}  &  \textbf{88.4}  &  98.5  &  98.2  &  98.3  &  85.2  &  \textbf{85.9} &  \textbf{87.2}   \\
%         Collections & 47.0 &  \textbf{48.8}  &  \textbf{48.2}  &  94.4  &  \textbf{95.2}  &  \textbf{94.8}  &  99.7  & \textbf{100.0} & \textbf{100.0} &  93.9  &  \textbf{95.6}  &  \textbf{95.0}  \\
%         Compress &  49.2  & 48.6 &  49.0  &  95.2  & \textbf{96.6} &  \textbf{96.0}  &  100.0  &  100.0  &  99.9  &  94.7  &  \textbf{96.5}  &  \textbf{96.5}  \\
%         Csv & 50.0 & 50.0 & 50.0 & 99.0 & 99.0 & 99.0 & 100.0 & 99.9 &  100.0  &  99.5  &  \textbf{99.6}  &  \textbf{99.6}  \\
%         Gson &  48.8  & \textbf{49.0} & \textbf{49.0} &  94.6  &  \textbf{95.4}  &  \textbf{95.4}  & 100.0 & 100.0 & 100.0 &  93.0  &  \textbf{95.1}  &  \textbf{95.3}  \\
%         JacksonCore &  49.8  &  49.4  &  49.6  &  96.8  &  \textbf{98.4}  &  \textbf{98.2}  &  99.8  & \textbf{100.0} & \textbf{100} &  95.9  &  \textbf{98.7}  &  \textbf{98.6}  \\
%         JacksonXml & 50.0 & 50.0 & 50.0 &  96.4  &  \textbf{97.2}  &  \textbf{96.6}  & 100.0 & 100.0 & 100.0 &  99.1  &  \textbf{99.3}  &  \textbf{99.4}  \\
%         Jsoup &  49.4  &  \textbf{49.6}  &  49.2  &  96.8  & \textbf{98.0} & \textbf{98.0} &  99.9  & \textbf{100.0} & \textbf{100} &  96.3  &  \textbf{98.6}  &  \textbf{98.5}  \\
%         JxPath &  48.8  &  48.2  &  48.2  &  95.4  & \textbf{96.6} &  \textbf{96.0}  &  100.0  &  100.0  & 99.8 &  94.7  &  \textbf{96.9}  &  \textbf{96.1}  \\
%         Lang &  49.4  & 49.0 &  49.2  &  96.2  &  96.2  &  \textbf{96.4}  &  100.0  &  98.3  &  100.0  &  96.5  &  \textbf{96.9}  &  \textbf{96.9}  \\
%         Mockito & 50.0 &  49.8  &  49.4  &  96.8  & \textbf{97.0} & \textbf{97.0} &  99.8  &  99.8  &  99.6  &  96.3  &  \textbf{97.9}  &  \textbf{98.0}  \\
%         JacksonDatabind & 50.0 & 50.0 & 50.0 &  96.4  &  \textbf{97.2}  &  \textbf{97.4}  & 100.0 & 100.0 & 100.0 &  96.9  &  \textbf{98.0}  &  \textbf{98.2}  \\
%         Time &  48.4  &  48.4  &  48.4  &  95.8  &  \textbf{96.0}  & 95.8 &  100.0  &  100.0  &  100.0  &  96.0  &  \textbf{96.3}  &  \textbf{96.9}  \\
% \bottomrule
%     \end{tabular}
% }
% \end{table*}

% \noindent\textbf{Experiment Results: }Table~\ref{code-coverage-results} presents the results of the various experiments in terms of code coverage metrics, including branch coverage, instruction coverage, method coverage, and line coverage. These metrics were measured for the three experiments conducted with no literals (\nolit), with project-specific literals (\projlit), and with all literals (\alllit). The results are compared to the baseline, which represents the experiment conducted without inputs. In the following paragraphs we will first analyse  the different results from the code coverage experiments in term of branch coverage, instruction coverage, method coverage and line coverage. Then we will comment these results. \par
% % \begin{comment}
% %     Table ~\ref{code-coverage-results} presents the results of the various experiments in terms of code coverage metrics, including branch coverage, instruction coverage, method coverage, and line coverage. These metrics were measured for the three experiments conducted without inputs (EXP-1), with project-specific inputs (EXP-2), and with all inputs. The results are compared to the baseline, which represents the experiment conducted without inputs.
% % \end{comment}
% In terms of \textbf{branch coverage}, using mined inputs improves coverage by 2.6\% and 1.2\%  for the Codec and Collections projects, respectively. The Gson project showed a minor improvement of 0.2\%. For the remaining projects, there was a slight drop in coverage rates, except for CSV, JacksonXml, JacksonDatabind, and Joda Time, where no change was observed compared to the baseline. When using all inputs, the Collections project exhibited an improvement of 1.8\%. The Codec, Gson, and Jsoup projects also showed slight improvements. However, for CSV, JacksonXml, JacksonDatabind, and Joda Time, there was no change compared to the baseline. For the other projects, we observe a slight drop in coverage.

% Regarding \textbf{instruction coverage}, the experiment using project specific inputs resulted in improvements of 1.4\% and 1.47\% for Cli and JacksonCore projects, respectively. Similarly, when all inputs were used, improvements were observed for the Cli, JacksonCore, and Jsoup projects. With specific inputs, an improvement of 1.8\% was observed for the Codec project, and 1\% for JacksonDatabind. Except for CSV and Joda Time, which showed no change, the rest of the projects exhibited slight improvements. When using all inputs, an improvement of 1.2\% was observed for the JxPath project. With the exception of CSV and Lang, which showed no change, the other projects showed slight improvements.

% For \textbf{method coverage}, the experiment using specific inputs resulted in a slight improvement in coverage for the Cli, Collections, JacksonCore, Jsoup, and Lang projects. For CSV, Gson, JacksonXml, JacksonDatabind, and Time projects, there was no change compared to the baseline. However, the Codec, Compress, JxPath, and Mockito projects experienced a slight drop in coverage. When using all inputs, slight improvements were observed for the Cli, Collections, JacksonCore, Jsoup, JxPath, Mockito, and Joda Time projects. For Gson, JacksonXml, and JacksonDatabind, no change was observed compared to the baseline. However, there was a slight drop in coverage for the Codec, Compress, CSV, and Lang projects.

% In terms of \textbf{line coverage}, the experiments using inputs extracted by \name showed improvements across all projects. Projects such as Gson, JacksonCore, and Jsoup exhibited an average increase in line coverage of at least 2\%. The experiment using specific inputs resulted in an average improvement of 1.54\% for projects such as Cli, Codec, Collections, Compress, JxPath, Mockito, and JacksonDatabind. When using all inputs, there was a slight improvement for the Apache Commons Codec project, and an average improvement of 1.52\% for the Cli, Collections, Compress, Mockito, and JacksonDatabind projects. The JxPath project showed an increase of 2.24\% when all inputs were used. However, there was only a slight improvement for the Apache Commons Csv, Jackson-dataformat-xml, Apache Commons Lang, and Joda Time projects.

% Overall, the results for instruction and line coverage are quite interesting, as EvoSuite already achieves high levels of coverage by default. The improvements observed, whether slight or significant, indicate the potential of combining our approach with the baseline to increase the code coverage rate.


% \highlight{Summary of \textbf{RQ4:} Across various projects, the integration of \name-extracted inputs in the test generation process led to an average improvement of approximately 1.15\% in branch coverage, 1.17\% in instruction coverage, and  1.25\% in line coverage, with notable increases in specific projects like 'Codec' (up to 2.6\%) and 'JxPath' (up to 2.24\%). These enhancements, although seemingly modest, are critical for bug detection, as they help uncover potential defects and edge cases, thereby improving software quality and reliability. This improvement is particularly significant considering that EvoSuite already achieves high coverage levels, demonstrating the added value of combining traditional test generation methods with advanced input extraction techniques like those used in \name.}


% % \highlight{Summary of \textbf{RQ4:} Incorporating relevant inputs extracted by \name enhances the adequacy of automatically generated test cases, resulting in higher code coverage. By leveraging the extracted inputs in the test generation process, the generated tests exhibit improved coverage of the software code, indicating the effectiveness of \name in enhancing test adequacy. It is worth noting that EvoSuite already achieves high levels of coverage by default, and the improvements observed indicate the potential of combining the baseline approach with the utilization of extracted inputs to increase the code coverage rate further.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{[RQ4]: Effect of \name-extracted inputs on code coverage}
\noindent\textbf{Experiment Goal: }
The objective of this experiment is to evaluate the impact of \name-extracted inputs on the code coverage achieved by automatically generated test cases. Specifically, the experiment aims to determine whether incorporating inputs extracted by \name from bug reports can improve the coverage metrics of the generated tests compared to those generated without any external inputs. This evaluation is crucial to understand the extent to which these inputs contribute to more thorough testing, thereby enhancing the detection of potential defects.

\noindent\textbf{Experiment Design: }
To assess the impact of \name-extracted inputs on test adequacy, we conducted a series of experiments focusing on key code coverage metrics, including branch, instruction, method, and line coverage. These metrics provide a quantitative measure of how extensively the test suite exercises the software code. The experiments were conducted using both EvoSuite and Randoop as the test generation tools on a selection of projects from the Defects4J dataset. 

For this experiment, we selected some recent versions of the same projects in the Defects4J dataset. The selected projects and their versions are as follows: Apache Commons Cli 1.5.0, Apache Commons Codec 1.15, Apache Commons Collections 4-4.4, Apache Commons Compress 1.2.1, Apache Commons Csv 1.9.0, Gson 2.9.1, Jackson-core 2.14-rc2, Jackson-dataformat-xml 2.14.0-rc2, Jackson-databind 2.14.0-rc2, Jsoup 1.15.3, Apache Commons Jxpath 1.3, Apache Commons Lang 3-3.12.0, Mockito 4.8.1, Joda Time 2.12.0.
We excluded projects Closure and Math because either Evosuite crashed, failed to generate tests, or generated uncompilable tests. 

The experimental setup was the same as in Section~\ref{RQ3-experiment-design}, each class had a three-minute time limit for test generation, with experiments conducted five times to ensure reliable results. The coverage was measured using the JaCoCo tool\footnote{https://github.com/jacoco/jacoco}, a widely used coverage measurement tool in the
literature.

\noindent\textbf{Experiment Results: }
Branch coverage results (Table~\ref{branch-coverage-results}) show that incorporating \name-extracted inputs generally led to improvements in many projects. Notably, using LLM-enhanced inputs (ProjLitLLM, AllLitLLM) resulted in the highest branch coverage in several projects, such as Codec (41.0\%), Collections (50.0\%), Compress (50.0\%), and Jsoup (50.0\%). These findings suggest that the use of LLM filtering refines the test inputs, leading to more comprehensive branch coverage. The results also indicate that EvoSuite, when combined with LLM-enhanced inputs, outperforms the baseline NoLit configuration across most projects.

%%%%%%%%%%%%%%%%%%%%%%%%%%BRANCH COVERAGE
\begin{table*}
    \centering
    %\caption{Branch coverage results for different experiments}
    \caption{Branch coverage results for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}
    
    \label{branch-coverage-results}
    %\scriptsize
    \scalebox{0.60}
    {
        \begin{tabular}{l|cccccccccccccc}
            \toprule
            & \multicolumn{14}{c}{Branch coverage (\%)} \\
            \cmidrule{2-15}
            Projects & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 50.0 & -- & 49.4 & -- & 49.8 & -- & 50 & -- & 50.0 & -- & 48.4 & -- & 49.0 & -- \\
            Codec & 38.0 & 50 & 38.8 & 50 & 40.6 & 50 & 40.6 & 50.0 & 41.0 & 50.0 & 37.8 & 50.0 & 38.0 & 50.0 \\
            Collections & 47.0 & 47 & 48.8 & \textbf{50} & 48.2 & \textbf{50} & 49.8 & \textbf{50.0} & \textbf{50.0} & \textbf{50.0} & 48.2 & 48.0 & 48.7 & 49.0 \\
            Compress & 49.2 & --. & 48.6 & -- & 49.0 & -- & 49.0 & --& \textbf{50.0} & -- & 48.0 & -- & 48.5 & -- \\
            Csv & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- \\
            Gson & 48.8 & 50 & 49.0 & 50 & 49.0 & 50 & 49.0 & 50.0 & 50.0 & 50.0 & 48.0 & 50.0 & 48.8 & 50.0 \\
            JacksonCore & 49.8 & 50 & 49.4 & 50 & 49.6 & 50 & 49.8 & 50.0 & 49.9 & 50.0 & 49.4 & 50.0 & 49.6 & 50.0 \\
            JacksonXml & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 49.9 & -- & 50.0 & -- \\
            Jsoup & 49.4 & 50 & 49.6 & 50 & 49.2 & 50 & 49.8 & 50.0 & 49.8 & 50.0 & 49.4 & 50.0 & 49.6 & 50.0 \\
            JxPath & 48.8 & 50 & 48.2 & 50 & 48.2 & 50 & 49.0 & 50.0 & 50.0 & 50.0 & 48.4 & 49.0 & 48.8 & 50.0 \\
            Lang & 49.4 & 50 & 49.0 & 50 & 49.2 & 48 & 49.4 & 50.0 & 50.0 & 50.0 & 49.0 & 48.0 & 49.2 & 49.0 \\
            Mockito & 50.0 & -- & 49.8 & -- & 49.4 & -- & 49.8 & -- & 50.0 & -- & 49.7 & -- & 49.7 & -- \\
            JacksonDatabind & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- & 50.0 & -- \\
            Time & 48.4 & 50 & 48.4 & 50 & 48.4 & 50 & 49.0 & 50.0 & 49.7 & 50.0 & 48.4 & 50.0 & 49.0 & 50.0 \\
            \bottomrule
        \end{tabular}
    }
     \vspace{3mm}
\end{table*}

Regarding instruction coverage (Table~\ref{instruction-coverage-results}) the results indicate that LLM-enhanced inputs provided significant improvements in several projects. For example, Cli reached 99.0\% instruction coverage with AllLitLLM, while JacksonCore and Jsoup achieved coverage rates of 99.0\% and 98.0\%, respectively. These results demonstrate that the LLM filtering process effectively enhances the relevance of the extracted inputs, leading to better instruction coverage. Randoop, while generally achieving high coverage, also benefited from LLM-enhanced inputs, although the improvements were less pronounced compared to EvoSuite.

%%%%%%%%%%%%%%%%%%%%%%%%%%INSTRUCTION COVERAGE
\begin{table*}
    \centering
    %\caption{Instruction coverage results for different experiments}
    \caption{Instruction coverage results for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}
    \label{instruction-coverage-results}
    % \scriptsize
    \scalebox{0.60}
    {
        \begin{tabular}{l|cccccccccccccc}
            \toprule
            & \multicolumn{14}{c}{Instruction coverage (\%)} \\
            \cmidrule{2-15}
            Projects & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 96.2 & -- & 97.8 & -- & 97.8 & -- & 98.0 & -- & \textbf{99.0} & -- & 96.0 & -- & 97.0 & -- \\
            Codec & 86.6 & 70.0 & 86.8 & 68.0 & 88.4 & 64.0 & 87.0 & 70.0 & \textbf{91.0} & 72.0 & 85.0 & 85.0 & 89.0 & 89.0 \\
            Collections & 94.4 & 64.0 & 95.2 & 75.0 & 94.8 & 70.0 & 95.0 & 75.0 & \textbf{97.0} & 70.0 & 95.0 & 95.0 & 95.0 & 95.0 \\
            Compress & 95.2 & -- & 96.6 & -- & 96.0 & -- & \textbf{97.0} & --& \textbf{97.0} & -- & 93.0 & -- & 96.0 & -- \\
            Csv & 99.0 & -- & 99.0 & -- & 99.0 & -- & 99.0 & -- & 99.0 & -- & 99.0 & -- & 99.0 & -- \\
            Gson & 94.6 & 72.0 & 95.4 & 69.0 & 95.4 & 74.0 & \textbf{98.0} & 72.0 & 97.0 & 75.0 & 95.0 & 95.0 & 96.0 & 96.0 \\
            JacksonCore & 96.8 & 57.0 & 98.4 & 64.0 & 98.2 & 58.0 & \textbf{99.0} & 62.0 & \textbf{99.0} & 64.0 & \textbf{99.0} & \textbf{99.0} & \textbf{99.0} & \textbf{99.0} \\
            JacksonXml & 96.4 & -- & 97.2 & -- & 96.6 & -- & 97.0 & -- & \textbf{98.0} & -- & 96.0 & -- & 97.0 & -- \\
            Jsoup & 96.8 & 78.0 & \textbf{98.0} & 87.0 & \textbf{98.0} & 86.0 & 97.0 & 85.0 & \textbf{98.0} & 89.0 & 97.0 & 97.0 & 97.0 & 97.0 \\
            JxPath & 95.4 & 94.0 & 96.6 & \textbf{98.0} & 96.0 & 97.0 & \textbf{98.0} & 97.0 & 97.0 & \textbf{98.0} & 96.0 & 96.0 & 96.0 & 96.0 \\
            Lang & 96.2 & 89.0 & 96.2 & 90.0 & 96.4 & 90.0 & 97.0 & 90.0 & \textbf{98.0} & 90.0 & 95.0 & 95.0 & 95.0 & 95.0 \\
            Mockito & 96.8 & -- & 97.0 & -- & 97.0 & -- & 97.0 & -- & \textbf{98.0} & -- & 96.0 & -- & 97.0 & -- \\
            JacksonDatabind & 96.4 & -- & 97.2 & -- & 97.4 & -- & 97.0 & -- & \textbf{98.0} & -- & 95.0 & -- & 96.0 & -- \\
            Time & 95.8 & 87.0 & \textbf{96.0} & 89.0 & 95.8 & 89.0 & \textbf{96.0} & 89.0 & \textbf{96.0} & 89.0 & \textbf{96.0} & \textbf{96.0} & \textbf{96.0} & \textbf{96.0} \\
            \bottomrule
        \end{tabular}
    }
    \vspace{3mm}
\end{table*}


Method coverage results (Table~\ref{method-coverage-results}) reveal that the incorporation of \name-extracted inputs, particularly when enhanced with LLM filtering, consistently achieved high coverage across almost all projects. Cli, JacksonCore, and Jsoup reached 100.0\% method coverage with several input configurations, indicating the effectiveness of these inputs in ensuring that all methods are exercised by the generated tests. The LLM-enhanced configurations (ProjLitLLM, AllLitLLM) often matched or slightly exceeded the baseline method coverage, underscoring their utility in generating comprehensive test suites.

%%%%%%%%%%%%%%%%%%%%%%%%%%METHOD COVERAGE
\begin{table*}
    \centering
    %\caption{Method coverage results for different experiments}
    \caption{Method coverage results for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}
    \label{method-coverage-results}
    % \scriptsize
    \scalebox{0.55}
    {
        \begin{tabular}{l|cccccccccccccc}
            \toprule
            & \multicolumn{14}{c}{Method coverage (\%)} \\
            \cmidrule{2-15}
            Projects & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 99.8 & -- & \textbf{100.0} & -- & \textbf{100.0} & -- & \textbf{100.0} & -- & \textbf{100.0} & -- & \textbf{100.0} & -- & \textbf{100.0} & -- \\
            Codec & 98.5 & 99.8 & 98.2 & \textbf{99.9} & 98.3 & \textbf{99.9} & 99.7 & 99.8 & \textbf{99.9} & \textbf{99.9} & 99.8 & 98.8 & 99.7 & 99.8 \\
            Collections & 99.7 & 99.8 & \textbf{100.0} & 99.8 & \textbf{100.0} & 99.8 & \textbf{100.0} & 99.8 & \textbf{100.0} & 99.9 & 98.31 & 99.8 & 99.0 & 99.8 \\
            Compress & 100.0 & -- & 100.0 & -- & 99.9 & -- & 99.98 & --& 100.0 & -- & 99.98 & -- & 99.98 & -- \\
            Csv & 100.0 & -- & 99.9 & -- & 100.0 & -- & 99.98 & -- & 100.0 & -- & 99.9 & -- & 100.0 & -- \\
            Gson & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 99.9 & 100.0 & 99.9 \\
            JacksonCore & 99.8 & 99.8 & \textbf{100.0} & 99.8 & \textbf{100.0} & 99.9 & \textbf{100.0} & 99.8 & \textbf{100.0} & 99.9 & 98.0 & 97.4 & 98.9 & 99.8 \\
            JacksonXml & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- \\
            Jsoup & 99.9 & 99.9 & \textbf{100.0} & 99.9 & \textbf{100.0} & 99.9 & \textbf{100.0} & 99.9 & \textbf{100.0} & 99.9 & 99.8 & 99.8 & \textbf{100.0} & 99.8.0 \\
            JxPath & 100.0 & 97.4 & 100.0 & 96.4 & 99.8 & 95.8 & 100.0 & 97.4 & 100.0 & 98.0 & 100.0 & 96.4 & 100.0 & 96.4 \\
            Lang & 100.0 & 99.97 & 98.3 & 99.8 & 100.0 & 99.8 & 99.98 & 99.97 & 100.0 & 99.98 & 96.9 & 98.0 & 98.0 & 98.8 \\
            Mockito & 99.8 & -- & 99.8 & -- & 99.6 & -- & \textbf{100.0} & -- & \textbf{100.0} & -- & 99.4 & -- & 99.4 & -- \\
            JacksonDatabind & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- & 100.0 & -- \\
            Time & 100.0 & 99.98 & 100.0 & 99.98 & 100.0 & 99.98 & 99.98 & 99.98 & 100.0 & 99.98 & 99.7 & 99.98 & 99.8 & 99.98 \\
            \bottomrule
        \end{tabular}
    }
    \vspace{3mm}
\end{table*}


Line coverage results (Table~\ref{line-coverage-results}) further affirm the benefits of integrating LLM-enhanced inputs into the test generation process. The AllLitLLM configuration yielded the highest line coverage in projects such as Cli (98.8\%), Codec (89.0\%), JacksonCore (99.6\%), and Jsoup (99.9\%). These improvements, though modest, are critical in ensuring that more lines of code are exercised during testing, which increases the likelihood of uncovering potential defects. The results also indicate that LLM-enhanced inputs consistently outperform the baseline NoLit configuration, particularly in more complex projects where achieving high coverage is challenging.


%%%%%%%%%%%%%%%%%%%%%%%%%%LINE COVERAGE
\begin{table*}
    \centering
    %\caption{Line coverage results for different experiments}
    \caption{Line coverage results for different experiments. Definitions of terms used: NoLit refers to experiments where no literals were used (baseline). ProjLit refers to the use of project-specific literals, and AllLit includes all literals from all projects. LLM indicates that filtering was performed using LLM, while LLMOnly means LLM was used alone to extract inputs. Evo denotes experiments conducted with EvoSuite, and Ran refers to those conducted with Randoop. "Databind" in the projects column refers to the jacksonDatabind project.}
    \label{line-coverage-results}
    % \scriptsize
    \scalebox{0.56}
    {
        \begin{tabular}{l|cccccccccccccc}
            \toprule
            & \multicolumn{14}{c}{Line coverage (\%)} \\
            \cmidrule{2-15}
            Projects & \multicolumn{2}{c|}{NoLit} & \multicolumn{2}{c|}{ProjLit} & \multicolumn{2}{c|}{AllLit} & \multicolumn{2}{c|}{ProjLitLLM} & \multicolumn{2}{c|}{AllLitLLM} & \multicolumn{2}{c|}{ProjLitLLMOnly} & \multicolumn{2}{c}{AllLitLLMOnly} \\
            & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran & Evo & Ran \\
            \midrule
            Cli & 96.7 & -- & 97.9 & -- & 98.1 & -- & 98.6 & -- & \textbf{98.8} & -- & 93.4 & -- & 95.2 & -- \\
            Codec & 85.2 & 69.39 & 85.9 & 70.44 & 87.2 & 70.8 & 85.0 & 70.9 & \textbf{89.0} & 71.0 & 83.0 & 69.46 & 83.5 & 70.8 \\
            Collections & 93.9 & 82.25 & 95.6 & 78.81 & 95.0 & 77.37 & 96.0 & 79.63 & \textbf{96.97} & 82.25 & 94.0 & 77.37 & 95.0 & 77.60 \\
            Compress & 94.7 & --. & 96.5 & -- & 96.5 & -- & 97.8 & --& \textbf{97.9} & -- & 94.6 & -- & 95.88 & -- \\
            Csv & 99.5 & -- & 99.6 & -- & 99.6 & -- & 99.7 & -- & \textbf{99.8} & -- & 99.1 & -- & 99.3 & -- \\
            Gson & 93.0 & 82.98 & 95.1 & 77.64 & 95.3 & 75.60 & 96.0 & 82.28 & \textbf{96.5} & 83.0 & 93.8 & 75.50 & 94.5 & 75.70 \\
            JacksonCore & 95.9 & 65.64 & 98.7 & 67.0 & 98.6 & 67.25 & 98.99 & 67.81 & \textbf{99.6} & 67.70 & 95.8 & 66.90 & 96.4 & 67.15 \\
            JacksonXml & 99.1 & -- & 99.3 & -- & 99.4 & -- & \textbf{99.5} & -- & 99.49 & -- & 97.3 & -- & 98.4 & -- \\
            Jsoup & 96.3 & 82.28 & 98.6 & 81.27 & 98.5 & 81.68 & 98.9 & 82.47 & \textbf{99.9} & 82.95 & 94.88 & 81.27 & 98.7 & 81.68 \\
            JxPath & 94.7 & 89.78 & 96.9 & 84.02 & 96.1 & 84.18 & 97.88 & 89.78 & \textbf{98.8} & 90.23 & 94.5 & 84.02 & 95.09 & 86.0 \\
            Lang & 96.5 & 90.98 & 96.9 & 90.63 & 96.9 & 91.12 & 96.98 & 91.65 & \textbf{97.9} & 92.0 & 93.0 & 90.98 & 95.24 & 91.12 \\
            Mockito & 96.3 & -- & 97.9 & -- & 98.0 & -- & 98.46 & -- & \textbf{98.9} & -- & 94.46 & -- & 95.32 & -- \\
            JacksonDatabind & 96.9 & -- & 98.0 & -- & 98.2 & -- & \textbf{98.99} & -- & \textbf{98.99} & -- & 96.23 & -- & 96.5 & -- \\
            Time & 96.0 & 92.71 & 96.3 & 93.01 & \textbf{96.9} & 93.38 & 96.47 & 93.45 & 96.47 & 93.80 & 95.33 & 92.71 & 95.9 & 92.71 \\
            \bottomrule
        \end{tabular}
    }
    \vspace{3mm}
\end{table*}



\highlight{Summary of \textbf{RQ4:} The integration of \name-extracted inputs in the test generation process has a noticeable positive impact on code coverage across various projects. On average, incorporating these inputs led to improvements in branch coverage (up to 2.0\%), instruction coverage (up to 3.0\%), method coverage (up to 1.5\%), and line coverage (up to 3.6\%) compared to the baseline with no inputs. Notable enhancements were observed in projects such as JacksonCore, Jsoup, and JxPath, where coverage metrics improved significantly with the use of LLM-filtered inputs. Although the improvements may seem modest, they are significant given that EvoSuite already achieves high baseline coverage. This demonstrates the added value of using \name to extract relevant inputs, contributing to more comprehensive test coverage and, by extension, higher software quality and reliability.
}

==> Sections/setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

% The goal of our empirical study is to determine if \name can extract relevant inputs from bug reports and to determine if these inputs improve the quality of tests generated by automated test generators.
% The research questions defined to address the feasibility of extracting relevant inputs from bug reports for enriching automatic test case generation will be introduced in the next subsection. This section also introduces the dataset and the testing environment. The implementation of our approach and all related data for the experiments of this paper is publicly available in a currently anonymous repository at: \url{https://anonymous.4open.science/r/BRMiner-C853}. 
% %\lp{add correct link}
The goal of our empirical study is to evaluate the effectiveness of \name in extracting relevant inputs from bug reports and to assess whether these inputs enhance the quality of tests generated by automated test generation tools such as EvoSuite and Randoop. BRMiner integrates a Large Language Model (LLM), specifically GPT-3.5-turbo, to refine the extracted inputs through a filtering process, thereby improving the relevance and effectiveness of the generated test cases. Additionally, we employed Randoop as a complementary test generation tool to benchmark our results against those obtained with EvoSuite. The prompts designed for the Tree of Thoughts (ToT) technique used in the LLM filtering process will also be discussed in detail.

In the following subsections, we present the research questions guiding our study, describe the dataset used for evaluation, and detail the experimental setup, including the LLM parameters, prompt design, and the testing environment. The implementation of our approach and all related experimental data is publicly available in a currently anonymous repository at: \url{https://anonymous.4open.science/r/BRMiner-C853}.

\subsection{Research Questions}
% \begin{itemize}
%     \item {\bf RQ1:} To what extent are relevant inputs from bug reports incorporated into manually written test cases by humans?
%     \item {\bf RQ2:} What is the rate of actual relevant inputs among the potential inputs extracted by \name?
%     \item {\bf RQ3:} Do tests generated using all the relevant inputs extracted by \name exhibit a higher bug detection rate compared to tests generated without utilizing these inputs?
%     \item {\bf RQ4:} Does the utilization of all extracted relevant inputs by \name result in higher code coverage compared to tests generated without using these inputs?
% \end{itemize}  
\vspace{0.2cm}\noindent\textbf{RQ1: To what extent are relevant inputs from bug reports incorporated into manually written test cases by humans?}
This research question seeks to explore the prevalence and consistency of relevant inputs from bug reports within manually written test cases. The goal is to determine: \ding{182}~How frequently developers include these inputs in their test cases when patching bugs; and \ding{183}~Whether BRMiner can automatically identify these relevant inputs that are commonly present in successful patched versions. The study will involve analyzing a large-scale dataset, such as Defects4J, by intersecting tokens from bug reports with literals extracted from test cases to measure alignment.

\vspace{0.2cm}\noindent\textbf{RQ2: What is the relevance of actual inputs among the potential inputs extracted by BRMiner?}
This question focuses on evaluating the efficacy of BRMiner in extracting relevant inputs from bug reports within the context of the Defects4J projects. The objective is to measure: \ding{182}~The proportion of extracted inputs that are genuinely useful for generating effective test cases; and \ding{183}~The tool’s effectiveness in minimizing irrelevant inputs. This evaluation is conducted using three configurations: BRMiner, the combination of Regex + Javalang in the BRMiner approach, and the baseline LLM alone.

\vspace{0.2cm}\noindent\textbf{RQ3: Do tests generated using all the relevant inputs extracted by BRMiner exhibit a higher bug detection rate compared to tests generated without utilizing these inputs?}
This research question examines whether the inclusion of inputs extracted by BRMiner enhances the bug detection capability of generated test cases. Specifically, it assesses: \ding{182}~Whether these extracted inputs lead to a higher rate of bug detection when compared to test cases generated without BRMiner's inputs; and \ding{183}~How the use of these inputs impacts the overall effectiveness of tools like EvoSuite and Randoop in identifying software defects.

\vspace{0.2cm}\noindent\textbf{RQ4: Does the utilization of all extracted relevant inputs by BRMiner result in higher code coverage compared to tests generated without using these inputs?}
This question aims to evaluate the impact of BRMiner’s extracted inputs on code coverage metrics in automatically generated test cases. The focus is on: \ding{182}~Determining whether incorporating these inputs results in more comprehensive exploration of the codebase; and \ding{183}~Assessing if these inputs help uncover additional execution paths that might be missed by standard test generation methods. The experiment will compare the code coverage metrics—such as branch, instruction, method, and line coverage—between test cases generated with and without BRMiner’s inputs.



\subsection{Dataset}
\label{subsec:dataset}
To address our research questions, we utilized the version 2.0.0 of Defects4J~\citep{just2014defects4j}, an open-source database designed for software testing and debugging research. Defects4J provides a collection of real software defects described in user-written bug reports, each project consisting of a buggy program version and a fixed program version. Since our study focuses on the use of bug reports, JFreeChart was excluded due to the lack of sufficient and consistent bug report information.

\subsection{Large Language Model}
\label{subsec:large-language-model}
In our study, we utilized OpenAI's GPT-3.5-turbo model to enhance the relevance of extracted inputs from bug reports in the BRMiner approach. GPT-3.5-turbo is a state-of-the-art language model with a token limit of 4,096 tokens, which includes both the input and output tokens in each interaction. To optimize the model's performance, we set the token limit to the maximum allowable, ensuring that as much contextual information as possible could be included in each prompt.

For the filtering process, we maintained the model's default parameters, setting the temperature to 0.7 to balance creativity and coherence in the generated outputs. The temperature setting controls the randomness of the model's predictions, with a value of 0.7 providing a good mix of deterministic and diverse responses.

To manage the token limits effectively, especially given the potential length of bug reports, we employed OpenAI’s tiktoken\footnote{\url{https://github.com/openai/tiktoken}} library. This library allowed us to count and manage tokens within prompts, ensuring that we stayed within the model's constraints while maximizing the information provided to the model. When necessary, we adjusted the content of the prompts by prioritizing key elements such as the title, description, comments, and extracted inputs, while omitting less critical information to avoid exceeding the token limit. This approach enabled us to leverage the full capacity of GPT-3.5-turbo for refining input relevance in our experiments.


\subsection{Prompt Design}
\label{subsec:prompt-design}
Effective prompt design is crucial in leveraging Large Language Models (LLMs) for tasks such as input refinement in test case generation. Drawing inspiration from established research in unit test generation~\citep{siddiq2024using, chen2023chatunitest, tang2024chatgpt}, we carefully crafted prompts to guide the LLMs toward extracting relevant and high-quality inputs. Our approach leverages the Tree of Thoughts (ToT) prompting technique, which helps the LLM explore different reasoning paths and refine its output based on the contextual information provided.
Each prompt consists of two key components: a Natural Language Description (NLD) that outlines the task and a Contextual Data Placeholder (CDP) that includes extracted inputs and relevant bug report details. We will delve into the specifics of each part and explain how they contribute to the overall effectiveness of the BRMiner approach.
\begin{itemize}[leftmargin=0.2cm]

\item \textbf{Natural Language Description:} The NLD is designed to clearly and concisely instruct the LLM on the task at hand. It includes:
\begin{itemize}
    \item (i) A role-playing directive that positions the LLM as a software engineering expert tasked with analyzing bug reports, enhancing the model’s focus on identifying relevant inputs~\citep{chen2023chatunitest, tang2024chatgpt}.
    \item (ii) A task-specific directive to identify and refine potential test inputs from the provided bug report details, guiding the LLM to consider both the extracted literals and the semantic context of the bug.
    \item (iii) A control statement that requires the output to be formatted in a structured JSON format, ensuring the results are easy to parse and integrate into the test generation process.
\end{itemize}

\item \textbf{Contextual Data:} This section of the prompt varies depending on the configuration:
\begin{itemize}
    \item (i) For the BRMiner configuration, the prompt includes the extracted literals (strings and numeric values) from the bug reports, as well as the title, description, and comments. This combination allows the LLM to refine the inputs based on both raw data and the broader context provided by the bug report.
    \item (ii) For the LLM Alone baseline, the prompt consists only of the bug report details without any pre-extracted inputs, allowing the LLM to independently generate potential test inputs.
\end{itemize}

\end{itemize}


The design of these prompts is illustrated in Figure~\ref{fig:prompt-templates}, which provides examples of the ToT prompts used in both the BRMiner approach and the LLM Alone baseline. By structuring the prompts in this manner, we aim to harness the full potential of GPT-3.5-turbo in refining and generating inputs that are both relevant and effective for test case generation.

\begin{figure}[ht]
\centering

\begin{minipage}[b]{\textwidth}
    \centering
    \fbox{\parbox{\textwidth}{
        \captionof{subfigure}{ToT Prompting in LLM Alone Baseline}
        \texttt{
Imagine three different software engineering experts working on maintaining a software project hosted on GitHub or Jira. Their task is to analyze a bug report, specifically its Title, Description, and Comments, to identify potential test inputs that can trigger the described bug. 
Consider the following bug report with title \textbf{[Title]}. Below is the description of the bug report:\textbf{[Description]}.
Here are the comments associated with the bug report: \textbf{[Comments]}
Each expert should propose potential inputs classified as String, Float, Integer, that could be relevant for triggering the bug. They must discuss the relevance of these inputs and discard any that are deemed irrelevant. Finally, they should compile a list of relevant inputs in the following JSON format for ease of use:
\textbf{[JSON\_FORMAT]}
Please ensure the complete JSON file is placed between the three quotes \textbf{``` ```} for easy extraction.
        }
        \label{fig:tot-llm}
    }}
\end{minipage}

\vspace{3mm} % Espace entre les sous-figures

\begin{minipage}[b]{\textwidth}
    \centering
    \fbox{\parbox{\textwidth}{
        \captionof{subfigure}{ToT Prompting in BRMiner Approach}
        \texttt{
Imagine three different software engineering experts working on maintaining a software project hosted on GitHub or Jira. Their task is to analyze the contents of a bug report, including its Title, Description, and Comments, to determine potential test inputs that could be used to trigger the described bug.
Consider the following bug report with title \textbf{[Title]}. Below is the description of the bug report: \textbf{[Description]}.
Here are the comments associated with the bug report: \textbf{[Comments]}
The following inputs have been automatically extracted from this bug report: \textbf{[INPUTS-LIST]}.
The experts must analyze both the bug report and these extracted inputs, then select relevant inputs classified as String, Float, Integer. They should discuss the relevance of all chosen inputs, discarding any that are deemed irrelevant. Finally, they should compile a complete list of relevant inputs in the following JSON format:
\textbf{[JSON\_FORMAT]}
Please ensure the complete JSON file is placed between the three quotes \textbf{``` ```} for easy extraction.
        }
        \label{fig:tot-brminer}
    }}
\end{minipage}

\caption{Examples of ToT prompt design used for relevant inputs extraction.}
\label{fig:prompt-templates}
\vspace{3mm}
\end{figure}


\subsection{Testing Environment}
% We used EvoSuite\footnote{\url{https://github.com/EvoSuite/evosuite}} for our experiments. We used version 1.2.1, the latest available version to utilize the latest features and improvements available at the time of our study. Regarding the generation of the test suite, our modification of EvoSuite's source code involves the inclusion of \name inputs into EvoSuite static input pool, effectively using these inputs as seed inputs within EvoSuite (Figure~\ref{fig:approach}) in addition to those from the dynamic pool. By this process we can transform inputs from \name into test cases.

% % Regarding the time budget for test generation, we allocated respectively one minute and three minutes per class. 
% The optimal time budget for EvoSuite test generation can vary depending on factors such as code complexity and testing objectives. Researchers have used different time budgets in their studies, considering practical considerations and code characteristics. In our study, we chose a realistic time budget of three minutes per test case generation, which aligns with acceptable time constraints typically considered by developers. Previous work~\citep{fraser2015does,arcuri2013parameter,inproceedings,shamshiri2015automatically} has shown that the three-minute time budget is in most cases, sufficient for EvoSuite. This choice ensures that the experiments are conducted within a reasonable timeframe while accounting for real-world constraints.
% %\jk{I do not understand. Is it 1 min or 3 min? please clarify. Do you want to say: "up to 3 min"?  }

% We utilized the Dynamic Symbolic Execution approach for test generation, using branch, method, and line coverage as criteria. To achieve our objectives of bug detection and comprehensive testing, we disabled the minimization option in EvoSuite, which is enabled by default. Additionally, assertion minimization was disabled to maintain the comprehensiveness of the generated tests. All other parameters were set to their default settings, ensuring consistency with commonly adopted configurations in the research community.

% To ensure reliable and robust results, we performed the experiments in five iterations and aggregated the outcomes. This iterative approach helps mitigate the impact of random variations and ensures the stability of our findings.
% Experiments on EvoSuite are conducted on a machine with AMD EPYC 7552 48-Core Processor, 3.2 GHz and 640 GB RAM but not all of these resources were allocated to our experiments..

% %The experiments on bug detection and code coverage were conducted on specific open-source Java projects from the Defects4J benchmark, as described in Section~\ref{subsec:dataset}.
\subsubsection{EvoSuite SBST Tool}
For our experiments, we ussed EvoSuite\footnote{\url{https://github.com/EvoSuite/evosuite}} version 1.2.1, the latest version available at the time of our study. EvoSuite is a Search-Based Software Testing (SBST) tool that automatically generates test cases with a focus on maximizing code coverage. To integrate BRMiner, we modified EvoSuite's source code to include inputs extracted by BRMiner into EvoSuite's static input pool (Figure~\ref{fig:approach}). This modification allowed us to use BRMiner’s inputs as seed inputs, enhancing the generation of test cases that are more aligned with the real-world scenarios described in bug reports.

Dynamic Symbolic Execution (DSE) was employed during test generation, with branch, method, and line coverage as the primary criteria. We disabled the minimization option in EvoSuite to maintain comprehensive test generation, ensuring that all possible scenarios are tested. Assertion minimization was also disabled to preserve the thoroughness of the generated tests. All other EvoSuite parameters were left at their default settings to align with standard practices in the research community.

To ensure robustness and reliability, each experiment was repeated five times, with results aggregated across these iterations. This iterative approach helps reduce the impact of random variations, providing a more stable and accurate evaluation of the tool’s performance.

\subsubsection{Randoop}
We also conducted experiments using Randoop\footnote{\url{https://randoop.github.io/randoop/}} version 4.3.1, a feedback-directed random testing tool. Randoop automatically generates unit tests for Java programs by randomly combining methods and constructors, then executing them to detect unexpected behavior or crashes. Randoop produces two types of unit tests: error-revealing tests and regression tests. For this study, we focused on error-revealing tests, which are designed to identify potential errors in the classes under test. These tests are particularly useful for detecting exceptions or errors during the execution of the generated tests.

To handle potential issues such as infinite loops or methods that wait for user input, we configured Randoop to run each test in a separate thread by setting the --usethreads option to true. The --call-timeout was set to its default value of 5000 milliseconds, ensuring that any non-returning method calls are stopped forcefully after the specified time limit. This setup helps prevent Randoop from stalling during test generation, although it does result in a decrease in generation speed.

\subsubsection{Time Budget}
For both EvoSuite and Randoop, we allocated a time budget of three minutes per test case generation. This time budget was selected based on practical considerations, as it aligns with the typical constraints faced by developers. Previous studies~\citep{fraser2015does, arcuri2013parameter, shamshiri2015automatically} have demonstrated that a three-minute time budget is sufficient for effective test case generation in most cases. This consistent time budget across tools ensures comparability between the results obtained from EvoSuite and Randoop.

\subsubsection{Hardware}
All experiments were conducted on a machine equipped with an AMD EPYC 7552 48-Core Processor running at 3.2 GHz, with 640 GB of RAM. While not all of these resources were allocated for the experiments, the hardware provided sufficient computational power to run the experiments efficiently within the allotted time budget. This setup ensures that the results are reliable and reproducible under similar conditions.







